A Practical Walk-on-Boundary Method for Boundary Value Problems

We introduce the walk-on-boundary (WoB) method for solving boundary value problems to computer graphics. WoB is a grid-free Monte Carlo solver for certain classes of second order partial differential equations. A similar Monte Carlo solver, the walk-on-spheres (WoS) method, has been recently popularized in computer graphics due to its advantages over traditional spatial discretization-based alternatives. We show that WoB's intrinsic properties yield further advantages beyond those of WoS. Unlike WoS, WoB naturally supports various boundary conditions (Dirichlet, Neumann, Robin, and mixed) for both interior and exterior domains. WoB builds upon boundary integral formulations, and it is mathematically more similar to light transport simulation in rendering than the random walk formulation of WoS. This similarity between WoB and rendering allows us to implement WoB on top of Monte Carlo ray tracing, and to incorporate advanced rendering techniques (e.g., bidirectional estimators with multiple importance sampling, the virtual point lights method, and Markov chain Monte Carlo) into WoB. WoB does not suffer from the intrinsic bias of WoS near the boundary and can estimate solutions precisely on the boundary. Our numerical results highlight the advantages of WoB over WoS as an attractive alternative to solve boundary value problems based on Monte Carlo.

==> Figures/2DResults/Exterior/Dirichlet.tex <==
10000 0.785454
20000 0.568678
30000 0.469626
40000 0.411916
50000 0.374561
60000 0.347385
70000 0.324748
80000 0.307208
90000 0.293868
100000 0.282527
110000 0.272456
120000 0.2643
130000 0.257672
140000 0.250341
150000 0.243667
160000 0.23909
170000 0.23421
180000 0.229896
190000 0.226129
200000 0.222468
210000 0.219157
220000 0.216606
230000 0.213684
240000 0.211676
250000 0.209628
260000 0.207887
270000 0.20548
280000 0.203727
290000 0.201881
300000 0.199754
310000 0.197724
320000 0.196567
330000 0.194909
340000 0.1934
350000 0.191939
360000 0.190914
370000 0.189816
380000 0.188411
390000 0.187366
400000 0.186464
410000 0.18595
420000 0.185152
430000 0.183926
440000 0.182876
450000 0.181879
460000 0.18099
470000 0.180283
480000 0.179431
490000 0.178561
500000 0.177862
510000 0.177277
520000 0.17657
530000 0.175957
540000 0.175292
550000 0.174748
560000 0.174245
570000 0.173732
580000 0.173007
590000 0.17232
600000 0.171915
610000 0.171157
620000 0.170443
630000 0.169887
640000 0.169623
650000 0.168844
660000 0.16852
670000 0.168215
680000 0.167685
690000 0.167135
700000 0.166604
710000 0.166129
720000 0.165805
730000 0.165303
740000 0.164861
750000 0.164331
760000 0.163879
770000 0.163679
780000 0.163284
790000 0.162906
800000 0.162454
810000 0.162319
820000 0.162191
830000 0.16185
840000 0.161617
850000 0.161348
860000 0.161051
870000 0.160909
880000 0.160733
890000 0.160292
900000 0.160072
910000 0.159932
920000 0.159767
930000 0.159501
940000 0.159329
950000 0.159046
960000 0.158862
970000 0.15848
980000 0.158171
990000 0.158099
1000000 0.157974
1010000 0.157798
1020000 0.157665
1030000 0.157485
1040000 0.157307
1050000 0.157111
1060000 0.156799
1070000 0.156711
1080000 0.156534
1090000 0.156396
1100000 0.156251
1110000 0.156108
1120000 0.155795
1130000 0.155626
1140000 0.155516
1150000 0.155291
1160000 0.155094
1170000 0.155018
1180000 0.154854
1190000 0.154881
1200000 0.154689
1210000 0.154535
1220000 0.154325
1230000 0.154123
1240000 0.15399
1250000 0.153896
1260000 0.153727
1270000 0.153618
1280000 0.153557
1290000 0.153415
1300000 0.15329
1310000 0.153227
1320000 0.153096
1330000 0.153029
1340000 0.152833
1350000 0.15267
1360000 0.152534
1370000 0.152298
1380000 0.152215
1390000 0.152104
1400000 0.152036
1410000 0.151989
1420000 0.151894
1430000 0.151749
1440000 0.151676
1450000 0.151481
1460000 0.151298
1470000 0.15127
1480000 0.151236
1490000 0.151079
1500000 0.150934
1510000 0.150856
1520000 0.150787
1530000 0.150812
1540000 0.150766
1550000 0.150696
1560000 0.150583
1570000 0.150458
1580000 0.150333
1590000 0.150297
1600000 0.150253
1610000 0.150268
1620000 0.150174
1630000 0.150112
1640000 0.15006
1650000 0.149894
1660000 0.149796
1670000 0.149729
1680000 0.149625
1690000 0.149502
1700000 0.14941
1710000 0.149343
1720000 0.149272
1730000 0.14922
1740000 0.149258
1750000 0.149232
1760000 0.149202
1770000 0.149117
1780000 0.148982
1790000 0.148965
1800000 0.148784
1810000 0.148749
1820000 0.148667
1830000 0.148521
1840000 0.14833
1850000 0.148323
1860000 0.148148
1870000 0.148051
1880000 0.148027
1890000 0.147926
1900000 0.147912
1910000 0.14785
1920000 0.147721
1930000 0.147712
1940000 0.147683
1950000 0.147546
1960000 0.14746
1970000 0.147444
1980000 0.147399
1990000 0.147377
2000000 0.147351
2010000 0.147312
2020000 0.14735
2030000 0.147337
2040000 0.147264
2050000 0.147141
2060000 0.147142
2070000 0.147067
2080000 0.147047
2090000 0.147043
2100000 0.147043
2110000 0.146968
2120000 0.146979
2130000 0.146934
2140000 0.146852
2150000 0.146866
2160000 0.146831
2170000 0.146804
2180000 0.146801
2190000 0.146779
2200000 0.146755
2210000 0.146657
2220000 0.146577
2230000 0.146478
2240000 0.146413
2250000 0.146358
2260000 0.14639
2270000 0.146336
2280000 0.146297
2290000 0.146295
2300000 0.146251
2310000 0.146208
2320000 0.146149
2330000 0.146131
2340000 0.146133
2350000 0.1461
2360000 0.146078
2370000 0.146015
2380000 0.145938
2390000 0.145856
2400000 0.145826
2410000 0.145721
2420000 0.145716
2430000 0.145644
2440000 0.145538
2450000 0.145508
2460000 0.1455
2470000 0.145452
2480000 0.145435
2490000 0.145391
2500000 0.145285
2510000 0.145277
2520000 0.145269
2530000 0.145248
2540000 0.145264
2550000 0.145197
2560000 0.145115
2570000 0.145095
2580000 0.145007
2590000 0.144956
2600000 0.14496
2610000 0.144966
2620000 0.144909
2630000 0.14485
2640000 0.144766
2650000 0.144749
2660000 0.14477
2670000 0.14471
2680000 0.144669
2690000 0.144663
2700000 0.144656
2710000 0.144642
2720000 0.144646
2730000 0.144559
2740000 0.144503
2750000 0.144466
2760000 0.144427
2770000 0.144367
2780000 0.144338
2790000 0.144345
2800000 0.144355
2810000 0.144309
2820000 0.144274
2830000 0.144278
2840000 0.144284
2850000 0.144288
2860000 0.144289
2870000 0.144296
2880000 0.144314
2890000 0.144256
2900000 0.144193
2910000 0.144125
2920000 0.144083
2930000 0.14406
2940000 0.144063
2950000 0.144058
2960000 0.143993
2970000 0.143976
2980000 0.143956
2990000 0.143933
3000000 0.143895
3010000 0.143854
3020000 0.143841
3030000 0.143806
3040000 0.1438
3050000 0.143779
3060000 0.143768
3070000 0.143741
3080000 0.143657
3090000 0.143629
3100000 0.143546
3110000 0.143504
3120000 0.14347
3130000 0.143443
3140000 0.143414
3150000 0.143416
3160000 0.143397
3170000 0.143404
3180000 0.143362
3190000 0.14333
3200000 0.143341
3210000 0.143289
3220000 0.143262
3230000 0.143284
3240000 0.143317
3250000 0.143272
3260000 0.143243
3270000 0.143189
3280000 0.143206
3290000 0.143173
3300000 0.14318
3310000 0.143184
3320000 0.143204
3330000 0.143175
3340000 0.143166
3350000 0.143143
3360000 0.143119
3370000 0.14305
3380000 0.143113
3390000 0.143096
3400000 0.143091
3410000 0.143031
3420000 0.143028
3430000 0.143018
3440000 0.143032
3450000 0.143021
3460000 0.142998
3470000 0.142982
3480000 0.142943
3490000 0.142916
3500000 0.142892
3510000 0.142876
3520000 0.142848
3530000 0.142816
3540000 0.142785
3550000 0.142791
3560000 0.142779
3570000 0.142734
3580000 0.142746
3590000 0.142743
3600000 0.142746
3610000 0.142767
3620000 0.142775
3630000 0.142732
3640000 0.14271
3650000 0.142708
3660000 0.142711
3670000 0.142694
3680000 0.142684
3690000 0.142703
3700000 0.14267
3710000 0.142618
3720000 0.142625
3730000 0.142652
3740000 0.14263
3750000 0.142623
3760000 0.142611
3770000 0.142589
3780000 0.142567
3790000 0.142552
3800000 0.142543
3810000 0.142523
3820000 0.142482
3830000 0.142496
3840000 0.142474
3850000 0.142468
3860000 0.142458
3870000 0.142475
3880000 0.142464
3890000 0.142453
3900000 0.142408
3910000 0.14239
3920000 0.142448
3930000 0.142412
3940000 0.142385
3950000 0.142368
3960000 0.142364
3970000 0.142337
3980000 0.142324
3990000 0.142336
4000000 0.142343
4010000 0.14233
4020000 0.142311
4030000 0.142297
4040000 0.142283
4050000 0.142264
4060000 0.142248
4070000 0.142215
4080000 0.142218
4090000 0.142199
4100000 0.142202
4110000 0.142171
4120000 0.142168
4130000 0.142179
4140000 0.142159
4150000 0.14217
4160000 0.142177
4170000 0.142159
4180000 0.142139
4190000 0.142127
4200000 0.142105
4210000 0.14211
4220000 0.14208
4230000 0.142062
4240000 0.142051
4250000 0.142057
4260000 0.142065
4270000 0.142067
4280000 0.142035
4290000 0.142043
4300000 0.142026
4310000 0.142015
4320000 0.142035
4330000 0.142026
4340000 0.142015
4350000 0.142005
4360000 0.141994
4370000 0.14201
4380000 0.142
4390000 0.14196
4400000 0.141959
4410000 0.141987
4420000 0.141958
4430000 0.141977
4440000 0.14198
4450000 0.141964
4460000 0.141977
4470000 0.141975
4480000 0.141952
4490000 0.14194
4500000 0.141922
4510000 0.141945
4520000 0.141901
4530000 0.141893
4540000 0.141868
4550000 0.14189
4560000 0.141872
4570000 0.141879
4580000 0.141839
4590000 0.141815
4600000 0.141784
4610000 0.141759
4620000 0.141746
4630000 0.141745
4640000 0.141751
4650000 0.141711
4660000 0.141707
4670000 0.141687
4680000 0.141678
4690000 0.141673
4700000 0.141645
4710000 0.141628
4720000 0.141623
4730000 0.141624
4740000 0.141621
4750000 0.141573
4760000 0.141582
4770000 0.141563
4780000 0.141547
4790000 0.141541
4800000 0.141528
4810000 0.141519
4820000 0.141508
4830000 0.141525
4840000 0.141522
4850000 0.141506
4860000 0.141511
4870000 0.1415
4880000 0.141476
4890000 0.141439
4900000 0.141448
4910000 0.141418
4920000 0.141412
4930000 0.141397
4940000 0.141392
4950000 0.141373
4960000 0.14136
4970000 0.141369
4980000 0.141369
4990000 0.141375
5000000 0.141353
5010000 0.141373
5020000 0.141371
5030000 0.141391
5040000 0.141381
5050000 0.14137
5060000 0.141385
5070000 0.141376
5080000 0.141346
5090000 0.141332
5100000 0.141305
5110000 0.141291
5120000 0.141259
5130000 0.141244
5140000 0.141236
5150000 0.141234
5160000 0.141228
5170000 0.141211
5180000 0.141189
5190000 0.141206
5200000 0.141185
5210000 0.141174
5220000 0.141168
5230000 0.141146
5240000 0.141134
5250000 0.141136
5260000 0.141134
5270000 0.141151
5280000 0.14114
5290000 0.141176
5300000 0.141184
5310000 0.141162
5320000 0.141147
5330000 0.141165
5340000 0.141141
5350000 0.141101
5360000 0.141091
5370000 0.141095
5380000 0.141073
5390000 0.141085
5400000 0.141057
5410000 0.141047
5420000 0.141034
5430000 0.141005
5440000 0.14098
5450000 0.14097
5460000 0.140943
5470000 0.140948
5480000 0.140955
5490000 0.140954
5500000 0.140971
5510000 0.140963
5520000 0.140959
5530000 0.140947
5540000 0.140922
5550000 0.140944
5560000 0.140934
5570000 0.14094
5580000 0.140933
5590000 0.140938
5600000 0.140952
5610000 0.140935
5620000 0.14092
5630000 0.14088
5640000 0.140854
5650000 0.140854
5660000 0.140861
5670000 0.140854
5680000 0.140871
5690000 0.140866
5700000 0.140876
5710000 0.140854
5720000 0.140854
5730000 0.140853
5740000 0.140858
5750000 0.140839
5760000 0.140822
5770000 0.140822
5780000 0.140811
5790000 0.14077
5800000 0.140759
5810000 0.140777
5820000 0.140741
5830000 0.140718
5840000 0.140698
5850000 0.140697
5860000 0.14071
5870000 0.140707
5880000 0.140678
5890000 0.140657
5900000 0.140639
5910000 0.140652
5920000 0.140633
5930000 0.140615
5940000 0.140614
5950000 0.140615
5960000 0.140589
5970000 0.140584
5980000 0.140549
5990000 0.140549
6000000 0.140551
6010000 0.140558
6020000 0.140552
6030000 0.140541
6040000 0.14051
6050000 0.14051
6060000 0.140522
6070000 0.140508
6080000 0.140515
6090000 0.140504
6100000 0.140509
6110000 0.140531
6120000 0.140513
6130000 0.140494
6140000 0.140487
6150000 0.140472
6160000 0.140462
6170000 0.140459
6180000 0.140491
6190000 0.140487
6200000 0.140496
6210000 0.140491
6220000 0.140474
6230000 0.14049
6240000 0.14048
6250000 0.140454
6260000 0.140443
6270000 0.140428
6280000 0.140425
6290000 0.140408
6300000 0.14039
6310000 0.140396
6320000 0.140394
6330000 0.140411
6340000 0.140384
6350000 0.140386
6360000 0.140372
6370000 0.140392
6380000 0.14038
6390000 0.140384
6400000 0.140366
6410000 0.140356
6420000 0.140339
6430000 0.140332
6440000 0.140344
6450000 0.14035
6460000 0.140361
6470000 0.140342
6480000 0.140331
6490000 0.140331
6500000 0.14032
6510000 0.140302
6520000 0.140278
6530000 0.140284
6540000 0.140283
6550000 0.140264
6560000 0.140237
6570000 0.14024
6580000 0.140229
6590000 0.140215
6600000 0.140208
6610000 0.140199
6620000 0.140197
6630000 0.140201
6640000 0.140199
6650000 0.140191
6660000 0.140184
6670000 0.140189
6680000 0.140218
6690000 0.140201
6700000 0.140237
6710000 0.140235
6720000 0.140253
6730000 0.140267
6740000 0.140286
6750000 0.140284
6760000 0.140273
6770000 0.140271
6780000 0.140256
6790000 0.140212
6800000 0.140198
6810000 0.140185
6820000 0.140179
6830000 0.140174
6840000 0.140172
6850000 0.140158
6860000 0.140144
6870000 0.140156
6880000 0.140138
6890000 0.140119
6900000 0.14011
6910000 0.140108
6920000 0.140093
6930000 0.14009
6940000 0.140101
6950000 0.140086
6960000 0.140076
6970000 0.140091
6980000 0.140074
6990000 0.140049
7000000 0.140055
7010000 0.140039
7020000 0.140024
7030000 0.140024
7040000 0.140027
7050000 0.140043
7060000 0.140043
7070000 0.140046
7080000 0.140057
7090000 0.140058
7100000 0.140047
7110000 0.140043
7120000 0.140042
7130000 0.140055
7140000 0.140031
7150000 0.140025
7160000 0.14003
7170000 0.14001
7180000 0.13999
7190000 0.139989
7200000 0.139979
7210000 0.139983
7220000 0.139962
7230000 0.139957
7240000 0.139951
7250000 0.13996
7260000 0.13997
7270000 0.139981
7280000 0.139977
7290000 0.139974
7300000 0.139986
7310000 0.14
7320000 0.140016
7330000 0.140017
7340000 0.140025
7350000 0.140015
7360000 0.139989
7370000 0.139987
7380000 0.139995
7390000 0.140003
7400000 0.139995
7410000 0.139989
7420000 0.139987
7430000 0.139969
7440000 0.13995
7450000 0.139924
7460000 0.139914
7470000 0.139915
7480000 0.139928
7490000 0.139915
7500000 0.139897
7510000 0.139885
7520000 0.139887
7530000 0.139885
7540000 0.139867
7550000 0.139871
7560000 0.139857
7570000 0.139847
7580000 0.139856
7590000 0.139862
7600000 0.139862
7610000 0.139846
7620000 0.139837
7630000 0.139846
7640000 0.13985
7650000 0.139848
7660000 0.139837
7670000 0.139826
7680000 0.139822
7690000 0.139826
7700000 0.139845
7710000 0.139852
7720000 0.139837
7730000 0.139838
7740000 0.139832
7750000 0.139815
7760000 0.139811
7770000 0.139809
7780000 0.139822
7790000 0.139824
7800000 0.139825
7810000 0.139825
7820000 0.139813
7830000 0.139807
7840000 0.139807
7850000 0.139787
7860000 0.139791
7870000 0.139796
7880000 0.13981
7890000 0.139808
7900000 0.139811
7910000 0.139805
7920000 0.139792
7930000 0.139804
7940000 0.139792
7950000 0.139801
7960000 0.139794
7970000 0.13979
7980000 0.13979
7990000 0.139778
8000000 0.139763
8010000 0.139752
8020000 0.139747
8030000 0.139755
8040000 0.139746
8050000 0.139743
8060000 0.139741
8070000 0.139737
8080000 0.139732
8090000 0.139735
8100000 0.139728
8110000 0.139738
8120000 0.139739
8130000 0.139741
8140000 0.139725
8150000 0.13972
8160000 0.139714
8170000 0.139708
8180000 0.139704
8190000 0.139691
8200000 0.139698
8210000 0.139702
8220000 0.139696
8230000 0.139685
8240000 0.139687
8250000 0.13968
8260000 0.13967
8270000 0.139657
8280000 0.139663
8290000 0.139666
8300000 0.139657
8310000 0.139645
8320000 0.139629
8330000 0.139633
8340000 0.139639
8350000 0.139629
8360000 0.139625
8370000 0.139611
8380000 0.139605
8390000 0.139618
8400000 0.139638
8410000 0.13964
8420000 0.13965
8430000 0.139638
8440000 0.139635
8450000 0.139631
8460000 0.139628
8470000 0.139612
8480000 0.139613
8490000 0.139602
8500000 0.139605
8510000 0.139617
8520000 0.139619
8530000 0.139602
8540000 0.13961
8550000 0.139611
8560000 0.139604
8570000 0.139594
8580000 0.139593
8590000 0.139579
8600000 0.139584
8610000 0.139603
8620000 0.139614
8630000 0.13961
8640000 0.139601
8650000 0.139587
8660000 0.139575
8670000 0.139583
8680000 0.13956
8690000 0.139552
8700000 0.139541
8710000 0.139531
8720000 0.139526
8730000 0.13951
8740000 0.139523
8750000 0.13952
8760000 0.139524
8770000 0.139526
8780000 0.139522
8790000 0.139533
8800000 0.139529
8810000 0.139536
8820000 0.13953
8830000 0.139512
8840000 0.139504
8850000 0.139507
8860000 0.139519
8870000 0.139526
8880000 0.139524
8890000 0.13951
8900000 0.139517
8910000 0.139521
8920000 0.139524
8930000 0.139515
8940000 0.139504
8950000 0.139506
8960000 0.139513
8970000 0.139517
8980000 0.139485
8990000 0.13949
9000000 0.139474
9010000 0.139476
9020000 0.139493
9030000 0.139488
9040000 0.139482
9050000 0.139469
9060000 0.139474
9070000 0.139467
9080000 0.13947
9090000 0.139472
9100000 0.13946
9110000 0.139467
9120000 0.139455
9130000 0.139456
9140000 0.139448
9150000 0.139423
9160000 0.139404
9170000 0.139403
9180000 0.139399
9190000 0.139382
9200000 0.139384
9210000 0.139391
9220000 0.139387
9230000 0.139357
9240000 0.139351
9250000 0.139346
9260000 0.139342
9270000 0.139331
9280000 0.139329
9290000 0.139342
9300000 0.139327
9310000 0.139327
9320000 0.139315
9330000 0.139311
9340000 0.139318
9350000 0.139316
9360000 0.139315
9370000 0.139311
9380000 0.139306
9390000 0.139295
9400000 0.139284
9410000 0.139285
9420000 0.139284
9430000 0.139277
9440000 0.13928
9450000 0.139288
9460000 0.139303
9470000 0.139303
9480000 0.139297
9490000 0.139307
9500000 0.139303
9510000 0.139299
9520000 0.139297
9530000 0.139294
9540000 0.139294
9550000 0.1393
9560000 0.139295
9570000 0.139291
9580000 0.139276
9590000 0.139266
9600000 0.139265
9610000 0.139271
9620000 0.139272
9630000 0.139264
9640000 0.139257
9650000 0.13927
9660000 0.139266
9670000 0.139253
9680000 0.139261
9690000 0.139265
9700000 0.13925
9710000 0.139255
9720000 0.139256
9730000 0.139242
9740000 0.139234
9750000 0.139234
9760000 0.139234
9770000 0.139215
9780000 0.139214
9790000 0.139217
9800000 0.139213
9810000 0.139212
9820000 0.1392
9830000 0.13919
9840000 0.139191
9850000 0.139186
9860000 0.139187
9870000 0.139188
9880000 0.139184
9890000 0.139195
9900000 0.139189
9910000 0.13918
9920000 0.139186
9930000 0.13918
9940000 0.139168
9950000 0.139161
9960000 0.139167
9970000 0.139156
9980000 0.139152
9990000 0.13915
10000000 0.139144


==> Figures/2DResults/Exterior/Mixed.tex <==
10000 1.19675
20000 0.861699
30000 0.709474
40000 0.620931
50000 0.564256
60000 0.523375
70000 0.490205
80000 0.467341
90000 0.447617
100000 0.432702
110000 0.417411
120000 0.404681
130000 0.393176
140000 0.385328
150000 0.37709
160000 0.368826
170000 0.363039
180000 0.360195
190000 0.354201
200000 0.349271
210000 0.34553
220000 0.340906
230000 0.336648
240000 0.332173
250000 0.327879
260000 0.324853
270000 0.322491
280000 0.319089
290000 0.316929
300000 0.314847
310000 0.312258
320000 0.310058
330000 0.307436
340000 0.305894
350000 0.304326
360000 0.30254
370000 0.301286
380000 0.299799
390000 0.298332
400000 0.296912
410000 0.295668
420000 0.29401
430000 0.293003
440000 0.292284
450000 0.290907
460000 0.289821
470000 0.288863
480000 0.287761
490000 0.286302
500000 0.285557
510000 0.284462
520000 0.283556
530000 0.28275
540000 0.282047
550000 0.281516
560000 0.281012
570000 0.280159
580000 0.279351
590000 0.27905
600000 0.278527
610000 0.277942
620000 0.277038
630000 0.276645
640000 0.275963
650000 0.275528
660000 0.274959
670000 0.274338
680000 0.273509
690000 0.272453
700000 0.272017
710000 0.271787
720000 0.271272
730000 0.27042
740000 0.270086
750000 0.269552
760000 0.268828
770000 0.268275
780000 0.267724
790000 0.267562
800000 0.266916
810000 0.26634
820000 0.266164
830000 0.266015
840000 0.265493
850000 0.265289
860000 0.264644
870000 0.264306
880000 0.263895
890000 0.263627
900000 0.263526
910000 0.26336
920000 0.263187
930000 0.262793
940000 0.262556
950000 0.262313
960000 0.261999
970000 0.261904
980000 0.261546
990000 0.261287
1000000 0.260961
1010000 0.260568
1020000 0.260461
1030000 0.260168
1040000 0.259995
1050000 0.259989
1060000 0.259659
1070000 0.259588
1080000 0.259277
1090000 0.259171
1100000 0.258887
1110000 0.258759
1120000 0.258553
1130000 0.258371
1140000 0.258193
1150000 0.258099
1160000 0.257913
1170000 0.257773
1180000 0.257571
1190000 0.257293
1200000 0.257105
1210000 0.256842
1220000 0.256564
1230000 0.256468
1240000 0.256313
1250000 0.256111
1260000 0.255972
1270000 0.255731
1280000 0.255564
1290000 0.255481
1300000 0.255307
1310000 0.255198
1320000 0.254976
1330000 0.254872
1340000 0.254701
1350000 0.254527
1360000 0.254405
1370000 0.254205
1380000 0.254222
1390000 0.254069
1400000 0.253805
1410000 0.253634
1420000 0.253495
1430000 0.253199
1440000 0.252993
1450000 0.252748
1460000 0.252614
1470000 0.252432
1480000 0.252357
1490000 0.25246
1500000 0.25236
1510000 0.252237
1520000 0.25212
1530000 0.252125
1540000 0.252132
1550000 0.25188
1560000 0.251934
1570000 0.251805
1580000 0.251802
1590000 0.251733
1600000 0.251703
1610000 0.251526
1620000 0.251375
1630000 0.251215
1640000 0.251022
1650000 0.250992
1660000 0.250802
1670000 0.250726
1680000 0.250571
1690000 0.250419
1700000 0.250244
1710000 0.250166
1720000 0.250171
1730000 0.250144
1740000 0.250161
1750000 0.250025
1760000 0.24995
1770000 0.249913
1780000 0.249727
1790000 0.249608
1800000 0.249465
1810000 0.249321
1820000 0.249208
1830000 0.249207
1840000 0.249156
1850000 0.249029
1860000 0.248968
1870000 0.248899
1880000 0.248916
1890000 0.248859
1900000 0.248736
1910000 0.248712
1920000 0.248635
1930000 0.248656
1940000 0.248667
1950000 0.248576
1960000 0.248434
1970000 0.248403
1980000 0.248341
1990000 0.24822
2000000 0.248115
2010000 0.247924
2020000 0.247852
2030000 0.247692
2040000 0.24753
2050000 0.247497
2060000 0.247488
2070000 0.247385
2080000 0.247392
2090000 0.247322
2100000 0.247195
2110000 0.247137
2120000 0.247013
2130000 0.24693
2140000 0.246783
2150000 0.246734
2160000 0.246719
2170000 0.24663
2180000 0.246529
2190000 0.246508
2200000 0.246482
2210000 0.246473
2220000 0.246465
2230000 0.246373
2240000 0.246344
2250000 0.246365
2260000 0.246272
2270000 0.246157
2280000 0.246117
2290000 0.246129
2300000 0.246119
2310000 0.245951
2320000 0.245954
2330000 0.245935
2340000 0.245976
2350000 0.24592
2360000 0.245861
2370000 0.245807
2380000 0.245753
2390000 0.24573
2400000 0.2457
2410000 0.245698
2420000 0.245641
2430000 0.245693
2440000 0.245711
2450000 0.245609
2460000 0.245575
2470000 0.24552
2480000 0.245438
2490000 0.245436
2500000 0.245387
2510000 0.245339
2520000 0.245275
2530000 0.24531
2540000 0.245277
2550000 0.245159
2560000 0.245103
2570000 0.245127
2580000 0.245098
2590000 0.24507
2600000 0.244999
2610000 0.244962
2620000 0.244957
2630000 0.244978
2640000 0.244875
2650000 0.244778
2660000 0.244684
2670000 0.244541
2680000 0.244556
2690000 0.244472
2700000 0.244459
2710000 0.244383
2720000 0.244299
2730000 0.244215
2740000 0.244185
2750000 0.244108
2760000 0.244094
2770000 0.24403
2780000 0.243943
2790000 0.243899
2800000 0.243991
2810000 0.243924
2820000 0.243925
2830000 0.243943
2840000 0.243865
2850000 0.243774
2860000 0.243734
2870000 0.243681
2880000 0.243666
2890000 0.243721
2900000 0.243717
2910000 0.243709
2920000 0.243673
2930000 0.243631
2940000 0.243544
2950000 0.243526
2960000 0.243508
2970000 0.24345
2980000 0.243373
2990000 0.243304
3000000 0.243289
3010000 0.243327
3020000 0.24337
3030000 0.243292
3040000 0.243234
3050000 0.243203
3060000 0.243227
3070000 0.24316
3080000 0.243069
3090000 0.243005
3100000 0.242985
3110000 0.242969
3120000 0.242957
3130000 0.242935
3140000 0.242894
3150000 0.24292
3160000 0.242905
3170000 0.242861
3180000 0.242912
3190000 0.242902
3200000 0.24289
3210000 0.242862
3220000 0.242847
3230000 0.242843
3240000 0.242827
3250000 0.242812
3260000 0.242748
3270000 0.242633
3280000 0.242615
3290000 0.242567
3300000 0.24256
3310000 0.242513
3320000 0.242462
3330000 0.242473
3340000 0.242498
3350000 0.242501
3360000 0.242465
3370000 0.24248
3380000 0.242376
3390000 0.242335
3400000 0.242293
3410000 0.242295
3420000 0.242255
3430000 0.242156
3440000 0.242129
3450000 0.242086
3460000 0.242061
3470000 0.24202
3480000 0.242011
3490000 0.242012
3500000 0.241999
3510000 0.241992
3520000 0.241979
3530000 0.241906
3540000 0.241877
3550000 0.241839
3560000 0.241846
3570000 0.241804
3580000 0.241769
3590000 0.241735
3600000 0.241706
3610000 0.241703
3620000 0.24169
3630000 0.24166
3640000 0.24165
3650000 0.241609
3660000 0.241598
3670000 0.241553
3680000 0.241574
3690000 0.241582
3700000 0.241561
3710000 0.24149
3720000 0.241467
3730000 0.24142
3740000 0.241395
3750000 0.241393
3760000 0.241397
3770000 0.241381
3780000 0.24138
3790000 0.241357
3800000 0.241341
3810000 0.241306
3820000 0.241266
3830000 0.241249
3840000 0.241253
3850000 0.241224
3860000 0.241155
3870000 0.241139
3880000 0.241136
3890000 0.2411
3900000 0.241074
3910000 0.241055
3920000 0.241054
3930000 0.241018
3940000 0.240938
3950000 0.240882
3960000 0.240887
3970000 0.240907
3980000 0.240859
3990000 0.240845
4000000 0.240845
4010000 0.24079
4020000 0.24076
4030000 0.240731
4040000 0.24068
4050000 0.240632
4060000 0.240638
4070000 0.240614
4080000 0.240589
4090000 0.240571
4100000 0.240559
4110000 0.240528
4120000 0.240498
4130000 0.240535
4140000 0.240485
4150000 0.240441
4160000 0.240411
4170000 0.240361
4180000 0.240293
4190000 0.240215
4200000 0.240216
4210000 0.240177
4220000 0.240145
4230000 0.240127
4240000 0.240107
4250000 0.240112
4260000 0.240068
4270000 0.240075
4280000 0.240032
4290000 0.240034
4300000 0.240012
4310000 0.239978
4320000 0.239987
4330000 0.239968
4340000 0.239966
4350000 0.239947
4360000 0.239919
4370000 0.239912
4380000 0.239931
4390000 0.239945
4400000 0.239919
4410000 0.239898
4420000 0.239901
4430000 0.239859
4440000 0.239828
4450000 0.239798
4460000 0.239833
4470000 0.239785
4480000 0.239765
4490000 0.239751
4500000 0.239729
4510000 0.239708
4520000 0.239676
4530000 0.239712
4540000 0.239727
4550000 0.239712
4560000 0.23973
4570000 0.239736
4580000 0.239749
4590000 0.239696
4600000 0.239693
4610000 0.239691
4620000 0.239661
4630000 0.239644
4640000 0.239635
4650000 0.239638
4660000 0.239606
4670000 0.239588
4680000 0.239594
4690000 0.239542
4700000 0.239548
4710000 0.23956
4720000 0.23956
4730000 0.239567
4740000 0.23955
4750000 0.239513
4760000 0.239497
4770000 0.239524
4780000 0.239505
4790000 0.23949
4800000 0.239463
4810000 0.239469
4820000 0.239448
4830000 0.239433
4840000 0.239428
4850000 0.239434
4860000 0.239388
4870000 0.239367
4880000 0.239352
4890000 0.239364
4900000 0.239335
4910000 0.239341
4920000 0.239327
4930000 0.23931
4940000 0.239312
4950000 0.239321
4960000 0.239297
4970000 0.239254
4980000 0.239265
4990000 0.239312
5000000 0.239288
5010000 0.239265
5020000 0.239238
5030000 0.239241
5040000 0.239208
5050000 0.239175
5060000 0.239142
5070000 0.239154
5080000 0.239161
5090000 0.239179
5100000 0.239135
5110000 0.239111
5120000 0.239107
5130000 0.23909
5140000 0.239065
5150000 0.239072
5160000 0.239049
5170000 0.23905
5180000 0.239054
5190000 0.239064
5200000 0.239036
5210000 0.239012
5220000 0.238977
5230000 0.238923
5240000 0.238914
5250000 0.238936
5260000 0.238934
5270000 0.238908
5280000 0.238914
5290000 0.238882
5300000 0.238893
5310000 0.238922
5320000 0.238907
5330000 0.238881
5340000 0.238867
5350000 0.238804
5360000 0.238792
5370000 0.2388
5380000 0.238788
5390000 0.238772
5400000 0.238744
5410000 0.238749
5420000 0.238717
5430000 0.238724
5440000 0.238738
5450000 0.238713
5460000 0.238692
5470000 0.238671
5480000 0.238674
5490000 0.238667
5500000 0.238686
5510000 0.238704
5520000 0.238718
5530000 0.238706
5540000 0.238698
5550000 0.238671
5560000 0.238645
5570000 0.238603
5580000 0.238597
5590000 0.238578
5600000 0.238519
5610000 0.238526
5620000 0.238557
5630000 0.238538
5640000 0.238548
5650000 0.238536
5660000 0.238518
5670000 0.238496
5680000 0.238498
5690000 0.238517
5700000 0.238526
5710000 0.238526
5720000 0.238487
5730000 0.238449
5740000 0.238419
5750000 0.238387
5760000 0.238361
5770000 0.238348
5780000 0.238303
5790000 0.238292
5800000 0.238327
5810000 0.238333
5820000 0.23836
5830000 0.238362
5840000 0.238338
5850000 0.238338
5860000 0.238323
5870000 0.238315
5880000 0.238309
5890000 0.238286
5900000 0.238302
5910000 0.238321
5920000 0.2383
5930000 0.238272
5940000 0.238283
5950000 0.23826
5960000 0.238244
5970000 0.23821
5980000 0.238187
5990000 0.238211
6000000 0.238218
6010000 0.238205
6020000 0.238209
6030000 0.238213
6040000 0.238193
6050000 0.238197
6060000 0.238173
6070000 0.238171
6080000 0.238164
6090000 0.238138
6100000 0.238143
6110000 0.238122
6120000 0.23813
6130000 0.238108
6140000 0.238118
6150000 0.238098
6160000 0.238065
6170000 0.238023
6180000 0.238063
6190000 0.238057
6200000 0.23806
6210000 0.238058
6220000 0.238081
6230000 0.238094
6240000 0.238079
6250000 0.238075
6260000 0.238103
6270000 0.238109
6280000 0.238117
6290000 0.2381
6300000 0.238077
6310000 0.238063
6320000 0.238032
6330000 0.238016
6340000 0.237995
6350000 0.237991
6360000 0.237978
6370000 0.237995
6380000 0.237968
6390000 0.237935
6400000 0.237936
6410000 0.2379
6420000 0.237897
6430000 0.237903
6440000 0.237895
6450000 0.237903
6460000 0.237916
6470000 0.237911
6480000 0.237892
6490000 0.237888
6500000 0.237888
6510000 0.237905
6520000 0.237884
6530000 0.237868
6540000 0.2379
6550000 0.237897
6560000 0.237906
6570000 0.237901
6580000 0.237896
6590000 0.237903
6600000 0.237922
6610000 0.237907
6620000 0.237899
6630000 0.237882
6640000 0.237879
6650000 0.237853
6660000 0.237858
6670000 0.237855
6680000 0.23783
6690000 0.237819
6700000 0.237867
6710000 0.237858
6720000 0.237864
6730000 0.237889
6740000 0.237854
6750000 0.237849
6760000 0.237832
6770000 0.237814
6780000 0.237774
6790000 0.23777
6800000 0.237744
6810000 0.237731
6820000 0.237736
6830000 0.237719
6840000 0.237724
6850000 0.237742
6860000 0.237727
6870000 0.237725
6880000 0.237727
6890000 0.237707
6900000 0.237703
6910000 0.237695
6920000 0.237686
6930000 0.237674
6940000 0.237687
6950000 0.237665
6960000 0.237682
6970000 0.237671
6980000 0.237683
6990000 0.237686
7000000 0.237678
7010000 0.237654
7020000 0.237646
7030000 0.237606
7040000 0.237575
7050000 0.237572
7060000 0.237575
7070000 0.237571
7080000 0.23756
7090000 0.237551
7100000 0.237565
7110000 0.237563
7120000 0.237557
7130000 0.23757
7140000 0.23755
7150000 0.237548
7160000 0.237548
7170000 0.237508
7180000 0.237516
7190000 0.237517
7200000 0.237515
7210000 0.237512
7220000 0.237511
7230000 0.237494
7240000 0.237507
7250000 0.237507
7260000 0.237495
7270000 0.237492
7280000 0.237486
7290000 0.237456
7300000 0.23745
7310000 0.237437
7320000 0.237428
7330000 0.237428
7340000 0.237433
7350000 0.237426
7360000 0.237407
7370000 0.237403
7380000 0.237399
7390000 0.237374
7400000 0.237396
7410000 0.237393
7420000 0.237387
7430000 0.237383
7440000 0.237383
7450000 0.237401
7460000 0.237395
7470000 0.237395
7480000 0.237374
7490000 0.23738
7500000 0.23735
7510000 0.237345
7520000 0.237363
7530000 0.237342
7540000 0.237314
7550000 0.237318
7560000 0.237327
7570000 0.237297
7580000 0.237272
7590000 0.237284
7600000 0.237256
7610000 0.237241
7620000 0.237214
7630000 0.237193
7640000 0.237176
7650000 0.237181
7660000 0.237169
7670000 0.237167
7680000 0.237163
7690000 0.237176
7700000 0.237197
7710000 0.237195
7720000 0.237189
7730000 0.237153
7740000 0.237151
7750000 0.237145
7760000 0.237141
7770000 0.237132
7780000 0.237134
7790000 0.237139
7800000 0.237133
7810000 0.237097
7820000 0.237081
7830000 0.237075
7840000 0.237082
7850000 0.237088
7860000 0.237087
7870000 0.237106
7880000 0.237086
7890000 0.237091
7900000 0.237059
7910000 0.237063
7920000 0.237049
7930000 0.237067
7940000 0.237067
7950000 0.237059
7960000 0.23705
7970000 0.237045
7980000 0.237036
7990000 0.237035
8000000 0.237027
8010000 0.23705
8020000 0.23704
8030000 0.237039
8040000 0.23703
8050000 0.237039
8060000 0.237022
8070000 0.237037
8080000 0.237032
8090000 0.237027
8100000 0.237009
8110000 0.237009
8120000 0.236998
8130000 0.237009
8140000 0.236999
8150000 0.237
8160000 0.237004
8170000 0.237006
8180000 0.237019
8190000 0.237032
8200000 0.237024
8210000 0.237023
8220000 0.237028
8230000 0.237023
8240000 0.237012
8250000 0.237
8260000 0.237016
8270000 0.237015
8280000 0.236996
8290000 0.23699
8300000 0.236975
8310000 0.236984
8320000 0.237008
8330000 0.237008
8340000 0.236978
8350000 0.236969
8360000 0.236982
8370000 0.236994
8380000 0.236991
8390000 0.236981
8400000 0.236997
8410000 0.236984
8420000 0.236961
8430000 0.236957
8440000 0.236958
8450000 0.236963
8460000 0.236968
8470000 0.236965
8480000 0.236935
8490000 0.236926
8500000 0.236915
8510000 0.23692
8520000 0.236922
8530000 0.236907
8540000 0.236904
8550000 0.236929
8560000 0.236915
8570000 0.236908
8580000 0.236912
8590000 0.236898
8600000 0.236879
8610000 0.236881
8620000 0.23689
8630000 0.236876
8640000 0.236831
8650000 0.236835
8660000 0.23682
8670000 0.236822
8680000 0.236835
8690000 0.236826
8700000 0.236824
8710000 0.236814
8720000 0.236791
8730000 0.23677
8740000 0.236739
8750000 0.236739
8760000 0.236733
8770000 0.236722
8780000 0.23671
8790000 0.236727
8800000 0.236716
8810000 0.236687
8820000 0.236661
8830000 0.236676
8840000 0.23668
8850000 0.236661
8860000 0.236652
8870000 0.236676
8880000 0.236677
8890000 0.236663
8900000 0.236664
8910000 0.236659
8920000 0.23664
8930000 0.236631
8940000 0.236619
8950000 0.236614
8960000 0.236604
8970000 0.236586
8980000 0.23658
8990000 0.236584
9000000 0.236577
9010000 0.236564
9020000 0.236573
9030000 0.236571
9040000 0.236566
9050000 0.23659
9060000 0.236601
9070000 0.236599
9080000 0.23659
9090000 0.236576
9100000 0.236569
9110000 0.236565
9120000 0.236571
9130000 0.236564
9140000 0.236563
9150000 0.236561
9160000 0.236544
9170000 0.236551
9180000 0.236563
9190000 0.236583
9200000 0.236588
9210000 0.236604
9220000 0.236606
9230000 0.236615
9240000 0.236615
9250000 0.236612
9260000 0.236647
9270000 0.236627
9280000 0.23662
9290000 0.236623
9300000 0.23661
9310000 0.236623
9320000 0.236607
9330000 0.236615
9340000 0.2366
9350000 0.236599
9360000 0.236587
9370000 0.236575
9380000 0.236555
9390000 0.236537
9400000 0.236519
9410000 0.236529
9420000 0.236546
9430000 0.236542
9440000 0.236543
9450000 0.236532
9460000 0.236529
9470000 0.236519
9480000 0.236513
9490000 0.236516
9500000 0.23652
9510000 0.23652
9520000 0.236509
9530000 0.236485
9540000 0.236479
9550000 0.236484
9560000 0.236487
9570000 0.236503
9580000 0.23651
9590000 0.236489
9600000 0.236464
9610000 0.236448
9620000 0.236439
9630000 0.236441
9640000 0.236435
9650000 0.236442
9660000 0.236454
9670000 0.236442
9680000 0.236423
9690000 0.236429
9700000 0.23643
9710000 0.236437
9720000 0.23642
9730000 0.236421
9740000 0.236408
9750000 0.236411
9760000 0.236407
9770000 0.236397
9780000 0.236395
9790000 0.236399
9800000 0.23639
9810000 0.236396
9820000 0.236399
9830000 0.236402
9840000 0.236398
9850000 0.236405
9860000 0.236419
9870000 0.236431
9880000 0.236428
9890000 0.236446
9900000 0.236429
9910000 0.236429
9920000 0.236419
9930000 0.236426
9940000 0.236439
9950000 0.236442
9960000 0.236441
9970000 0.236428
9980000 0.236422
9990000 0.236439
10000000 0.23643


==> Figures/2DResults/Exterior/NeumannBackward.tex <==
10000 2.40141
20000 1.70193
30000 1.38104
40000 1.20112
50000 1.06435
60000 0.976447
70000 0.903894
80000 0.844218
90000 0.798557
100000 0.756486
110000 0.718416
120000 0.685859
130000 0.658495
140000 0.635983
150000 0.616318
160000 0.598193
170000 0.581288
180000 0.564616
190000 0.550243
200000 0.538851
210000 0.526599
220000 0.513881
230000 0.502514
240000 0.491926
250000 0.481118
260000 0.473685
270000 0.465125
280000 0.457045
290000 0.448065
300000 0.441155
310000 0.433834
320000 0.426498
330000 0.419748
340000 0.414359
350000 0.407958
360000 0.40265
370000 0.397298
380000 0.39234
390000 0.386873
400000 0.382009
410000 0.377025
420000 0.372999
430000 0.368402
440000 0.363545
450000 0.360869
460000 0.356572
470000 0.353132
480000 0.348415
490000 0.345065
500000 0.341995
510000 0.338837
520000 0.335839
530000 0.332664
540000 0.329359
550000 0.326441
560000 0.323753
570000 0.320916
580000 0.318584
590000 0.31563
600000 0.31337
610000 0.310928
620000 0.308666
630000 0.30636
640000 0.304451
650000 0.302175
660000 0.299687
670000 0.297258
680000 0.295703
690000 0.293886
700000 0.291634
710000 0.289902
720000 0.287874
730000 0.28576
740000 0.28433
750000 0.282077
760000 0.280374
770000 0.278505
780000 0.276309
790000 0.274423
800000 0.272752
810000 0.271409
820000 0.269581
830000 0.268141
840000 0.266705
850000 0.264989
860000 0.263128
870000 0.261289
880000 0.2601
890000 0.258532
900000 0.257068
910000 0.255604
920000 0.25442
930000 0.252645
940000 0.251634
950000 0.250401
960000 0.248954
970000 0.247777
980000 0.246402
990000 0.24508
1000000 0.243941
1010000 0.242611
1020000 0.241151
1030000 0.240247
1040000 0.239374
1050000 0.238295
1060000 0.237297
1070000 0.236339
1080000 0.23487
1090000 0.233808
1100000 0.232516
1110000 0.231875
1120000 0.230666
1130000 0.229429
1140000 0.228204
1150000 0.227484
1160000 0.22671
1170000 0.225679
1180000 0.225039
1190000 0.224175
1200000 0.2231
1210000 0.222376
1220000 0.221426
1230000 0.220393
1240000 0.219653
1250000 0.21859
1260000 0.217439
1270000 0.216336
1280000 0.215365
1290000 0.214337
1300000 0.213452
1310000 0.212889
1320000 0.211652
1330000 0.21082
1340000 0.210068
1350000 0.209157
1360000 0.208286
1370000 0.207225
1380000 0.206497
1390000 0.205926
1400000 0.205464
1410000 0.204557
1420000 0.203818
1430000 0.203106
1440000 0.202475
1450000 0.201977
1460000 0.201307
1470000 0.200694
1480000 0.200087
1490000 0.199767
1500000 0.198914
1510000 0.198166
1520000 0.19756
1530000 0.197108
1540000 0.196266
1550000 0.195538
1560000 0.194995
1570000 0.19441
1580000 0.193853
1590000 0.19309
1600000 0.192448
1610000 0.192085
1620000 0.191457
1630000 0.19108
1640000 0.190583
1650000 0.190079
1660000 0.189624
1670000 0.189138
1680000 0.188586
1690000 0.188098
1700000 0.187495
1710000 0.186724
1720000 0.186052
1730000 0.185453
1740000 0.184976
1750000 0.184536
1760000 0.184048
1770000 0.183585
1780000 0.183125
1790000 0.182715
1800000 0.182223
1810000 0.181687
1820000 0.181341
1830000 0.180981
1840000 0.180272
1850000 0.179617
1860000 0.179001
1870000 0.178569
1880000 0.17785
1890000 0.177349
1900000 0.176806
1910000 0.176382
1920000 0.175879
1930000 0.175141
1940000 0.174739
1950000 0.17416
1960000 0.173634
1970000 0.173142
1980000 0.172753
1990000 0.172392
2000000 0.172038
2010000 0.171579
2020000 0.171152
2030000 0.170646
2040000 0.170275
2050000 0.169962
2060000 0.169324
2070000 0.169084
2080000 0.168772
2090000 0.168433
2100000 0.168108
2110000 0.167871
2120000 0.167566
2130000 0.167359
2140000 0.167065
2150000 0.166756
2160000 0.166306
2170000 0.165895
2180000 0.165394
2190000 0.164968
2200000 0.164794
2210000 0.164338
2220000 0.164001
2230000 0.163519
2240000 0.163224
2250000 0.162833
2260000 0.162515
2270000 0.162321
2280000 0.161831
2290000 0.161682
2300000 0.16134
2310000 0.161014
2320000 0.160335
2330000 0.160018
2340000 0.159764
2350000 0.159346
2360000 0.159021
2370000 0.158481
2380000 0.158156
2390000 0.15767
2400000 0.157485
2410000 0.157226
2420000 0.156918
2430000 0.156634
2440000 0.156197
2450000 0.155777
2460000 0.155424
2470000 0.155094
2480000 0.154825
2490000 0.154645
2500000 0.154226
2510000 0.153928
2520000 0.153578
2530000 0.153351
2540000 0.153171
2550000 0.152902
2560000 0.15259
2570000 0.15214
2580000 0.151995
2590000 0.151839
2600000 0.15148
2610000 0.151156
2620000 0.150775
2630000 0.150519
2640000 0.150266
2650000 0.15005
2660000 0.149585
2670000 0.149301
2680000 0.148904
2690000 0.148747
2700000 0.148547
2710000 0.148349
2720000 0.148184
2730000 0.148024
2740000 0.14779
2750000 0.147498
2760000 0.147285
2770000 0.146913
2780000 0.146696
2790000 0.146453
2800000 0.146358
2810000 0.146201
2820000 0.145932
2830000 0.145541
2840000 0.145304
2850000 0.145043
2860000 0.144944
2870000 0.144706
2880000 0.144519
2890000 0.144346
2900000 0.144074
2910000 0.14374
2920000 0.143462
2930000 0.143168
2940000 0.143031
2950000 0.142677
2960000 0.142428
2970000 0.142187
2980000 0.141932
2990000 0.1417
3000000 0.14162
3010000 0.141441
3020000 0.141197
3030000 0.141047
3040000 0.140786
3050000 0.140666
3060000 0.14044
3070000 0.140206
3080000 0.139994
3090000 0.13981
3100000 0.13947
3110000 0.139242
3120000 0.139078
3130000 0.138892
3140000 0.138715
3150000 0.138604
3160000 0.138362
3170000 0.138086
3180000 0.137912
3190000 0.137677
3200000 0.137486
3210000 0.137226
3220000 0.137069
3230000 0.136808
3240000 0.136549
3250000 0.136397
3260000 0.13623
3270000 0.136014
3280000 0.135826
3290000 0.135565
3300000 0.135392
3310000 0.135194
3320000 0.134967
3330000 0.134772
3340000 0.134614
3350000 0.134346
3360000 0.134117
3370000 0.133984
3380000 0.133752
3390000 0.133642
3400000 0.133443
3410000 0.133242
3420000 0.132977
3430000 0.132853
3440000 0.132544
3450000 0.132315
3460000 0.13209
3470000 0.131952
3480000 0.131698
3490000 0.131561
3500000 0.131361
3510000 0.131229
3520000 0.131088
3530000 0.13096
3540000 0.130668
3550000 0.13046
3560000 0.130163
3570000 0.13002
3580000 0.129912
3590000 0.129804
3600000 0.129588
3610000 0.129498
3620000 0.129235
3630000 0.129016
3640000 0.128835
3650000 0.128702
3660000 0.128599
3670000 0.128436
3680000 0.128257
3690000 0.128175
3700000 0.127966
3710000 0.12769
3720000 0.127572
3730000 0.127349
3740000 0.12716
3750000 0.127081
3760000 0.126888
3770000 0.126674
3780000 0.126343
3790000 0.126205
3800000 0.126
3810000 0.125993
3820000 0.125837
3830000 0.125813
3840000 0.125601
3850000 0.125351
3860000 0.125257
3870000 0.12503
3880000 0.12496
3890000 0.124791
3900000 0.124751
3910000 0.124537
3920000 0.124326
3930000 0.124175
3940000 0.124132
3950000 0.123916
3960000 0.123918
3970000 0.123802
3980000 0.123612
3990000 0.123425
4000000 0.123259
4010000 0.123122
4020000 0.123002
4030000 0.122816
4040000 0.122666
4050000 0.122553
4060000 0.122488
4070000 0.122385
4080000 0.122249
4090000 0.122213
4100000 0.12205
4110000 0.121943
4120000 0.121691
4130000 0.121529
4140000 0.121392
4150000 0.1213
4160000 0.121193
4170000 0.121055
4180000 0.120938
4190000 0.120897
4200000 0.120769
4210000 0.120567
4220000 0.120466
4230000 0.120256
4240000 0.120166
4250000 0.120128
4260000 0.119961
4270000 0.119856
4280000 0.119701
4290000 0.119531
4300000 0.119395
4310000 0.119304
4320000 0.119181
4330000 0.118977
4340000 0.118872
4350000 0.118739
4360000 0.118598
4370000 0.11851
4380000 0.118403
4390000 0.118342
4400000 0.118269
4410000 0.118145
4420000 0.118078
4430000 0.117976
4440000 0.117882
4450000 0.117827
4460000 0.117653
4470000 0.117645
4480000 0.117503
4490000 0.117411
4500000 0.117335
4510000 0.117209
4520000 0.11711
4530000 0.116978
4540000 0.116901
4550000 0.116738
4560000 0.11661
4570000 0.116501
4580000 0.116393
4590000 0.116413
4600000 0.116285
4610000 0.1162
4620000 0.116028
4630000 0.115894
4640000 0.115773
4650000 0.115699
4660000 0.115613
4670000 0.115469
4680000 0.11538
4690000 0.115286
4700000 0.115193
4710000 0.115086
4720000 0.114987
4730000 0.114817
4740000 0.114646
4750000 0.114536
4760000 0.11436
4770000 0.114301
4780000 0.114181
4790000 0.113976
4800000 0.113873
4810000 0.113798
4820000 0.11375
4830000 0.113614
4840000 0.113479
4850000 0.113306
4860000 0.113199
4870000 0.113087
4880000 0.112945
4890000 0.112787
4900000 0.11269
4910000 0.112587
4920000 0.112441
4930000 0.112315
4940000 0.11224
4950000 0.112213
4960000 0.112091
4970000 0.111926
4980000 0.111782
4990000 0.111651
5000000 0.111585
5010000 0.11146
5020000 0.111262
5030000 0.111101
5040000 0.110916
5050000 0.11082
5060000 0.110686
5070000 0.110606
5080000 0.110536
5090000 0.110438
5100000 0.110399
5110000 0.110274
5120000 0.110213
5130000 0.110081
5140000 0.109903
5150000 0.109867
5160000 0.109805
5170000 0.109685
5180000 0.109659
5190000 0.109655
5200000 0.109592
5210000 0.109513
5220000 0.109437
5230000 0.109412
5240000 0.109275
5250000 0.109143
5260000 0.109024
5270000 0.108962
5280000 0.108883
5290000 0.108773
5300000 0.108632
5310000 0.108537
5320000 0.108435
5330000 0.108405
5340000 0.108377
5350000 0.108308
5360000 0.108163
5370000 0.10807
5380000 0.107936
5390000 0.10784
5400000 0.107647
5410000 0.107476
5420000 0.107386
5430000 0.107297
5440000 0.107253
5450000 0.107227
5460000 0.107062
5470000 0.106968
5480000 0.106852
5490000 0.106782
5500000 0.106716
5510000 0.106668
5520000 0.10652
5530000 0.106433
5540000 0.106334
5550000 0.106277
5560000 0.106166
5570000 0.10608
5580000 0.106
5590000 0.105943
5600000 0.105892
5610000 0.105735
5620000 0.1056
5630000 0.105467
5640000 0.10539
5650000 0.105316
5660000 0.105226
5670000 0.105127
5680000 0.105032
5690000 0.104948
5700000 0.104873
5710000 0.10473
5720000 0.104654
5730000 0.104495
5740000 0.104346
5750000 0.104196
5760000 0.104071
5770000 0.104014
5780000 0.103974
5790000 0.103859
5800000 0.10366
5810000 0.10373
5820000 0.103662
5830000 0.103605
5840000 0.103584
5850000 0.1035
5860000 0.103419
5870000 0.103285
5880000 0.103282
5890000 0.103175
5900000 0.103111
5910000 0.103041
5920000 0.102951
5930000 0.10286
5940000 0.102856
5950000 0.1028
5960000 0.102686
5970000 0.102588
5980000 0.102417
5990000 0.102326
6000000 0.102236
6010000 0.102158
6020000 0.102105
6030000 0.101968
6040000 0.101851
6050000 0.101699
6060000 0.101683
6070000 0.101658
6080000 0.101586
6090000 0.101442
6100000 0.101356
6110000 0.101297
6120000 0.101206
6130000 0.101206
6140000 0.101139
6150000 0.101085
6160000 0.10105
6170000 0.100974
6180000 0.100828
6190000 0.100764
6200000 0.100711
6210000 0.100595
6220000 0.100502
6230000 0.100448
6240000 0.100342
6250000 0.100206
6260000 0.100119
6270000 0.0999909
6280000 0.099896
6290000 0.0998522
6300000 0.0997798
6310000 0.099674
6320000 0.09956
6330000 0.0994434
6340000 0.0993258
6350000 0.0993308
6360000 0.0993101
6370000 0.0992489
6380000 0.0991021
6390000 0.0990436
6400000 0.0990126
6410000 0.0988485
6420000 0.0987374
6430000 0.0986034
6440000 0.0985419
6450000 0.0984234
6460000 0.0983355
6470000 0.0982968
6480000 0.0982814
6490000 0.0981951
6500000 0.0981211
6510000 0.0980017
6520000 0.0979526
6530000 0.0979438
6540000 0.0978739
6550000 0.0978604
6560000 0.0977958
6570000 0.0977399
6580000 0.0976538
6590000 0.0976534
6600000 0.0975869
6610000 0.0974935
6620000 0.097386
6630000 0.0972299
6640000 0.0972288
6650000 0.0971849
6660000 0.0971044
6670000 0.097065
6680000 0.0969457
6690000 0.0968715
6700000 0.0967811
6710000 0.096739
6720000 0.096606
6730000 0.0965218
6740000 0.0964358
6750000 0.0963674
6760000 0.0963217
6770000 0.0962746
6780000 0.0962201
6790000 0.0961772
6800000 0.0960667
6810000 0.0959969
6820000 0.0959275
6830000 0.0958206
6840000 0.0957153
6850000 0.0955916
6860000 0.0955039
6870000 0.0954508
6880000 0.0954569
6890000 0.0953807
6900000 0.09533
6910000 0.0953162
6920000 0.0952114
6930000 0.0951743
6940000 0.0950777
6950000 0.0949877
6960000 0.09497
6970000 0.0949203
6980000 0.0948965
6990000 0.0947257
7000000 0.0946733
7010000 0.0946402
7020000 0.094534
7030000 0.0944863
7040000 0.0944351
7050000 0.09439
7060000 0.0943164
7070000 0.0942221
7080000 0.0941889
7090000 0.0940968
7100000 0.0940441
7110000 0.0940039
7120000 0.0939426
7130000 0.0939046
7140000 0.0938649
7150000 0.093811
7160000 0.0937284
7170000 0.0936852
7180000 0.0935832
7190000 0.093528
7200000 0.0934623
7210000 0.0933608
7220000 0.093351
7230000 0.0932685
7240000 0.0932192
7250000 0.0931681
7260000 0.0930904
7270000 0.0930193
7280000 0.0929531
7290000 0.0928369
7300000 0.0927657
7310000 0.092725
7320000 0.0926306
7330000 0.0926293
7340000 0.0926093
7350000 0.0925701
7360000 0.0925025
7370000 0.0924295
7380000 0.0923854
7390000 0.0923685
7400000 0.0923331
7410000 0.0922462
7420000 0.0921615
7430000 0.0920245
7440000 0.0919313
7450000 0.0919
7460000 0.0918299
7470000 0.091744
7480000 0.0916901
7490000 0.091692
7500000 0.0916261
7510000 0.0915539
7520000 0.0915107
7530000 0.0914395
7540000 0.0913419
7550000 0.091274
7560000 0.0912103
7570000 0.0911577
7580000 0.0910792
7590000 0.0909661
7600000 0.0909126
7610000 0.0908728
7620000 0.090875
7630000 0.0907898
7640000 0.0907309
7650000 0.0907107
7660000 0.0906301
7670000 0.0905518
7680000 0.0904695
7690000 0.0904303
7700000 0.0903529
7710000 0.0903454
7720000 0.0902905
7730000 0.0902131
7740000 0.090168
7750000 0.0900898
7760000 0.0900663
7770000 0.0900382
7780000 0.0900048
7790000 0.0899156
7800000 0.089832
7810000 0.0897648
7820000 0.0897175
7830000 0.0896398
7840000 0.0895897
7850000 0.0895324
7860000 0.0894836
7870000 0.0894339
7880000 0.0894166
7890000 0.0893979
7900000 0.0893149
7910000 0.0892711
7920000 0.0891928
7930000 0.0891178
7940000 0.0891143
7950000 0.0890519
7960000 0.0889846
7970000 0.0889638
7980000 0.088938
7990000 0.0889272
8000000 0.0888575
8010000 0.0888087
8020000 0.0887459
8030000 0.0886946
8040000 0.0886233
8050000 0.0885667
8060000 0.0885156
8070000 0.0885272
8080000 0.0884573
8090000 0.0883726
8100000 0.0882966
8110000 0.0882068
8120000 0.0881786
8130000 0.0880689
8140000 0.0880042
8150000 0.0879644
8160000 0.087936
8170000 0.0878764
8180000 0.0877533
8190000 0.0877434
8200000 0.087725
8210000 0.0876734
8220000 0.0876299
8230000 0.0876116
8240000 0.0875362
8250000 0.0874765
8260000 0.0874269
8270000 0.0874532
8280000 0.0874549
8290000 0.0874286
8300000 0.0873876
8310000 0.0873179
8320000 0.0872765
8330000 0.0872263
8340000 0.0871599
8350000 0.0871181
8360000 0.0871147
8370000 0.0870612
8380000 0.0870114
8390000 0.0869545
8400000 0.0868784
8410000 0.0868348
8420000 0.0867789
8430000 0.0867551
8440000 0.0867216
8450000 0.0866987
8460000 0.0866985
8470000 0.0866802
8480000 0.0866782
8490000 0.0866828
8500000 0.0866192
8510000 0.0865676
8520000 0.0865138
8530000 0.0864463
8540000 0.0863824
8550000 0.086356
8560000 0.0863379
8570000 0.0862271
8580000 0.0861662
8590000 0.0861729
8600000 0.0861644
8610000 0.0861277
8620000 0.086148
8630000 0.0861426
8640000 0.0860692
8650000 0.0859962
8660000 0.0859594
8670000 0.0858768
8680000 0.0858331
8690000 0.0858207
8700000 0.0857716
8710000 0.0857362
8720000 0.0856587
8730000 0.0855585
8740000 0.0855661
8750000 0.0855233
8760000 0.0854989
8770000 0.0854354
8780000 0.0854067
8790000 0.0853657
8800000 0.0853139
8810000 0.0852332
8820000 0.0851679
8830000 0.0851443
8840000 0.085085
8850000 0.0850386
8860000 0.0850322
8870000 0.0849683
8880000 0.0849196
8890000 0.08491
8900000 0.0848675
8910000 0.0848553
8920000 0.0848132
8930000 0.0847188
8940000 0.084695
8950000 0.0846714
8960000 0.0846166
8970000 0.0845456
8980000 0.0845443
8990000 0.0845018
9000000 0.0844605
9010000 0.0844347
9020000 0.0844273
9030000 0.0844172
9040000 0.0843686
9050000 0.084326
9060000 0.0842768
9070000 0.0842282
9080000 0.084217
9090000 0.0841432
9100000 0.0840764
9110000 0.0840136
9120000 0.084014
9130000 0.0840079
9140000 0.0839775
9150000 0.0839152
9160000 0.0838325
9170000 0.0837643
9180000 0.0837211
9190000 0.0837032
9200000 0.0836509
9210000 0.0835886
9220000 0.0835335
9230000 0.0834685
9240000 0.0833933
9250000 0.0833454
9260000 0.0832823
9270000 0.0832028
9280000 0.0831175
9290000 0.0830602
9300000 0.0830238
9310000 0.0829739
9320000 0.0829212
9330000 0.082874
9340000 0.0828221
9350000 0.0827899
9360000 0.0827658
9370000 0.0827422
9380000 0.0826983
9390000 0.0826854
9400000 0.0826738
9410000 0.0826516
9420000 0.0825901
9430000 0.0825672
9440000 0.0825625
9450000 0.0825387
9460000 0.0825413
9470000 0.0824531
9480000 0.0824298
9490000 0.0823599
9500000 0.0823781
9510000 0.0823282
9520000 0.0823117
9530000 0.0823524
9540000 0.0822891
9550000 0.0822421
9560000 0.0821733
9570000 0.0821469
9580000 0.0820987
9590000 0.0821053
9600000 0.0820709
9610000 0.0820367
9620000 0.0819939
9630000 0.0819381
9640000 0.0819551
9650000 0.0819292
9660000 0.0819063
9670000 0.0818775
9680000 0.081862
9690000 0.0817943
9700000 0.0817562
9710000 0.0817275
9720000 0.0816543
9730000 0.0816231
9740000 0.0815848
9750000 0.0815942
9760000 0.0815568
9770000 0.081521
9780000 0.0814836
9790000 0.0814228
9800000 0.081396
9810000 0.0813799
9820000 0.0812983
9830000 0.0812366
9840000 0.0811846
9850000 0.081144
9860000 0.0811087
9870000 0.0810269
9880000 0.0809752
9890000 0.0810109
9900000 0.0809745
9910000 0.0809209
9920000 0.0809575
9930000 0.0809039
9940000 0.0808077
9950000 0.0807615
9960000 0.0807293
9970000 0.0806846
9980000 0.0806575
9990000 0.0806507
10000000 0.0806435


==> Figures/2DResults/Exterior/NeumannForward.tex <==
10000 1.14043
20000 0.811777
30000 0.669579
40000 0.572862
50000 0.511311
60000 0.467499
70000 0.432095
80000 0.405151
90000 0.382995
100000 0.364247
110000 0.344678
120000 0.331316
130000 0.317905
140000 0.306621
150000 0.295814
160000 0.286139
170000 0.27766
180000 0.270198
190000 0.263197
200000 0.257911
210000 0.253095
220000 0.24746
230000 0.242181
240000 0.237816
250000 0.232628
260000 0.228005
270000 0.223213
280000 0.219513
290000 0.215675
300000 0.211754
310000 0.208409
320000 0.20497
330000 0.201865
340000 0.199043
350000 0.196165
360000 0.193719
370000 0.191213
380000 0.188924
390000 0.186012
400000 0.183511
410000 0.180981
420000 0.178679
430000 0.176202
440000 0.174145
450000 0.171957
460000 0.17029
470000 0.168648
480000 0.166444
490000 0.164482
500000 0.162771
510000 0.160888
520000 0.15957
530000 0.158267
540000 0.157036
550000 0.155712
560000 0.154046
570000 0.152965
580000 0.151738
590000 0.150423
600000 0.148974
610000 0.148288
620000 0.147673
630000 0.146356
640000 0.145236
650000 0.144318
660000 0.143435
670000 0.142344
680000 0.141191
690000 0.140059
700000 0.13935
710000 0.138433
720000 0.137384
730000 0.136678
740000 0.135625
750000 0.13458
760000 0.133751
770000 0.13292
780000 0.132184
790000 0.131431
800000 0.130789
810000 0.129821
820000 0.129247
830000 0.128411
840000 0.127739
850000 0.126971
860000 0.126153
870000 0.125554
880000 0.124959
890000 0.124173
900000 0.123331
910000 0.122862
920000 0.122189
930000 0.121522
940000 0.120884
950000 0.12051
960000 0.120017
970000 0.119176
980000 0.118675
990000 0.118017
1000000 0.117465
1010000 0.116847
1020000 0.116325
1030000 0.115808
1040000 0.115441
1050000 0.115161
1060000 0.114703
1070000 0.114247
1080000 0.113599
1090000 0.113062
1100000 0.112458
1110000 0.112083
1120000 0.11178
1130000 0.111437
1140000 0.111063
1150000 0.110757
1160000 0.110436
1170000 0.110077
1180000 0.109711
1190000 0.109093
1200000 0.108624
1210000 0.108244
1220000 0.107882
1230000 0.107279
1240000 0.106968
1250000 0.106683
1260000 0.10632
1270000 0.105838
1280000 0.105406
1290000 0.104957
1300000 0.104605
1310000 0.104253
1320000 0.103888
1330000 0.103574
1340000 0.103306
1350000 0.102851
1360000 0.102497
1370000 0.10215
1380000 0.101865
1390000 0.101454
1400000 0.101356
1410000 0.100974
1420000 0.100641
1430000 0.100412
1440000 0.10015
1450000 0.0998643
1460000 0.0994109
1470000 0.0993204
1480000 0.0991739
1490000 0.09868
1500000 0.0984989
1510000 0.0981508
1520000 0.0979155
1530000 0.0975787
1540000 0.0973224
1550000 0.0970078
1560000 0.0966945
1570000 0.0963962
1580000 0.0961541
1590000 0.0959214
1600000 0.0956514
1610000 0.0953906
1620000 0.0950047
1630000 0.0948079
1640000 0.0944784
1650000 0.0943157
1660000 0.0941406
1670000 0.0939744
1680000 0.0937337
1690000 0.0934637
1700000 0.093316
1710000 0.0930744
1720000 0.0929028
1730000 0.09275
1740000 0.0925337
1750000 0.0923009
1760000 0.0920219
1770000 0.0917589
1780000 0.0915875
1790000 0.0913116
1800000 0.0911477
1810000 0.0909106
1820000 0.0906895
1830000 0.0904704
1840000 0.0902519
1850000 0.0899858
1860000 0.0897124
1870000 0.0894876
1880000 0.089246
1890000 0.0890354
1900000 0.0887463
1910000 0.0886018
1920000 0.0884461
1930000 0.0883149
1940000 0.0880833
1950000 0.0878684
1960000 0.0876694
1970000 0.0875171
1980000 0.087292
1990000 0.0871059
2000000 0.0869923
2010000 0.0868463
2020000 0.0866838
2030000 0.0865169
2040000 0.0864504
2050000 0.0862295
2060000 0.0860372
2070000 0.0857147
2080000 0.0854762
2090000 0.0852216
2100000 0.0850333
2110000 0.0847878
2120000 0.08461
2130000 0.0844259
2140000 0.0843445
2150000 0.0841849
2160000 0.084107
2170000 0.0839485
2180000 0.0837693
2190000 0.0836301
2200000 0.083457
2210000 0.0832683
2220000 0.0831657
2230000 0.0829774
2240000 0.0827436
2250000 0.0826231
2260000 0.0824637
2270000 0.0822852
2280000 0.0820389
2290000 0.0818955
2300000 0.0816959
2310000 0.081483
2320000 0.0813615
2330000 0.0812767
2340000 0.0811166
2350000 0.0811023
2360000 0.0810355
2370000 0.0808901
2380000 0.0807264
2390000 0.0805711
2400000 0.0804076
2410000 0.0801472
2420000 0.0801148
2430000 0.0799958
2440000 0.079863
2450000 0.079733
2460000 0.0796453
2470000 0.0794584
2480000 0.079363
2490000 0.0791713
2500000 0.0791179
2510000 0.0789917
2520000 0.0788499
2530000 0.0787541
2540000 0.0785238
2550000 0.0783376
2560000 0.0781967
2570000 0.0779675
2580000 0.0779211
2590000 0.0776792
2600000 0.0775355
2610000 0.077359
2620000 0.0772044
2630000 0.0771027
2640000 0.0770205
2650000 0.0768146
2660000 0.0766984
2670000 0.0764703
2680000 0.0762718
2690000 0.076227
2700000 0.0761453
2710000 0.0760138
2720000 0.0758645
2730000 0.075748
2740000 0.0756605
2750000 0.075437
2760000 0.0752787
2770000 0.0751952
2780000 0.075094
2790000 0.0748713
2800000 0.0747707
2810000 0.074669
2820000 0.074541
2830000 0.0744887
2840000 0.0743295
2850000 0.0742358
2860000 0.0741786
2870000 0.0740264
2880000 0.0738559
2890000 0.073773
2900000 0.0736775
2910000 0.0735902
2920000 0.0733787
2930000 0.07324
2940000 0.0731432
2950000 0.0729771
2960000 0.0728412
2970000 0.0727106
2980000 0.0726386
2990000 0.0725426
3000000 0.0724596
3010000 0.0723804
3020000 0.0722785
3030000 0.0722633
3040000 0.0722124
3050000 0.0721214
3060000 0.0719522
3070000 0.0718569
3080000 0.0717858
3090000 0.0716058
3100000 0.0715504
3110000 0.0714899
3120000 0.0713943
3130000 0.0713408
3140000 0.0712357
3150000 0.0711499
3160000 0.0710717
3170000 0.0709549
3180000 0.0708836
3190000 0.0707414
3200000 0.0706457
3210000 0.0705828
3220000 0.0704758
3230000 0.0703361
3240000 0.0703411
3250000 0.0702281
3260000 0.0701912
3270000 0.0701077
3280000 0.0700593
3290000 0.0699857
3300000 0.0698791
3310000 0.0697694
3320000 0.0696606
3330000 0.0696396
3340000 0.0695446
3350000 0.069401
3360000 0.0693496
3370000 0.0692348
3380000 0.0692049
3390000 0.0690833
3400000 0.0689514
3410000 0.0688609
3420000 0.0687238
3430000 0.0685925
3440000 0.0685627
3450000 0.0685598
3460000 0.0684565
3470000 0.0684025
3480000 0.0683684
3490000 0.0683149
3500000 0.068204
3510000 0.0681245
3520000 0.0680356
3530000 0.0678741
3540000 0.0678201
3550000 0.0677599
3560000 0.0676916
3570000 0.0675916
3580000 0.0675433
3590000 0.0674255
3600000 0.067367
3610000 0.0672799
3620000 0.0672846
3630000 0.0671963
3640000 0.0671425
3650000 0.0671071
3660000 0.0670479
3670000 0.0670205
3680000 0.066907
3690000 0.0668278
3700000 0.066768
3710000 0.0667139
3720000 0.0666752
3730000 0.0666045
3740000 0.066491
3750000 0.0664276
3760000 0.0663822
3770000 0.0663827
3780000 0.0663114
3790000 0.0662213
3800000 0.0661548
3810000 0.0661039
3820000 0.0659412
3830000 0.0658536
3840000 0.0658049
3850000 0.0657966
3860000 0.065728
3870000 0.0656133
3880000 0.065515
3890000 0.0654497
3900000 0.0653837
3910000 0.0653289
3920000 0.065275
3930000 0.0651715
3940000 0.0650683
3950000 0.065059
3960000 0.0650354
3970000 0.0649152
3980000 0.0648842
3990000 0.0647881
4000000 0.0647259
4010000 0.0646407
4020000 0.0645864
4030000 0.0644708
4040000 0.0643781
4050000 0.0643133
4060000 0.0642618
4070000 0.0642227
4080000 0.0641331
4090000 0.0640654
4100000 0.0640293
4110000 0.0640265
4120000 0.0639579
4130000 0.0638679
4140000 0.0638086
4150000 0.0637278
4160000 0.0636508
4170000 0.0635428
4180000 0.0634224
4190000 0.0633577
4200000 0.0633227
4210000 0.0633036
4220000 0.0632756
4230000 0.0632115
4240000 0.0631689
4250000 0.063072
4260000 0.0630589
4270000 0.0629697
4280000 0.0628767
4290000 0.062798
4300000 0.0626835
4310000 0.0626658
4320000 0.0626567
4330000 0.0626155
4340000 0.0625853
4350000 0.0625548
4360000 0.0625026
4370000 0.0624159
4380000 0.0623521
4390000 0.0623489
4400000 0.0623064
4410000 0.062212
4420000 0.0622228
4430000 0.062156
4440000 0.0621149
4450000 0.062039
4460000 0.0619758
4470000 0.0618989
4480000 0.0618399
4490000 0.0617918
4500000 0.0617043
4510000 0.0616196
4520000 0.0615772
4530000 0.0615611
4540000 0.0615117
4550000 0.061389
4560000 0.0613375
4570000 0.0613352
4580000 0.0613162
4590000 0.0612517
4600000 0.0612151
4610000 0.0611851
4620000 0.0610977
4630000 0.0610797
4640000 0.0610582
4650000 0.0610355
4660000 0.0609385
4670000 0.0608978
4680000 0.0609089
4690000 0.0608686
4700000 0.060813
4710000 0.0607679
4720000 0.0606889
4730000 0.0606472
4740000 0.0606423
4750000 0.0605646
4760000 0.0605757
4770000 0.0605024
4780000 0.0604753
4790000 0.0604951
4800000 0.0604325
4810000 0.0603963
4820000 0.0603816
4830000 0.0603111
4840000 0.060266
4850000 0.0602973
4860000 0.0602833
4870000 0.0602025
4880000 0.0601941
4890000 0.0601848
4900000 0.0601433
4910000 0.0601251
4920000 0.0600771
4930000 0.0600538
4940000 0.0600696
4950000 0.0599703
4960000 0.0599292
4970000 0.0598643
4980000 0.0597628
4990000 0.0597319
5000000 0.0596636
5010000 0.0596543
5020000 0.0595997
5030000 0.0595993
5040000 0.0595685
5050000 0.0595429
5060000 0.0594917
5070000 0.0594868
5080000 0.0594281
5090000 0.0594087
5100000 0.0593704
5110000 0.0592652
5120000 0.0592361
5130000 0.0592011
5140000 0.0591465
5150000 0.0591232
5160000 0.0590798
5170000 0.0590408
5180000 0.0589758
5190000 0.0589712
5200000 0.0589422
5210000 0.058901
5220000 0.0588679
5230000 0.0587634
5240000 0.0587375
5250000 0.0587365
5260000 0.0586808
5270000 0.0586681
5280000 0.0586448
5290000 0.0586093
5300000 0.0586188
5310000 0.058575
5320000 0.0585301
5330000 0.0585016
5340000 0.0584575
5350000 0.0584071
5360000 0.0583911
5370000 0.058343
5380000 0.0583243
5390000 0.058268
5400000 0.0582027
5410000 0.0581554
5420000 0.0581397
5430000 0.0580943
5440000 0.0580821
5450000 0.0580749
5460000 0.0580413
5470000 0.0579996
5480000 0.0579751
5490000 0.057959
5500000 0.0579089
5510000 0.0578566
5520000 0.0578695
5530000 0.0578274
5540000 0.0577807
5550000 0.0577287
5560000 0.057688
5570000 0.0576223
5580000 0.0576006
5590000 0.0576066
5600000 0.0575661
5610000 0.0575354
5620000 0.0575297
5630000 0.0574674
5640000 0.057396
5650000 0.0573499
5660000 0.0573113
5670000 0.0573015
5680000 0.0572564
5690000 0.0572174
5700000 0.0571739
5710000 0.0571196
5720000 0.0570806
5730000 0.0570492
5740000 0.057044
5750000 0.0570107
5760000 0.0569968
5770000 0.0569704
5780000 0.0569508
5790000 0.0569086
5800000 0.056844
5810000 0.0568407
5820000 0.0567992
5830000 0.0567472
5840000 0.0566994
5850000 0.0566676
5860000 0.056682
5870000 0.0566377
5880000 0.056598
5890000 0.0565594
5900000 0.0564865
5910000 0.0564543
5920000 0.0564128
5930000 0.0564001
5940000 0.0563633
5950000 0.0562959
5960000 0.0562759
5970000 0.0562565
5980000 0.0561857
5990000 0.0561424
6000000 0.0560601
6010000 0.0560543
6020000 0.056013
6030000 0.0559811
6040000 0.0559519
6050000 0.0559307
6060000 0.055884
6070000 0.055857
6080000 0.0558489
6090000 0.0558201
6100000 0.0557909
6110000 0.0557199
6120000 0.0557224
6130000 0.0556642
6140000 0.0556218
6150000 0.0555875
6160000 0.0555418
6170000 0.0554784
6180000 0.0554224
6190000 0.055404
6200000 0.0553938
6210000 0.0553985
6220000 0.0553638
6230000 0.0553462
6240000 0.055309
6250000 0.0552695
6260000 0.0552665
6270000 0.055205
6280000 0.0551453
6290000 0.0551536
6300000 0.0551219
6310000 0.0550688
6320000 0.0550534
6330000 0.0550085
6340000 0.0549748
6350000 0.0549381
6360000 0.05492
6370000 0.0548839
6380000 0.0548423
6390000 0.054797
6400000 0.0547642
6410000 0.0547246
6420000 0.0547281
6430000 0.054739
6440000 0.0546819
6450000 0.0546545
6460000 0.0546102
6470000 0.0545753
6480000 0.054528
6490000 0.0545191
6500000 0.054492
6510000 0.0544539
6520000 0.0544401
6530000 0.0544018
6540000 0.0543943
6550000 0.0543783
6560000 0.0543506
6570000 0.0543133
6580000 0.0542655
6590000 0.0542386
6600000 0.0542188
6610000 0.0541811
6620000 0.0541908
6630000 0.0541716
6640000 0.0541261
6650000 0.0540848
6660000 0.0540117
6670000 0.0539785
6680000 0.0539496
6690000 0.0539583
6700000 0.0539244
6710000 0.0538852
6720000 0.0538549
6730000 0.0538084
6740000 0.0537861
6750000 0.0537635
6760000 0.0537556
6770000 0.0537436
6780000 0.053704
6790000 0.0536847
6800000 0.0536485
6810000 0.0536624
6820000 0.0535995
6830000 0.0536069
6840000 0.0535912
6850000 0.0535794
6860000 0.0535523
6870000 0.0535187
6880000 0.0535205
6890000 0.0535052
6900000 0.053503
6910000 0.0534774
6920000 0.0534532
6930000 0.0534085
6940000 0.053388
6950000 0.0533678
6960000 0.0533427
6970000 0.0533326
6980000 0.0533454
6990000 0.0533022
7000000 0.0532955
7010000 0.0532809
7020000 0.0532801
7030000 0.0532486
7040000 0.0532068
7050000 0.0531876
7060000 0.0531675
7070000 0.0531263
7080000 0.0531205
7090000 0.0531076
7100000 0.0530467
7110000 0.0530293
7120000 0.052971
7130000 0.0529864
7140000 0.0529991
7150000 0.0529847
7160000 0.0529836
7170000 0.0529684
7180000 0.0529495
7190000 0.0529159
7200000 0.0529022
7210000 0.0528871
7220000 0.0528959
7230000 0.0528662
7240000 0.0528392
7250000 0.0527834
7260000 0.0527471
7270000 0.0527032
7280000 0.0526946
7290000 0.0526586
7300000 0.0526411
7310000 0.0525994
7320000 0.0525626
7330000 0.052544
7340000 0.0525267
7350000 0.0525084
7360000 0.0525103
7370000 0.05251
7380000 0.0524632
7390000 0.0524479
7400000 0.0524097
7410000 0.0523361
7420000 0.0523186
7430000 0.0522814
7440000 0.0522448
7450000 0.0522077
7460000 0.0521563
7470000 0.0521276
7480000 0.0521176
7490000 0.0520866
7500000 0.0520495
7510000 0.0520218
7520000 0.0519936
7530000 0.0519969
7540000 0.0519864
7550000 0.0519446
7560000 0.0519391
7570000 0.0518849
7580000 0.0518416
7590000 0.0518189
7600000 0.0518022
7610000 0.051797
7620000 0.0517738
7630000 0.051752
7640000 0.0516933
7650000 0.0516511
7660000 0.0516354
7670000 0.0516321
7680000 0.0515989
7690000 0.0515738
7700000 0.0515517
7710000 0.0515475
7720000 0.0515392
7730000 0.0515085
7740000 0.0515006
7750000 0.0514442
7760000 0.0514003
7770000 0.0513862
7780000 0.0513837
7790000 0.0513637
7800000 0.0513203
7810000 0.0513089
7820000 0.0512553
7830000 0.0512591
7840000 0.0512153
7850000 0.05121
7860000 0.0512081
7870000 0.0512003
7880000 0.0511692
7890000 0.0511476
7900000 0.0511282
7910000 0.0511226
7920000 0.0511079
7930000 0.0510838
7940000 0.0510838
7950000 0.0510488
7960000 0.0510563
7970000 0.0510335
7980000 0.0509993
7990000 0.0509764
8000000 0.0509598
8010000 0.0509462
8020000 0.050895
8030000 0.0508561
8040000 0.0508317
8050000 0.050773
8060000 0.0507679
8070000 0.0507737
8080000 0.050742
8090000 0.0507288
8100000 0.050698
8110000 0.0506881
8120000 0.0506765
8130000 0.0506897
8140000 0.0506671
8150000 0.0506302
8160000 0.0505918
8170000 0.05059
8180000 0.0505769
8190000 0.0505476
8200000 0.0505646
8210000 0.0505467
8220000 0.0505254
8230000 0.0505071
8240000 0.0505044
8250000 0.0504931
8260000 0.050475
8270000 0.0504351
8280000 0.0504087
8290000 0.0503967
8300000 0.0503811
8310000 0.0503647
8320000 0.0503438
8330000 0.0503577
8340000 0.0503305
8350000 0.050278
8360000 0.0502546
8370000 0.0502543
8380000 0.0502279
8390000 0.0502121
8400000 0.05021
8410000 0.0502041
8420000 0.0501761
8430000 0.0501686
8440000 0.0501602
8450000 0.0501236
8460000 0.0501274
8470000 0.0501132
8480000 0.0501063
8490000 0.0501068
8500000 0.0501006
8510000 0.0500894
8520000 0.0500802
8530000 0.0500417
8540000 0.0500193
8550000 0.0499946
8560000 0.0499798
8570000 0.0499522
8580000 0.0499478
8590000 0.049951
8600000 0.0499232
8610000 0.0499092
8620000 0.0498743
8630000 0.049912
8640000 0.0498905
8650000 0.0499004
8660000 0.0498575
8670000 0.0498613
8680000 0.0498578
8690000 0.0498164
8700000 0.0497768
8710000 0.0497448
8720000 0.0497299
8730000 0.049732
8740000 0.0497349
8750000 0.0496975
8760000 0.0496804
8770000 0.0496549
8780000 0.0496248
8790000 0.0496014
8800000 0.0495964
8810000 0.0495694
8820000 0.0495545
8830000 0.0495408
8840000 0.0495201
8850000 0.0495011
8860000 0.0494825
8870000 0.049487
8880000 0.0494519
8890000 0.0494179
8900000 0.0494026
8910000 0.0493689
8920000 0.0493611
8930000 0.0493455
8940000 0.0493377
8950000 0.0493104
8960000 0.0492906
8970000 0.0492889
8980000 0.0492689
8990000 0.049272
9000000 0.0492568
9010000 0.0492485
9020000 0.0492257
9030000 0.0492211
9040000 0.049225
9050000 0.0492269
9060000 0.0492226
9070000 0.0491847
9080000 0.0491679
9090000 0.0491741
9100000 0.0491446
9110000 0.0491311
9120000 0.0491191
9130000 0.0491111
9140000 0.0490936
9150000 0.0490778
9160000 0.0491126
9170000 0.0490958
9180000 0.0490729
9190000 0.0490572
9200000 0.0490554
9210000 0.0490424
9220000 0.0490109
9230000 0.0489781
9240000 0.0489457
9250000 0.0489383
9260000 0.048887
9270000 0.0488655
9280000 0.0488664
9290000 0.0488626
9300000 0.0488497
9310000 0.0488273
9320000 0.048823
9330000 0.0488205
9340000 0.0487847
9350000 0.0487717
9360000 0.0487266
9370000 0.0486967
9380000 0.0486742
9390000 0.0486485
9400000 0.0486236
9410000 0.048623
9420000 0.0485858
9430000 0.0485604
9440000 0.0485172
9450000 0.048504
9460000 0.0484709
9470000 0.048467
9480000 0.0484605
9490000 0.048438
9500000 0.0484048
9510000 0.0483741
9520000 0.0483533
9530000 0.0483416
9540000 0.0483072
9550000 0.0482762
9560000 0.0482579
9570000 0.0482256
9580000 0.0481956
9590000 0.048182
9600000 0.0481706
9610000 0.0481322
9620000 0.0481164
9630000 0.0481081
9640000 0.0480887
9650000 0.0480963
9660000 0.0480842
9670000 0.0480675
9680000 0.0480432
9690000 0.0480358
9700000 0.0480097
9710000 0.0479782
9720000 0.0479537
9730000 0.0479383
9740000 0.0479326
9750000 0.0479185
9760000 0.047949
9770000 0.0479679
9780000 0.0479379
9790000 0.0479356
9800000 0.0479181
9810000 0.0479184
9820000 0.0479102
9830000 0.0479058
9840000 0.0478846
9850000 0.0478773
9860000 0.0478674
9870000 0.0478364
9880000 0.047819
9890000 0.0478203
9900000 0.0478089
9910000 0.0478025
9920000 0.0477795
9930000 0.0477892
9940000 0.0477724
9950000 0.0477588
9960000 0.0477585
9970000 0.0477336
9980000 0.0477226
9990000 0.0476875
10000000 0.0476621


==> Figures/2DResults/Exterior/Robin.tex <==
10000 1.04375
20000 0.759434
30000 0.61819
40000 0.541303
50000 0.492485
60000 0.445541
70000 0.414439
80000 0.389311
90000 0.368866
100000 0.350772
110000 0.335597
120000 0.324633
130000 0.312599
140000 0.304114
150000 0.2941
160000 0.285029
170000 0.278455
180000 0.270236
190000 0.264138
200000 0.259585
210000 0.253851
220000 0.248521
230000 0.244034
240000 0.239942
250000 0.235808
260000 0.231903
270000 0.228373
280000 0.225
290000 0.221301
300000 0.218123
310000 0.214612
320000 0.218799
330000 0.215466
340000 0.212431
350000 0.210852
360000 0.210419
370000 0.207234
380000 0.204706
390000 0.202086
400000 0.199585
410000 0.196975
420000 0.194933
430000 0.193044
440000 0.191007
450000 0.18903
460000 0.186888
470000 0.185136
480000 0.184355
490000 0.182504
500000 0.180754
510000 0.179708
520000 0.178411
530000 0.177037
540000 0.175956
550000 0.174696
560000 0.172864
570000 0.17166
580000 0.170607
590000 0.169173
600000 0.167959
610000 0.166991
620000 0.165786
630000 0.164943
640000 0.163887
650000 0.162495
660000 0.161376
670000 0.160415
680000 0.159281
690000 0.15902
700000 0.158251
710000 0.157649
720000 0.156905
730000 0.15589
740000 0.154891
750000 0.154252
760000 0.153378
770000 0.152584
780000 0.152031
790000 0.151224
800000 0.150461
810000 0.149903
820000 0.149315
830000 0.148599
840000 0.148037
850000 0.147836
860000 0.147437
870000 0.147275
880000 0.146545
890000 0.145936
900000 0.145428
910000 0.144643
920000 0.14402
930000 0.143788
940000 0.143829
950000 0.14322
960000 0.143054
970000 0.142613
980000 0.142044
990000 0.141447
1000000 0.140961
1010000 0.140381
1020000 0.13994
1030000 0.139396
1040000 0.139069
1050000 0.138571
1060000 0.138097
1070000 0.137629
1080000 0.13719
1090000 0.136972
1100000 0.136507
1110000 0.136193
1120000 0.135821
1130000 0.13563
1140000 0.135187
1150000 0.134675
1160000 0.134296
1170000 0.133835
1180000 0.133443
1190000 0.133191
1200000 0.132876
1210000 0.132535
1220000 0.132159
1230000 0.131786
1240000 0.131455
1250000 0.131083
1260000 0.130707
1270000 0.130523
1280000 0.13029
1290000 0.130027
1300000 0.129705
1310000 0.129282
1320000 0.128926
1330000 0.12844
1340000 0.128125
1350000 0.127831
1360000 0.127591
1370000 0.127256
1380000 0.126973
1390000 0.126668
1400000 0.126396
1410000 0.126136
1420000 0.125661
1430000 0.125392
1440000 0.125059
1450000 0.125186
1460000 0.124882
1470000 0.124948
1480000 0.124716
1490000 0.124478
1500000 0.124335
1510000 0.124037
1520000 0.123835
1530000 0.123573
1540000 0.123338
1550000 0.123045
1560000 0.122824
1570000 0.12251
1580000 0.122379
1590000 0.122223
1600000 0.122048
1610000 0.121747
1620000 0.121523
1630000 0.121288
1640000 0.121006
1650000 0.12066
1660000 0.120414
1670000 0.120273
1680000 0.120022
1690000 0.11975
1700000 0.119602
1710000 0.119506
1720000 0.119314
1730000 0.119135
1740000 0.119244
1750000 0.119105
1760000 0.118907
1770000 0.118783
1780000 0.118733
1790000 0.118561
1800000 0.118443
1810000 0.118196
1820000 0.11803
1830000 0.117884
1840000 0.117928
1850000 0.117732
1860000 0.117516
1870000 0.117373
1880000 0.117239
1890000 0.117072
1900000 0.116861
1910000 0.116689
1920000 0.116563
1930000 0.1164
1940000 0.116235
1950000 0.116039
1960000 0.115918
1970000 0.115702
1980000 0.115448
1990000 0.115242
2000000 0.115204
2010000 0.115161
2020000 0.114853
2030000 0.114738
2040000 0.114669
2050000 0.114455
2060000 0.114258
2070000 0.114086
2080000 0.113843
2090000 0.113684
2100000 0.113527
2110000 0.113211
2120000 0.113029
2130000 0.112859
2140000 0.11263
2150000 0.112417
2160000 0.112296
2170000 0.112322
2180000 0.112143
2190000 0.112041
2200000 0.111982
2210000 0.111862
2220000 0.111682
2230000 0.111546
2240000 0.112832
2250000 0.112663
2260000 0.112542
2270000 0.112395
2280000 0.112166
2290000 0.112116
2300000 0.112209
2310000 0.112102
2320000 0.111907
2330000 0.111877
2340000 0.111848
2350000 0.111651
2360000 0.111402
2370000 0.111256
2380000 0.111145
2390000 0.11104
2400000 0.110909
2410000 0.110847
2420000 0.110643
2430000 0.110585
2440000 0.110623
2450000 0.110568
2460000 0.110645
2470000 0.110546
2480000 0.110476
2490000 0.110412
2500000 0.110325
2510000 0.110201
2520000 0.110087
2530000 0.109953
2540000 0.109868
2550000 0.109742
2560000 0.109639
2570000 0.109447
2580000 0.109286
2590000 0.109187
2600000 0.109313
2610000 0.109129
2620000 0.109003
2630000 0.108983
2640000 0.108872
2650000 0.108746
2660000 0.108569
2670000 0.108475
2680000 0.108336
2690000 0.108221
2700000 0.108126
2710000 0.108004
2720000 0.107928
2730000 0.107807
2740000 0.107709
2750000 0.107608
2760000 0.107471
2770000 0.107359
2780000 0.107221
2790000 0.107128
2800000 0.107124
2810000 0.10704
2820000 0.106958
2830000 0.106986
2840000 0.106922
2850000 0.106817
2860000 0.107055
2870000 0.106952
2880000 0.106869
2890000 0.106747
2900000 0.106997
2910000 0.106893
2920000 0.10673
2930000 0.106598
2940000 0.1066
2950000 0.106481
2960000 0.106349
2970000 0.106293
2980000 0.106255
2990000 0.106188
3000000 0.106105
3010000 0.105999
3020000 0.10593
3030000 0.105921
3040000 0.105867
3050000 0.105765
3060000 0.105686
3070000 0.105635
3080000 0.105596
3090000 0.105532
3100000 0.105443
3110000 0.105374
3120000 0.10534
3130000 0.105242
3140000 0.105153
3150000 0.105105
3160000 0.105088
3170000 0.10492
3180000 0.1049
3190000 0.104819
3200000 0.104756
3210000 0.104653
3220000 0.104558
3230000 0.104511
3240000 0.1044
3250000 0.104325
3260000 0.104269
3270000 0.104169
3280000 0.104159
3290000 0.10414
3300000 0.104069
3310000 0.103959
3320000 0.103903
3330000 0.103832
3340000 0.103747
3350000 0.103646
3360000 0.103562
3370000 0.103511
3380000 0.103398
3390000 0.10334
3400000 0.103301
3410000 0.103244
3420000 0.103212
3430000 0.103123
3440000 0.103049
3450000 0.103144
3460000 0.103091
3470000 0.1031
3480000 0.103019
3490000 0.10298
3500000 0.102986
3510000 0.102927
3520000 0.102878
3530000 0.102792
3540000 0.102708
3550000 0.102634
3560000 0.102508
3570000 0.102428
3580000 0.102658
3590000 0.102636
3600000 0.102557
3610000 0.102477
3620000 0.102432
3630000 0.102395
3640000 0.102292
3650000 0.102249
3660000 0.102165
3670000 0.102164
3680000 0.102047
3690000 0.102021
3700000 0.101978
3710000 0.101928
3720000 0.101906
3730000 0.101803
3740000 0.101739
3750000 0.101729
3760000 0.101639
3770000 0.101527
3780000 0.101509
3790000 0.101585
3800000 0.101491
3810000 0.101428
3820000 0.101355
3830000 0.101304
3840000 0.101281
3850000 0.101212
3860000 0.101183
3870000 0.101153
3880000 0.101139
3890000 0.101152
3900000 0.101095
3910000 0.10101
3920000 0.100994
3930000 0.100938
3940000 0.100829
3950000 0.100783
3960000 0.1007
3970000 0.100673
3980000 0.100677
3990000 0.100645
4000000 0.100625
4010000 0.100566
4020000 0.100484
4030000 0.100428
4040000 0.100384
4050000 0.100326
4060000 0.100282
4070000 0.100247
4080000 0.100182
4090000 0.100149
4100000 0.100139
4110000 0.100109
4120000 0.100042
4130000 0.0999723
4140000 0.0999016
4150000 0.0998161
4160000 0.0997931
4170000 0.0997423
4180000 0.0996893
4190000 0.0996456
4200000 0.0995831
4210000 0.0996118
4220000 0.0995334
4230000 0.0995291
4240000 0.0994885
4250000 0.0994122
4260000 0.099378
4270000 0.0993556
4280000 0.0993269
4290000 0.0992807
4300000 0.0992109
4310000 0.0991636
4320000 0.0991497
4330000 0.0991336
4340000 0.099115
4350000 0.0990608
4360000 0.0990027
4370000 0.098926
4380000 0.0988941
4390000 0.0988663
4400000 0.0987691
4410000 0.0987654
4420000 0.0987402
4430000 0.0986825
4440000 0.098669
4450000 0.0986187
4460000 0.0988949
4470000 0.0988745
4480000 0.0988134
4490000 0.0987996
4500000 0.0987803
4510000 0.0987399
4520000 0.0986551
4530000 0.0986451
4540000 0.0986124
4550000 0.0985527
4560000 0.0985079
4570000 0.0984981
4580000 0.0984671
4590000 0.0984348
4600000 0.0985772
4610000 0.0985566
4620000 0.0985186
4630000 0.0984709
4640000 0.0984223
4650000 0.0983641
4660000 0.0983692
4670000 0.0983364
4680000 0.0982753
4690000 0.0982157
4700000 0.0981709
4710000 0.0981224
4720000 0.0980478
4730000 0.0980357
4740000 0.0979795
4750000 0.0979806
4760000 0.0979519
4770000 0.0979298
4780000 0.0978804
4790000 0.0977628
4800000 0.0977369
4810000 0.0977333
4820000 0.0978586
4830000 0.0977936
4840000 0.0977511
4850000 0.0977316
4860000 0.0976863
4870000 0.0976155
4880000 0.0976007
4890000 0.0975505
4900000 0.0975996
4910000 0.0975929
4920000 0.0975248
4930000 0.0974839
4940000 0.0974794
4950000 0.0974254
4960000 0.0973967
4970000 0.0973577
4980000 0.097293
4990000 0.0972558
5000000 0.0972051
5010000 0.0972229
5020000 0.0971123
5030000 0.0970788
5040000 0.0970283
5050000 0.0969875
5060000 0.0969586
5070000 0.0969292
5080000 0.0970314
5090000 0.0970063
5100000 0.0970065
5110000 0.0969341
5120000 0.0968895
5130000 0.0968678
5140000 0.0968384
5150000 0.0967925
5160000 0.0967797
5170000 0.096765
5180000 0.0967355
5190000 0.0967155
5200000 0.0967079
5210000 0.096674
5220000 0.0966092
5230000 0.0965664
5240000 0.0965467
5250000 0.096499
5260000 0.0964764
5270000 0.0964108
5280000 0.0963601
5290000 0.0963391
5300000 0.0963392
5310000 0.0963079
5320000 0.0962864
5330000 0.0962753
5340000 0.0962573
5350000 0.0962136
5360000 0.0961877
5370000 0.0961332
5380000 0.0961382
5390000 0.0960938
5400000 0.0960199
5410000 0.0960376
5420000 0.0960365
5430000 0.0959853
5440000 0.0959478
5450000 0.0959497
5460000 0.0959972
5470000 0.0960087
5480000 0.0960095
5490000 0.0959774
5500000 0.095958
5510000 0.095912
5520000 0.0958844
5530000 0.0958546
5540000 0.0958299
5550000 0.0958061
5560000 0.0957717
5570000 0.0957961
5580000 0.0957527
5590000 0.0957234
5600000 0.0956896
5610000 0.0956758
5620000 0.0956387
5630000 0.0956245
5640000 0.0955943
5650000 0.0955506
5660000 0.0955384
5670000 0.0955044
5680000 0.0954735
5690000 0.0954375
5700000 0.0954142
5710000 0.0954069
5720000 0.0953663
5730000 0.0953395
5740000 0.0953067
5750000 0.0953341
5760000 0.0953334
5770000 0.0952632
5780000 0.0952412
5790000 0.095225
5800000 0.0952215
5810000 0.0951611
5820000 0.0951335
5830000 0.0950873
5840000 0.0950622
5850000 0.095056
5860000 0.0950375
5870000 0.0949963
5880000 0.0949906
5890000 0.0949431
5900000 0.094903
5910000 0.0948588
5920000 0.0948124
5930000 0.0947946
5940000 0.0947854
5950000 0.0947265
5960000 0.0947206
5970000 0.0946713
5980000 0.0946505
5990000 0.0946301
6000000 0.0946265
6010000 0.0945847
6020000 0.0945432
6030000 0.0945436
6040000 0.0945119
6050000 0.094473
6060000 0.0944294
6070000 0.09439
6080000 0.0943899
6090000 0.0943474
6100000 0.0943356
6110000 0.0943318
6120000 0.094341
6130000 0.0943403
6140000 0.094314
6150000 0.0942856
6160000 0.0942665
6170000 0.0942528
6180000 0.0942385
6190000 0.0941973
6200000 0.0942246
6210000 0.0942184
6220000 0.0941994
6230000 0.0941921
6240000 0.0941485
6250000 0.0941289
6260000 0.0941311
6270000 0.0940788
6280000 0.0940363
6290000 0.0940013
6300000 0.0939661
6310000 0.0939444
6320000 0.0938837
6330000 0.0938459
6340000 0.0938392
6350000 0.0938452
6360000 0.0938191
6370000 0.0938198
6380000 0.0937989
6390000 0.0937321
6400000 0.0937422
6410000 0.0936964
6420000 0.0936589
6430000 0.0936518
6440000 0.093634
6450000 0.0936242
6460000 0.0936094
6470000 0.0936112
6480000 0.0935569
6490000 0.0935411
6500000 0.0934758
6510000 0.0934406
6520000 0.0934145
6530000 0.0933963
6540000 0.0933635
6550000 0.0933848
6560000 0.0933357
6570000 0.0933162
6580000 0.0932736
6590000 0.0932085
6600000 0.0931877
6610000 0.0931652
6620000 0.093125
6630000 0.0931371
6640000 0.0931154
6650000 0.0930767
6660000 0.0930719
6670000 0.0930855
6680000 0.0930672
6690000 0.0930331
6700000 0.0930618
6710000 0.0930405
6720000 0.0929639
6730000 0.0929349
6740000 0.0929038
6750000 0.0928635
6760000 0.0928314
6770000 0.0928249
6780000 0.0928046
6790000 0.0927984
6800000 0.0927358
6810000 0.092698
6820000 0.0926367
6830000 0.0925973
6840000 0.0925989
6850000 0.0926233
6860000 0.0926173
6870000 0.0925753
6880000 0.0925801
6890000 0.092541
6900000 0.0925367
6910000 0.0925254
6920000 0.0925356
6930000 0.0925351
6940000 0.0925006
6950000 0.0924772
6960000 0.0924598
6970000 0.0924732
6980000 0.0924692
6990000 0.0924323
7000000 0.0924196
7010000 0.0923816
7020000 0.0923498
7030000 0.0923209
7040000 0.0923
7050000 0.092322
7060000 0.0923013
7070000 0.0922743
7080000 0.092251
7090000 0.0922262
7100000 0.0921926
7110000 0.0921655
7120000 0.0921492
7130000 0.0921468
7140000 0.0921259
7150000 0.0921133
7160000 0.0920667
7170000 0.0920501
7180000 0.0920101
7190000 0.0919784
7200000 0.0919427
7210000 0.0919256
7220000 0.0919248
7230000 0.0918969
7240000 0.0919011
7250000 0.0918645
7260000 0.0918415
7270000 0.0918239
7280000 0.0918056
7290000 0.0917778
7300000 0.0917436
7310000 0.0917359
7320000 0.0916974
7330000 0.0917007
7340000 0.0916745
7350000 0.0916529
7360000 0.0916675
7370000 0.0916572
7380000 0.0916372
7390000 0.0916316
7400000 0.0916348
7410000 0.0915992
7420000 0.0915903
7430000 0.0915688
7440000 0.0915508
7450000 0.0915293
7460000 0.0915093
7470000 0.0915102
7480000 0.0915211
7490000 0.0914948
7500000 0.0914814
7510000 0.0914496
7520000 0.0914339
7530000 0.0914167
7540000 0.0914061
7550000 0.0913958
7560000 0.091397
7570000 0.0913729
7580000 0.0913681
7590000 0.0913687
7600000 0.0913213
7610000 0.0913262
7620000 0.0913069
7630000 0.0913045
7640000 0.0912804
7650000 0.0912591
7660000 0.0912367
7670000 0.091232
7680000 0.0912109
7690000 0.0912011
7700000 0.0912298
7710000 0.0912297
7720000 0.0912683
7730000 0.0912308
7740000 0.091226
7750000 0.0912032
7760000 0.0911663
7770000 0.0911452
7780000 0.0911252
7790000 0.0911364
7800000 0.091123
7810000 0.0911047
7820000 0.0910982
7830000 0.0910783
7840000 0.0910335
7850000 0.0909978
7860000 0.0909915
7870000 0.090983
7880000 0.0909802
7890000 0.0909613
7900000 0.0909412
7910000 0.0909338
7920000 0.0909186
7930000 0.0909154
7940000 0.0908892
7950000 0.0908774
7960000 0.0908377
7970000 0.0908362
7980000 0.0907892
7990000 0.0907867
8000000 0.0907835
8010000 0.0907991
8020000 0.0907823
8030000 0.0907743
8040000 0.0907495
8050000 0.0907406
8060000 0.0907502
8070000 0.0907634
8080000 0.0907523
8090000 0.0907304
8100000 0.0907233
8110000 0.090708
8120000 0.0906966
8130000 0.0906861
8140000 0.0906972
8150000 0.0906889
8160000 0.0906598
8170000 0.090636
8180000 0.0906136
8190000 0.0906054
8200000 0.0906039
8210000 0.0905703
8220000 0.0905644
8230000 0.0905646
8240000 0.0905496
8250000 0.0905302
8260000 0.0905092
8270000 0.0904877
8280000 0.0904682
8290000 0.0904418
8300000 0.0904485
8310000 0.0904412
8320000 0.0904252
8330000 0.0904208
8340000 0.0903996
8350000 0.0904175
8360000 0.0904079
8370000 0.0903846
8380000 0.0903809
8390000 0.0903872
8400000 0.0903713
8410000 0.0903645
8420000 0.090357
8430000 0.0903568
8440000 0.090369
8450000 0.0903554
8460000 0.0903153
8470000 0.0902915
8480000 0.0902747
8490000 0.0902551
8500000 0.0902464
8510000 0.0902209
8520000 0.0901813
8530000 0.0901738
8540000 0.0901544
8550000 0.0901526
8560000 0.0901604
8570000 0.0901577
8580000 0.0901263
8590000 0.0901146
8600000 0.0901062
8610000 0.0900885
8620000 0.0900679
8630000 0.0900452
8640000 0.0900468
8650000 0.0900358
8660000 0.0900116
8670000 0.0900118
8680000 0.0900124
8690000 0.0900497
8700000 0.0900458
8710000 0.0900221
8720000 0.0900299
8730000 0.0900236
8740000 0.0900162
8750000 0.0900325
8760000 0.0900222
8770000 0.0900213
8780000 0.0899956
8790000 0.0899784
8800000 0.0899971
8810000 0.0899904
8820000 0.0899896
8830000 0.089963
8840000 0.0899668
8850000 0.0899457
8860000 0.0899699
8870000 0.08996
8880000 0.0899476
8890000 0.0899126
8900000 0.0899137
8910000 0.0899135
8920000 0.0899008
8930000 0.0898847
8940000 0.089876
8950000 0.0898677
8960000 0.0898428
8970000 0.0898285
8980000 0.0898016
8990000 0.0898006
9000000 0.0897946
9010000 0.0897889
9020000 0.0897629
9030000 0.0897592
9040000 0.0897327
9050000 0.0897157
9060000 0.089727
9070000 0.0896975
9080000 0.0897114
9090000 0.0897333
9100000 0.0897054
9110000 0.0896938
9120000 0.0896767
9130000 0.0896745
9140000 0.0896768
9150000 0.0896623
9160000 0.0896498
9170000 0.0896481
9180000 0.0896344
9190000 0.0896019
9200000 0.0895972
9210000 0.0895878
9220000 0.0895744
9230000 0.0895672
9240000 0.0895535
9250000 0.0895611
9260000 0.0895589
9270000 0.0895404
9280000 0.089538
9290000 0.0895358
9300000 0.0895276
9310000 0.0895424
9320000 0.0895111
9330000 0.0895148
9340000 0.0894933
9350000 0.0894853
9360000 0.0894785
9370000 0.08948
9380000 0.0894772
9390000 0.0894794
9400000 0.0894661
9410000 0.0894562
9420000 0.0894571
9430000 0.0894456
9440000 0.0894341
9450000 0.0894488
9460000 0.089426
9470000 0.0894155
9480000 0.0893925
9490000 0.089377
9500000 0.0893601
9510000 0.0893435
9520000 0.089337
9530000 0.0893428
9540000 0.0893365
9550000 0.0893317
9560000 0.0893113
9570000 0.0893059
9580000 0.0893036
9590000 0.0893113
9600000 0.0893158
9610000 0.0893116
9620000 0.0892866
9630000 0.0892703
9640000 0.0892725
9650000 0.0892555
9660000 0.0892386
9670000 0.0892319
9680000 0.0892252
9690000 0.0892229
9700000 0.089221
9710000 0.0891931
9720000 0.089163
9730000 0.0891465
9740000 0.0891308
9750000 0.0891281
9760000 0.0891083
9770000 0.0891018
9780000 0.0890782
9790000 0.0890683
9800000 0.0890621
9810000 0.0890587
9820000 0.0890966
9830000 0.0890754
9840000 0.0890693
9850000 0.0890714
9860000 0.0890734
9870000 0.0890917
9880000 0.0890726
9890000 0.0890727
9900000 0.089076
9910000 0.0890528
9920000 0.089055
9930000 0.089016
9940000 0.0890052
9950000 0.0890026
9960000 0.0889911
9970000 0.0889818
9980000 0.088962
9990000 0.0889688
10000000 0.0890398


==> Figures/2DResults/Interior/Dirichlet.tex <==
10000 0.388115
20000 0.275756
30000 0.2265
40000 0.196781
50000 0.176649
60000 0.163375
70000 0.151603
80000 0.142338
90000 0.133873
100000 0.126544
110000 0.120705
120000 0.116081
130000 0.112261
140000 0.108639
150000 0.105647
160000 0.102648
170000 0.0990948
180000 0.0963578
190000 0.0940859
200000 0.0919961
210000 0.089933
220000 0.0886069
230000 0.0867897
240000 0.0852875
250000 0.0838669
260000 0.0825013
270000 0.0814044
280000 0.0803591
290000 0.0791402
300000 0.0779008
310000 0.0769467
320000 0.0758052
330000 0.0750355
340000 0.07399
350000 0.0732494
360000 0.0723791
370000 0.0716291
380000 0.0708152
390000 0.0700937
400000 0.0694703
410000 0.0689042
420000 0.0682791
430000 0.0675711
440000 0.066887
450000 0.066203
460000 0.0656799
470000 0.0651819
480000 0.06458
490000 0.0641442
500000 0.0636498
510000 0.0631987
520000 0.0628494
530000 0.0623809
540000 0.0619354
550000 0.0615275
560000 0.0610133
570000 0.0606591
580000 0.0603246
590000 0.0599309
600000 0.0594665
610000 0.05913
620000 0.05882
630000 0.0585246
640000 0.0582016
650000 0.0579248
660000 0.0575988
670000 0.0575476
680000 0.0571708
690000 0.0569378
700000 0.0566839
710000 0.0565493
720000 0.0562777
730000 0.0560549
740000 0.0557582
750000 0.0554254
760000 0.0552023
770000 0.0550345
780000 0.0547919
790000 0.05464
800000 0.0545097
810000 0.0542966
820000 0.0541388
830000 0.053903
840000 0.0536972
850000 0.0536163
860000 0.0534857
870000 0.0532839
880000 0.0532042
890000 0.0530463
900000 0.0529275
910000 0.0528298
920000 0.0527573
930000 0.0526315
940000 0.0523788
950000 0.0522578
960000 0.0521469
970000 0.051889
980000 0.05169
990000 0.0515041
1000000 0.0513696
1010000 0.0511759
1020000 0.0510135
1030000 0.0507623
1040000 0.0506281
1050000 0.0505457
1060000 0.0504397
1070000 0.0503494
1080000 0.05025
1090000 0.0501946
1100000 0.0500488
1110000 0.0499063
1120000 0.0497173
1130000 0.0496165
1140000 0.0495217
1150000 0.0493631
1160000 0.0492443
1170000 0.049131
1180000 0.0490717
1190000 0.0489896
1200000 0.0488767
1210000 0.0487779
1220000 0.0486867
1230000 0.0485841
1240000 0.0484248
1250000 0.0482752
1260000 0.0481037
1270000 0.0480221
1280000 0.0479326
1290000 0.047838
1300000 0.0476917
1310000 0.0475186
1320000 0.0474036
1330000 0.0473404
1340000 0.0472641
1350000 0.0471919
1360000 0.0470336
1370000 0.0469104
1380000 0.0467894
1390000 0.0467007
1400000 0.0466615
1410000 0.0466048
1420000 0.0464996
1430000 0.0464247
1440000 0.0463376
1450000 0.0462741
1460000 0.0461389
1470000 0.0460841
1480000 0.0460015
1490000 0.0459443
1500000 0.045934
1510000 0.0458487
1520000 0.0457811
1530000 0.0456837
1540000 0.045623
1550000 0.0455507
1560000 0.0454325
1570000 0.0454036
1580000 0.0453153
1590000 0.0451988
1600000 0.0451133
1610000 0.0450614
1620000 0.0449859
1630000 0.0449082
1640000 0.0448395
1650000 0.0447983
1660000 0.0448078
1670000 0.0447168
1680000 0.0446591
1690000 0.0446001
1700000 0.0445515
1710000 0.0444986
1720000 0.0444221
1730000 0.0443963
1740000 0.0442927
1750000 0.044221
1760000 0.0441427
1770000 0.0440883
1780000 0.0440801
1790000 0.0440209
1800000 0.0439126
1810000 0.0438426
1820000 0.0437562
1830000 0.0437394
1840000 0.0436752
1850000 0.0436008
1860000 0.0435822
1870000 0.043525
1880000 0.0434314
1890000 0.0434189
1900000 0.0433534
1910000 0.0433236
1920000 0.0432696
1930000 0.0432525
1940000 0.0432303
1950000 0.0431942
1960000 0.0431838
1970000 0.0431448
1980000 0.0430592
1990000 0.0430192
2000000 0.0429587
2010000 0.0428819
2020000 0.0428091
2030000 0.0427649
2040000 0.042716
2050000 0.0426551
2060000 0.0426068
2070000 0.0425882
2080000 0.0425729
2090000 0.0425548
2100000 0.0425426
2110000 0.0425013
2120000 0.0424787
2130000 0.0424284
2140000 0.0423563
2150000 0.0423192
2160000 0.0422974
2170000 0.0422972
2180000 0.0422424
2190000 0.0421918
2200000 0.0421462
2210000 0.0421406
2220000 0.0420976
2230000 0.0420632
2240000 0.0419911
2250000 0.0419533
2260000 0.0419278
2270000 0.041885
2280000 0.0418487
2290000 0.0418194
2300000 0.0418117
2310000 0.041736
2320000 0.0416927
2330000 0.0416746
2340000 0.041607
2350000 0.0415795
2360000 0.0415781
2370000 0.0415455
2380000 0.0414974
2390000 0.0414698
2400000 0.0414687
2410000 0.0414109
2420000 0.0413811
2430000 0.0413326
2440000 0.0413249
2450000 0.0413063
2460000 0.0412938
2470000 0.0412657
2480000 0.0412399
2490000 0.0412594
2500000 0.0412028
2510000 0.0411748
2520000 0.0411299
2530000 0.0410905
2540000 0.0410604
2550000 0.0410436
2560000 0.0410401
2570000 0.0410353
2580000 0.0410225
2590000 0.0409646
2600000 0.0409391
2610000 0.040902
2620000 0.0408931
2630000 0.0408662
2640000 0.0408314
2650000 0.0407771
2660000 0.0407749
2670000 0.0407183
2680000 0.0406856
2690000 0.0406448
2700000 0.0405973
2710000 0.0405708
2720000 0.0405318
2730000 0.0404791
2740000 0.0404505
2750000 0.0404057
2760000 0.0403947
2770000 0.0403838
2780000 0.0403321
2790000 0.0403172
2800000 0.0402665
2810000 0.0402417
2820000 0.0402162
2830000 0.0401775
2840000 0.0401557
2850000 0.0401014
2860000 0.0400501
2870000 0.040038
2880000 0.039993
2890000 0.0399738
2900000 0.0399184
2910000 0.039883
2920000 0.0399028
2930000 0.0398529
2940000 0.0398305
2950000 0.0397966
2960000 0.0397834
2970000 0.0397648
2980000 0.039728
2990000 0.0397185
3000000 0.0396903
3010000 0.039682
3020000 0.039652
3030000 0.0396293
3040000 0.0395993
3050000 0.0395819
3060000 0.0395646
3070000 0.0395265
3080000 0.0395146
3090000 0.0395186
3100000 0.0394775
3110000 0.0394618
3120000 0.0394419
3130000 0.0394359
3140000 0.0393978
3150000 0.0393811
3160000 0.0393569
3170000 0.0393383
3180000 0.0393275
3190000 0.0393047
3200000 0.0393077
3210000 0.0392868
3220000 0.0392388
3230000 0.0392251
3240000 0.0392128
3250000 0.0392052
3260000 0.0391707
3270000 0.0391747
3280000 0.0391541
3290000 0.039146
3300000 0.0391353
3310000 0.0390932
3320000 0.0391112
3330000 0.0390766
3340000 0.0390501
3350000 0.0390314
3360000 0.0390066
3370000 0.0389947
3380000 0.0389727
3390000 0.0389817
3400000 0.0389677
3410000 0.0389408
3420000 0.0389293
3430000 0.0389191
3440000 0.0389074
3450000 0.0388922
3460000 0.0388591
3470000 0.0388535
3480000 0.0388401
3490000 0.0387988
3500000 0.038779
3510000 0.0387492
3520000 0.0387566
3530000 0.0387411
3540000 0.0387177
3550000 0.0386856
3560000 0.0386658
3570000 0.0386687
3580000 0.0386456
3590000 0.0386368
3600000 0.0386325
3610000 0.0386311
3620000 0.038608
3630000 0.038567
3640000 0.0385691
3650000 0.0385318
3660000 0.038546
3670000 0.0385357
3680000 0.0385173
3690000 0.0384931
3700000 0.038478
3710000 0.0384633
3720000 0.0384547
3730000 0.0384321
3740000 0.038423
3750000 0.0384022
3760000 0.0383842
3770000 0.0383916
3780000 0.0383793
3790000 0.0383666
3800000 0.0383578
3810000 0.0383394
3820000 0.0383465
3830000 0.0383182
3840000 0.0383028
3850000 0.0382679
3860000 0.0382576
3870000 0.0382276
3880000 0.0382207
3890000 0.0382178
3900000 0.0382129
3910000 0.0382298
3920000 0.0382094
3930000 0.0381829
3940000 0.038176
3950000 0.0381736
3960000 0.0381794
3970000 0.0381586
3980000 0.0381648
3990000 0.0381487
4000000 0.0381332
4010000 0.0381109
4020000 0.0380968
4030000 0.0380854
4040000 0.0380804
4050000 0.0380752
4060000 0.0380877
4070000 0.0380714
4080000 0.0380636
4090000 0.0380446
4100000 0.0380503
4110000 0.0380304
4120000 0.0380125
4130000 0.038013
4140000 0.0380114
4150000 0.0380085
4160000 0.0379941
4170000 0.0379784
4180000 0.0379813
4190000 0.0379634
4200000 0.0379606
4210000 0.0379548
4220000 0.0379555
4230000 0.0379304
4240000 0.0379203
4250000 0.0379044
4260000 0.0378849
4270000 0.0378732
4280000 0.037851
4290000 0.0378312
4300000 0.0378122
4310000 0.037806
4320000 0.0378015
4330000 0.0377913
4340000 0.0377918
4350000 0.0377875
4360000 0.0377822
4370000 0.0377818
4380000 0.0377667
4390000 0.0377631
4400000 0.0377687
4410000 0.0377446
4420000 0.0377369
4430000 0.0377266
4440000 0.0377176
4450000 0.0376983
4460000 0.0376863
4470000 0.0376589
4480000 0.0376421
4490000 0.0376286
4500000 0.0376254
4510000 0.037617
4520000 0.0376064
4530000 0.0376154
4540000 0.0376069
4550000 0.0376059
4560000 0.0375834
4570000 0.037573
4580000 0.0375698
4590000 0.037536
4600000 0.0375306
4610000 0.0375065
4620000 0.0374975
4630000 0.0374837
4640000 0.0374482
4650000 0.037444
4660000 0.0374305
4670000 0.0374203
4680000 0.0374026
4690000 0.0373987
4700000 0.0373858
4710000 0.0373664
4720000 0.0373543
4730000 0.0373388
4740000 0.0373155
4750000 0.0373086
4760000 0.0372958
4770000 0.0372798
4780000 0.0372618
4790000 0.0372429
4800000 0.0372285
4810000 0.0372026
4820000 0.0371809
4830000 0.037176
4840000 0.0371693
4850000 0.0371695
4860000 0.0371649
4870000 0.0371545
4880000 0.0371629
4890000 0.0371694
4900000 0.0371683
4910000 0.037161
4920000 0.037136
4930000 0.0371293
4940000 0.0371275
4950000 0.0371211
4960000 0.0371129
4970000 0.0370899
4980000 0.037084
4990000 0.0370755
5000000 0.0370633
5010000 0.0370504
5020000 0.0370562
5030000 0.0370496
5040000 0.0370497
5050000 0.0370414
5060000 0.0370455
5070000 0.0370324
5080000 0.0370145
5090000 0.037
5100000 0.0369992
5110000 0.0370046
5120000 0.036994
5130000 0.0369848
5140000 0.0369751
5150000 0.0369746
5160000 0.0369632
5170000 0.0369514
5180000 0.0369487
5190000 0.0369296
5200000 0.0369162
5210000 0.0369147
5220000 0.0369182
5230000 0.0368939
5240000 0.0368923
5250000 0.0368894
5260000 0.0368959
5270000 0.0368923
5280000 0.0368879
5290000 0.0368874
5300000 0.0368875
5310000 0.0368775
5320000 0.0368712
5330000 0.0368763
5340000 0.0368603
5350000 0.0368475
5360000 0.0368522
5370000 0.0368349
5380000 0.0368316
5390000 0.0368184
5400000 0.036807
5410000 0.0368037
5420000 0.0367907
5430000 0.036783
5440000 0.0367677
5450000 0.0367616
5460000 0.0367579
5470000 0.036753
5480000 0.036761
5490000 0.0367554
5500000 0.0367537
5510000 0.0367345
5520000 0.0367365
5530000 0.0367408
5540000 0.0367315
5550000 0.0367243
5560000 0.0367322
5570000 0.0367387
5580000 0.0367259
5590000 0.036718
5600000 0.0367173
5610000 0.0367079
5620000 0.0367017
5630000 0.0366878
5640000 0.0366975
5650000 0.036678
5660000 0.0366716
5670000 0.036693
5680000 0.0366757
5690000 0.0366832
5700000 0.0366536
5710000 0.0366638
5720000 0.0366761
5730000 0.0366728
5740000 0.0366682
5750000 0.0366498
5760000 0.036648
5770000 0.0366419
5780000 0.0366266
5790000 0.0366324
5800000 0.0366396
5810000 0.0366241
5820000 0.0366236
5830000 0.0366142
5840000 0.0366196
5850000 0.0366079
5860000 0.0366008
5870000 0.0365961
5880000 0.0365871
5890000 0.0365784
5900000 0.0365743
5910000 0.0365716
5920000 0.0365768
5930000 0.0365765
5940000 0.036571
5950000 0.0365694
5960000 0.0365579
5970000 0.0365596
5980000 0.036564
5990000 0.0365638
6000000 0.0365649
6010000 0.0365537
6020000 0.0365661
6030000 0.0365636
6040000 0.0365493
6050000 0.0365321
6060000 0.0365283
6070000 0.0365281
6080000 0.0365104
6090000 0.0365074
6100000 0.0365091
6110000 0.0365216
6120000 0.0365256
6130000 0.0365095
6140000 0.0365131
6150000 0.0365126
6160000 0.0365232
6170000 0.0365153
6180000 0.0365013
6190000 0.0364916
6200000 0.0364877
6210000 0.0364854
6220000 0.0364692
6230000 0.0364714
6240000 0.036473
6250000 0.0364643
6260000 0.0364659
6270000 0.0364604
6280000 0.0364511
6290000 0.0364398
6300000 0.0364492
6310000 0.036432
6320000 0.0364242
6330000 0.0364197
6340000 0.0364086
6350000 0.0364161
6360000 0.0363993
6370000 0.0363908
6380000 0.036383
6390000 0.0363705
6400000 0.0363629
6410000 0.0363492
6420000 0.0363371
6430000 0.0363288
6440000 0.0363235
6450000 0.0363239
6460000 0.0363253
6470000 0.0363193
6480000 0.036317
6490000 0.0363273
6500000 0.0363263
6510000 0.0363167
6520000 0.0363153
6530000 0.0362963
6540000 0.0362864
6550000 0.0362778
6560000 0.0362812
6570000 0.0362854
6580000 0.0362827
6590000 0.0362741
6600000 0.0362713
6610000 0.0362623
6620000 0.0362544
6630000 0.0362618
6640000 0.0362584
6650000 0.0362572
6660000 0.0362465
6670000 0.0362494
6680000 0.0362395
6690000 0.0362391
6700000 0.0362263
6710000 0.0362268
6720000 0.0362187
6730000 0.036208
6740000 0.0361992
6750000 0.0361934
6760000 0.0361739
6770000 0.0361728
6780000 0.0361672
6790000 0.036162
6800000 0.0361573
6810000 0.0361508
6820000 0.0361529
6830000 0.0361431
6840000 0.0361441
6850000 0.0361348
6860000 0.0361188
6870000 0.0361078
6880000 0.0360964
6890000 0.0360844
6900000 0.0360681
6910000 0.0360731
6920000 0.0360661
6930000 0.0360611
6940000 0.0360587
6950000 0.0360371
6960000 0.0360394
6970000 0.0360357
6980000 0.0360256
6990000 0.03603
7000000 0.0360126
7010000 0.0360008
7020000 0.0360011
7030000 0.0359906
7040000 0.0359869
7050000 0.0359811
7060000 0.0359824
7070000 0.0359938
7080000 0.03598
7090000 0.0359693
7100000 0.0359523
7110000 0.0359484
7120000 0.0359381
7130000 0.0359314
7140000 0.0359259
7150000 0.0359179
7160000 0.0359163
7170000 0.035914
7180000 0.0359141
7190000 0.0359068
7200000 0.0358973
7210000 0.0358968
7220000 0.0358993
7230000 0.0358953
7240000 0.0358846
7250000 0.0358805
7260000 0.0358759
7270000 0.0358606
7280000 0.0358611
7290000 0.0358538
7300000 0.0358583
7310000 0.035846
7320000 0.0358483
7330000 0.0358466
7340000 0.0358469
7350000 0.0358437
7360000 0.0358402
7370000 0.0358301
7380000 0.0358254
7390000 0.0358231
7400000 0.0358315
7410000 0.0358263
7420000 0.0358206
7430000 0.0358108
7440000 0.0358116
7450000 0.0358083
7460000 0.0357986
7470000 0.0358043
7480000 0.0358051
7490000 0.0357921
7500000 0.0357803
7510000 0.0357681
7520000 0.0357557
7530000 0.03576
7540000 0.0357555
7550000 0.0357486
7560000 0.0357509
7570000 0.0357451
7580000 0.0357515
7590000 0.035749
7600000 0.0357513
7610000 0.0357622
7620000 0.0357646
7630000 0.0357742
7640000 0.0357689
7650000 0.0357597
7660000 0.0357591
7670000 0.0357543
7680000 0.0357523
7690000 0.0357509
7700000 0.0357456
7710000 0.0357371
7720000 0.0357176
7730000 0.0357227
7740000 0.0357254
7750000 0.0357285
7760000 0.035719
7770000 0.035714
7780000 0.0357038
7790000 0.0357075
7800000 0.0357095
7810000 0.035702
7820000 0.0357025
7830000 0.0356976
7840000 0.0356907
7850000 0.0356971
7860000 0.0356892
7870000 0.0356953
7880000 0.0356898
7890000 0.035699
7900000 0.0356922
7910000 0.0356929
7920000 0.035694
7930000 0.0356897
7940000 0.0356856
7950000 0.0356874
7960000 0.0356804
7970000 0.03567
7980000 0.0356565
7990000 0.035661
8000000 0.0356504
8010000 0.0356429
8020000 0.0356374
8030000 0.0356264
8040000 0.0356269
8050000 0.0356232
8060000 0.035629
8070000 0.0356133
8080000 0.0356139
8090000 0.0356142
8100000 0.0356022
8110000 0.0356
8120000 0.0355889
8130000 0.0355899
8140000 0.0355836
8150000 0.0355745
8160000 0.0355761
8170000 0.0355688
8180000 0.0355782
8190000 0.0355734
8200000 0.0355638
8210000 0.0355667
8220000 0.03557
8230000 0.0355652
8240000 0.0355678
8250000 0.0355637
8260000 0.0355603
8270000 0.0355547
8280000 0.0355564
8290000 0.0355477
8300000 0.0355406
8310000 0.0355323
8320000 0.0355294
8330000 0.0355216
8340000 0.0355173
8350000 0.0355139
8360000 0.0355044
8370000 0.0354974
8380000 0.03549
8390000 0.0354908
8400000 0.0354883
8410000 0.0354904
8420000 0.0354811
8430000 0.0354725
8440000 0.0354747
8450000 0.0354723
8460000 0.0354617
8470000 0.0354582
8480000 0.0354616
8490000 0.0354674
8500000 0.0354496
8510000 0.0354531
8520000 0.0354436
8530000 0.0354409
8540000 0.0354292
8550000 0.0354153
8560000 0.0354118
8570000 0.0354096
8580000 0.0354076
8590000 0.0354053
8600000 0.0354093
8610000 0.0354076
8620000 0.0354097
8630000 0.0354147
8640000 0.0354133
8650000 0.0354101
8660000 0.0353925
8670000 0.035385
8680000 0.0353794
8690000 0.035374
8700000 0.0353777
8710000 0.035376
8720000 0.0353757
8730000 0.0353833
8740000 0.0353759
8750000 0.0353765
8760000 0.035369
8770000 0.0353761
8780000 0.0353629
8790000 0.035363
8800000 0.035359
8810000 0.0353637
8820000 0.0353612
8830000 0.0353585
8840000 0.0353542
8850000 0.0353504
8860000 0.0353441
8870000 0.0353521
8880000 0.0353436
8890000 0.0353444
8900000 0.0353378
8910000 0.0353243
8920000 0.0353153
8930000 0.0353134
8940000 0.035309
8950000 0.0353062
8960000 0.0353058
8970000 0.0353088
8980000 0.0353065
8990000 0.0353129
9000000 0.0353108
9010000 0.0353067
9020000 0.0353056
9030000 0.0353026
9040000 0.0352946
9050000 0.0352959
9060000 0.0352952
9070000 0.0353002
9080000 0.0353057
9090000 0.035305
9100000 0.0353042
9110000 0.0353059
9120000 0.0353009
9130000 0.0352981
9140000 0.0352932
9150000 0.0352897
9160000 0.0352927
9170000 0.0352853
9180000 0.035276
9190000 0.0352747
9200000 0.0352855
9210000 0.0352775
9220000 0.0352697
9230000 0.0352614
9240000 0.0352614
9250000 0.0352661
9260000 0.0352571
9270000 0.0352575
9280000 0.0352531
9290000 0.0352516
9300000 0.0352441
9310000 0.0352452
9320000 0.0352475
9330000 0.0352416
9340000 0.0352334
9350000 0.0352377
9360000 0.0352391
9370000 0.0352382
9380000 0.0352372
9390000 0.0352334
9400000 0.0352315
9410000 0.0352253
9420000 0.0352217
9430000 0.0352302
9440000 0.035224
9450000 0.0352234
9460000 0.03522
9470000 0.0352142
9480000 0.0352201
9490000 0.0352153
9500000 0.035217
9510000 0.0352219
9520000 0.0352135
9530000 0.0352117
9540000 0.0352118
9550000 0.0352109
9560000 0.0352022
9570000 0.0352005
9580000 0.0352032
9590000 0.0351975
9600000 0.0351956
9610000 0.0351905
9620000 0.0351951
9630000 0.0351979
9640000 0.0351989
9650000 0.0351975
9660000 0.0351987
9670000 0.0351918
9680000 0.0351921
9690000 0.0351816
9700000 0.0351767
9710000 0.0351723
9720000 0.0351653
9730000 0.0351595
9740000 0.0351593
9750000 0.0351589
9760000 0.0351524
9770000 0.0351486
9780000 0.0351535
9790000 0.0351553
9800000 0.0351582
9810000 0.0351458
9820000 0.035144
9830000 0.0351383
9840000 0.0351311
9850000 0.0351287
9860000 0.0351244
9870000 0.0351188
9880000 0.0351208
9890000 0.0351187
9900000 0.0351149
9910000 0.0351098
9920000 0.035102
9930000 0.0351012
9940000 0.0350998
9950000 0.0351021
9960000 0.0350975
9970000 0.0350979
9980000 0.0350925
9990000 0.0350906
10000000 0.0350891


==> Figures/2DResults/Interior/Mixed.tex <==
10000 0.549147
20000 0.395586
30000 0.321522
40000 0.277564
50000 0.268965
60000 0.245117
70000 0.233688
80000 0.215121
90000 0.201995
100000 0.19189
110000 0.183279
120000 0.183711
130000 0.178735
140000 0.172064
150000 0.165843
160000 0.160558
170000 0.157139
180000 0.152912
190000 0.148487
200000 0.144139
210000 0.140919
220000 0.138088
230000 0.134923
240000 0.132
250000 0.129681
260000 0.1272
270000 0.125032
280000 0.122556
290000 0.120314
300000 0.118544
310000 0.11679
320000 0.115141
330000 0.113315
340000 0.111914
350000 0.110147
360000 0.108782
370000 0.107403
380000 0.1063
390000 0.104992
400000 0.104098
410000 0.103089
420000 0.102067
430000 0.101187
440000 0.10023
450000 0.0990922
460000 0.098306
470000 0.0975227
480000 0.104118
490000 0.103385
500000 0.102365
510000 0.101323
520000 0.10034
530000 0.0993449
540000 0.0986731
550000 0.097828
560000 0.0969555
570000 0.0961329
580000 0.0955887
590000 0.0947051
600000 0.093953
610000 0.0934486
620000 0.092654
630000 0.0923226
640000 0.0914303
650000 0.0907961
660000 0.0900588
670000 0.089455
680000 0.0890277
690000 0.0883434
700000 0.0877433
710000 0.0871679
720000 0.0867569
730000 0.0862376
740000 0.085905
750000 0.0852743
760000 0.0847998
770000 0.0843404
780000 0.0840585
790000 0.0837412
800000 0.0831985
810000 0.0827163
820000 0.0823053
830000 0.0820754
840000 0.0816785
850000 0.0812026
860000 0.0808378
870000 0.0807452
880000 0.0804746
890000 0.0802149
900000 0.0799745
910000 0.0795672
920000 0.0793961
930000 0.0790179
940000 0.0786982
950000 0.0785104
960000 0.0782555
970000 0.0779039
980000 0.077545
990000 0.0772302
1000000 0.076962
1010000 0.0767261
1020000 0.0763307
1030000 0.0760518
1040000 0.0757254
1050000 0.0754947
1060000 0.0751563
1070000 0.0748592
1080000 0.0749264
1090000 0.0748246
1100000 0.0745023
1110000 0.0741272
1120000 0.0739064
1130000 0.0737586
1140000 0.0735086
1150000 0.0732556
1160000 0.0730658
1170000 0.0727854
1180000 0.0725238
1190000 0.0726773
1200000 0.0724643
1210000 0.0725493
1220000 0.072288
1230000 0.0720732
1240000 0.0717578
1250000 0.0715062
1260000 0.0712614
1270000 0.0710918
1280000 0.0708651
1290000 0.0707869
1300000 0.070543
1310000 0.0702941
1320000 0.0702117
1330000 0.070047
1340000 0.069833
1350000 0.0696673
1360000 0.0694667
1370000 0.0694828
1380000 0.0693836
1390000 0.0692091
1400000 0.0691079
1410000 0.0690161
1420000 0.0688323
1430000 0.0685919
1440000 0.0684772
1450000 0.0682718
1460000 0.0681316
1470000 0.0679849
1480000 0.067863
1490000 0.0676326
1500000 0.067454
1510000 0.067384
1520000 0.0672803
1530000 0.0671186
1540000 0.0670121
1550000 0.0668867
1560000 0.0667706
1570000 0.0666348
1580000 0.0664718
1590000 0.0663466
1600000 0.0661741
1610000 0.0660369
1620000 0.0659272
1630000 0.0658875
1640000 0.065745
1650000 0.0657165
1660000 0.0656314
1670000 0.0655474
1680000 0.0654521
1690000 0.0653182
1700000 0.0651983
1710000 0.0651123
1720000 0.0649209
1730000 0.0648345
1740000 0.0648138
1750000 0.064708
1760000 0.0646171
1770000 0.0645555
1780000 0.0644403
1790000 0.0644382
1800000 0.0643306
1810000 0.064223
1820000 0.0641235
1830000 0.0640234
1840000 0.0639251
1850000 0.0638184
1860000 0.063733
1870000 0.0636125
1880000 0.0635201
1890000 0.0634096
1900000 0.0633447
1910000 0.0632079
1920000 0.0631515
1930000 0.0631394
1940000 0.0631205
1950000 0.0630727
1960000 0.0629646
1970000 0.0629165
1980000 0.0628036
1990000 0.0627344
2000000 0.0626728
2010000 0.0626206
2020000 0.0625035
2030000 0.0624023
2040000 0.0623311
2050000 0.0622737
2060000 0.0621929
2070000 0.0621479
2080000 0.0620761
2090000 0.0619919
2100000 0.061971
2110000 0.0618286
2120000 0.0617056
2130000 0.0616305
2140000 0.0615501
2150000 0.0615048
2160000 0.0614143
2170000 0.0613459
2180000 0.0612555
2190000 0.0611808
2200000 0.0610568
2210000 0.0609446
2220000 0.0609069
2230000 0.0608329
2240000 0.0607234
2250000 0.0606506
2260000 0.0606136
2270000 0.0605288
2280000 0.0604785
2290000 0.0604114
2300000 0.0603671
2310000 0.0602707
2320000 0.0602606
2330000 0.060193
2340000 0.0601239
2350000 0.0600819
2360000 0.0599804
2370000 0.0599231
2380000 0.0598366
2390000 0.0597607
2400000 0.0596809
2410000 0.059638
2420000 0.0595543
2430000 0.0601372
2440000 0.0601006
2450000 0.0600683
2460000 0.0600168
2470000 0.0600141
2480000 0.0599873
2490000 0.0599436
2500000 0.0599176
2510000 0.0598481
2520000 0.0597962
2530000 0.0597164
2540000 0.0597025
2550000 0.0596451
2560000 0.0595979
2570000 0.0595597
2580000 0.0595408
2590000 0.0594882
2600000 0.0594697
2610000 0.0594487
2620000 0.0594011
2630000 0.0593701
2640000 0.0593136
2650000 0.0592492
2660000 0.0592431
2670000 0.0592281
2680000 0.0591501
2690000 0.0590976
2700000 0.0590831
2710000 0.0591069
2720000 0.0590537
2730000 0.0590068
2740000 0.0589278
2750000 0.0588969
2760000 0.0588774
2770000 0.058832
2780000 0.0587984
2790000 0.0587625
2800000 0.0587048
2810000 0.0586023
2820000 0.0592321
2830000 0.0592309
2840000 0.0592122
2850000 0.0591913
2860000 0.0591146
2870000 0.0590808
2880000 0.059029
2890000 0.0589463
2900000 0.0588727
2910000 0.0588746
2920000 0.0588797
2930000 0.0588038
2940000 0.0587255
2950000 0.0587001
2960000 0.0586852
2970000 0.0585997
2980000 0.05971
2990000 0.0596254
3000000 0.0595783
3010000 0.0595204
3020000 0.0595113
3030000 0.0594762
3040000 0.0594462
3050000 0.0594112
3060000 0.0593686
3070000 0.0593205
3080000 0.0592608
3090000 0.0592359
3100000 0.0591713
3110000 0.0591125
3120000 0.0590896
3130000 0.0590041
3140000 0.0589449
3150000 0.0589617
3160000 0.0589451
3170000 0.0588876
3180000 0.0588537
3190000 0.0588353
3200000 0.0587787
3210000 0.0587273
3220000 0.0586819
3230000 0.0586172
3240000 0.0586025
3250000 0.0585398
3260000 0.0585159
3270000 0.0584234
3280000 0.0584226
3290000 0.0584308
3300000 0.0584321
3310000 0.0583809
3320000 0.0583305
3330000 0.0583001
3340000 0.0582915
3350000 0.0582416
3360000 0.0582225
3370000 0.0581781
3380000 0.0584357
3390000 0.0584402
3400000 0.0584099
3410000 0.0583838
3420000 0.0583612
3430000 0.058307
3440000 0.0582868
3450000 0.0582517
3460000 0.0582187
3470000 0.058166
3480000 0.0581349
3490000 0.0581201
3500000 0.0580666
3510000 0.0580276
3520000 0.0579898
3530000 0.0579619
3540000 0.0579399
3550000 0.0579074
3560000 0.0578793
3570000 0.05786
3580000 0.0578583
3590000 0.0578108
3600000 0.0577925
3610000 0.0577614
3620000 0.0577504
3630000 0.0577157
3640000 0.0576709
3650000 0.0576387
3660000 0.0575907
3670000 0.0575392
3680000 0.0575232
3690000 0.0574612
3700000 0.0574203
3710000 0.0574078
3720000 0.0573985
3730000 0.0573888
3740000 0.0573634
3750000 0.0573238
3760000 0.0573069
3770000 0.0572663
3780000 0.0572438
3790000 0.0572189
3800000 0.0570617
3810000 0.0570361
3820000 0.0569577
3830000 0.0569647
3840000 0.05694
3850000 0.0569013
3860000 0.0568648
3870000 0.0568333
3880000 0.0567795
3890000 0.0567698
3900000 0.056727
3910000 0.0567033
3920000 0.0566751
3930000 0.0566452
3940000 0.0566288
3950000 0.0566162
3960000 0.0565985
3970000 0.0566107
3980000 0.0565873
3990000 0.0565361
4000000 0.0565013
4010000 0.0564897
4020000 0.0564835
4030000 0.0564208
4040000 0.0563807
4050000 0.0563587
4060000 0.0563452
4070000 0.0562777
4080000 0.0562522
4090000 0.0562341
4100000 0.0562349
4110000 0.0562115
4120000 0.0561672
4130000 0.0561382
4140000 0.0561048
4150000 0.0560713
4160000 0.0560547
4170000 0.056009
4180000 0.0560094
4190000 0.0559844
4200000 0.0559543
4210000 0.055942
4220000 0.0558914
4230000 0.0558627
4240000 0.0558236
4250000 0.0557923
4260000 0.0557401
4270000 0.055746
4280000 0.0557302
4290000 0.0557088
4300000 0.0557017
4310000 0.0556992
4320000 0.0556566
4330000 0.0556467
4340000 0.0556298
4350000 0.055559
4360000 0.0555374
4370000 0.0555305
4380000 0.0555244
4390000 0.0555275
4400000 0.0555241
4410000 0.0555147
4420000 0.0554921
4430000 0.0554914
4440000 0.0554665
4450000 0.0554233
4460000 0.0553842
4470000 0.0553536
4480000 0.0553269
4490000 0.0553044
4500000 0.0552918
4510000 0.0552904
4520000 0.0552796
4530000 0.0552657
4540000 0.0552131
4550000 0.05519
4560000 0.0551769
4570000 0.05517
4580000 0.0551637
4590000 0.0551295
4600000 0.0551358
4610000 0.0551158
4620000 0.0550887
4630000 0.0550811
4640000 0.0550885
4650000 0.0550966
4660000 0.055067
4670000 0.0550455
4680000 0.0550096
4690000 0.0549796
4700000 0.0549444
4710000 0.0549281
4720000 0.054917
4730000 0.054905
4740000 0.0548931
4750000 0.0548413
4760000 0.0548276
4770000 0.0548053
4780000 0.0547841
4790000 0.0547496
4800000 0.0547416
4810000 0.0547792
4820000 0.0547666
4830000 0.0547527
4840000 0.0547293
4850000 0.0547047
4860000 0.054674
4870000 0.0546447
4880000 0.054606
4890000 0.0545889
4900000 0.054574
4910000 0.0545763
4920000 0.0545591
4930000 0.0545295
4940000 0.054504
4950000 0.0544717
4960000 0.0544564
4970000 0.0544457
4980000 0.054419
4990000 0.054418
5000000 0.0544153
5010000 0.0543767
5020000 0.0543771
5030000 0.0543625
5040000 0.0543559
5050000 0.0543347
5060000 0.0543321
5070000 0.054327
5080000 0.0543241
5090000 0.0542995
5100000 0.0543615
5110000 0.0543559
5120000 0.0543438
5130000 0.0545604
5140000 0.0545408
5150000 0.0545354
5160000 0.0545071
5170000 0.054481
5180000 0.0544677
5190000 0.0544506
5200000 0.0544242
5210000 0.054399
5220000 0.0543958
5230000 0.0543849
5240000 0.0544016
5250000 0.0543868
5260000 0.0543595
5270000 0.0543707
5280000 0.0543665
5290000 0.0543454
5300000 0.0543609
5310000 0.0543477
5320000 0.0543474
5330000 0.0543608
5340000 0.0543546
5350000 0.0543201
5360000 0.0543205
5370000 0.0543159
5380000 0.0543343
5390000 0.0543286
5400000 0.0543201
5410000 0.0543142
5420000 0.0542807
5430000 0.0542747
5440000 0.054263
5450000 0.0542422
5460000 0.0542135
5470000 0.0542054
5480000 0.0542015
5490000 0.0542012
5500000 0.0541883
5510000 0.0541459
5520000 0.0541352
5530000 0.0541106
5540000 0.0541095
5550000 0.0540928
5560000 0.0540641
5570000 0.0540847
5580000 0.0540623
5590000 0.0540329
5600000 0.0540002
5610000 0.0539866
5620000 0.0539864
5630000 0.0539578
5640000 0.0539579
5650000 0.0539296
5660000 0.053922
5670000 0.0539224
5680000 0.0538999
5690000 0.0539088
5700000 0.0539075
5710000 0.0538972
5720000 0.0538911
5730000 0.0538905
5740000 0.0538717
5750000 0.053877
5760000 0.0538812
5770000 0.0538536
5780000 0.0538532
5790000 0.0538317
5800000 0.0538336
5810000 0.0538252
5820000 0.0538121
5830000 0.0537923
5840000 0.053779
5850000 0.0537543
5860000 0.0537409
5870000 0.0537365
5880000 0.0537126
5890000 0.0536782
5900000 0.0536559
5910000 0.0536321
5920000 0.0536033
5930000 0.0535968
5940000 0.0535824
5950000 0.0535817
5960000 0.0535757
5970000 0.0535731
5980000 0.0535904
5990000 0.0535976
6000000 0.0535858
6010000 0.0535687
6020000 0.0535545
6030000 0.0535347
6040000 0.0535692
6050000 0.0535506
6060000 0.0535276
6070000 0.0535127
6080000 0.0534797
6090000 0.0534752
6100000 0.0534567
6110000 0.0534324
6120000 0.0534026
6130000 0.0533864
6140000 0.0533752
6150000 0.0533603
6160000 0.0533423
6170000 0.0533258
6180000 0.0533187
6190000 0.0533025
6200000 0.0532871
6210000 0.0532967
6220000 0.0532964
6230000 0.0532926
6240000 0.0532862
6250000 0.0532746
6260000 0.0532462
6270000 0.0532237
6280000 0.053204
6290000 0.0531926
6300000 0.0531855
6310000 0.0531723
6320000 0.0531338
6330000 0.0531191
6340000 0.0531094
6350000 0.0531207
6360000 0.0530918
6370000 0.0530673
6380000 0.0530443
6390000 0.0530435
6400000 0.0530414
6410000 0.0530303
6420000 0.0530307
6430000 0.0530181
6440000 0.0530122
6450000 0.0530031
6460000 0.0529922
6470000 0.0529773
6480000 0.052962
6490000 0.0529649
6500000 0.0529474
6510000 0.0529348
6520000 0.0529453
6530000 0.0529361
6540000 0.0529164
6550000 0.0529128
6560000 0.0529067
6570000 0.0529021
6580000 0.0528852
6590000 0.0528586
6600000 0.0528484
6610000 0.0528243
6620000 0.052827
6630000 0.0528211
6640000 0.052829
6650000 0.0528012
6660000 0.0528051
6670000 0.0527936
6680000 0.0527746
6690000 0.052754
6700000 0.0527626
6710000 0.0527595
6720000 0.0527497
6730000 0.0527303
6740000 0.0527192
6750000 0.0527098
6760000 0.0527026
6770000 0.0527047
6780000 0.0526837
6790000 0.05269
6800000 0.0526956
6810000 0.0526832
6820000 0.0526582
6830000 0.0526507
6840000 0.0526495
6850000 0.0526526
6860000 0.0526452
6870000 0.0526327
6880000 0.0526207
6890000 0.0526305
6900000 0.0526091
6910000 0.052594
6920000 0.052574
6930000 0.0525777
6940000 0.0525577
6950000 0.0525936
6960000 0.0525991
6970000 0.0525864
6980000 0.0525634
6990000 0.0525454
7000000 0.05254
7010000 0.0525232
7020000 0.0524963
7030000 0.0524859
7040000 0.0524909
7050000 0.052484
7060000 0.0524739
7070000 0.0524476
7080000 0.0524523
7090000 0.0524467
7100000 0.0524349
7110000 0.0524204
7120000 0.0524133
7130000 0.0524275
7140000 0.0524164
7150000 0.0523912
7160000 0.0523983
7170000 0.05238
7180000 0.0523555
7190000 0.052362
7200000 0.0523427
7210000 0.0523246
7220000 0.0523155
7230000 0.0523079
7240000 0.0523066
7250000 0.0522891
7260000 0.052282
7270000 0.052253
7280000 0.0522427
7290000 0.052225
7300000 0.0522151
7310000 0.0521984
7320000 0.052185
7330000 0.0521854
7340000 0.0521807
7350000 0.0521672
7360000 0.0521609
7370000 0.052147
7380000 0.0521437
7390000 0.0521195
7400000 0.0521123
7410000 0.0521124
7420000 0.0521048
7430000 0.0520918
7440000 0.0520869
7450000 0.052093
7460000 0.0520824
7470000 0.0520864
7480000 0.0520815
7490000 0.0520724
7500000 0.052054
7510000 0.0520614
7520000 0.0520534
7530000 0.0520364
7540000 0.0520318
7550000 0.0520155
7560000 0.0520002
7570000 0.0519908
7580000 0.0519934
7590000 0.0519859
7600000 0.0519735
7610000 0.0519762
7620000 0.0519629
7630000 0.0519495
7640000 0.051948
7650000 0.0519421
7660000 0.0519329
7670000 0.0519382
7680000 0.0519255
7690000 0.0519104
7700000 0.0519166
7710000 0.0518992
7720000 0.0518944
7730000 0.0518921
7740000 0.0518812
7750000 0.0518719
7760000 0.0518707
7770000 0.0518694
7780000 0.0518786
7790000 0.0518658
7800000 0.0518608
7810000 0.0518412
7820000 0.0518281
7830000 0.0518234
7840000 0.0518027
7850000 0.0518095
7860000 0.0518194
7870000 0.0518002
7880000 0.0517796
7890000 0.0517588
7900000 0.0517594
7910000 0.0517618
7920000 0.0517437
7930000 0.0517519
7940000 0.0517485
7950000 0.0517384
7960000 0.051733
7970000 0.0517467
7980000 0.0517479
7990000 0.051737
8000000 0.0517119
8010000 0.0516989
8020000 0.0517054
8030000 0.0517007
8040000 0.051691
8050000 0.051683
8060000 0.0516751
8070000 0.0516633
8080000 0.0516824
8090000 0.0516806
8100000 0.0516685
8110000 0.0516571
8120000 0.0516563
8130000 0.0516407
8140000 0.0516244
8150000 0.051627
8160000 0.051625
8170000 0.0516152
8180000 0.0516102
8190000 0.0516053
8200000 0.0515978
8210000 0.0516026
8220000 0.0515908
8230000 0.0515834
8240000 0.0516252
8250000 0.0516251
8260000 0.0516169
8270000 0.0516121
8280000 0.0516079
8290000 0.051599
8300000 0.05159
8310000 0.0515888
8320000 0.0515915
8330000 0.0515895
8340000 0.0515753
8350000 0.0515689
8360000 0.0515382
8370000 0.0515211
8380000 0.0515063
8390000 0.0514936
8400000 0.0514894
8410000 0.0514825
8420000 0.0514826
8430000 0.0514715
8440000 0.0514644
8450000 0.051458
8460000 0.0514472
8470000 0.0514326
8480000 0.0514402
8490000 0.05143
8500000 0.0514141
8510000 0.0514231
8520000 0.0514123
8530000 0.0514003
8540000 0.0513989
8550000 0.0513961
8560000 0.0513868
8570000 0.05138
8580000 0.0513804
8590000 0.0513674
8600000 0.0513545
8610000 0.051336
8620000 0.0513328
8630000 0.0513403
8640000 0.0513203
8650000 0.0513341
8660000 0.0513446
8670000 0.0513388
8680000 0.0513125
8690000 0.0513067
8700000 0.0513021
8710000 0.0512881
8720000 0.0512738
8730000 0.0512782
8740000 0.0512589
8750000 0.0512568
8760000 0.0512507
8770000 0.0512485
8780000 0.0512275
8790000 0.0512282
8800000 0.0512306
8810000 0.0512294
8820000 0.0512289
8830000 0.0512157
8840000 0.0511958
8850000 0.051187
8860000 0.051178
8870000 0.0511644
8880000 0.0511488
8890000 0.0511332
8900000 0.0511379
8910000 0.051125
8920000 0.0511171
8930000 0.0511249
8940000 0.051126
8950000 0.0511246
8960000 0.0511177
8970000 0.051102
8980000 0.0510876
8990000 0.0510844
9000000 0.0510767
9010000 0.0510873
9020000 0.0510748
9030000 0.0510609
9040000 0.0510491
9050000 0.051048
9060000 0.0510268
9070000 0.0510301
9080000 0.0510265
9090000 0.0510082
9100000 0.0514248
9110000 0.0514101
9120000 0.0514028
9130000 0.051401
9140000 0.051386
9150000 0.0513651
9160000 0.0513565
9170000 0.0513464
9180000 0.0513391
9190000 0.0513402
9200000 0.051331
9210000 0.0513257
9220000 0.0513218
9230000 0.051319
9240000 0.0513141
9250000 0.0513145
9260000 0.0513113
9270000 0.0512978
9280000 0.0512923
9290000 0.0512843
9300000 0.051276
9310000 0.0512699
9320000 0.0512586
9330000 0.0512415
9340000 0.05125
9350000 0.051245
9360000 0.051239
9370000 0.0512364
9380000 0.0512306
9390000 0.0512287
9400000 0.0512224
9410000 0.0512095
9420000 0.0512081
9430000 0.0512167
9440000 0.0512256
9450000 0.0512357
9460000 0.0512177
9470000 0.0512118
9480000 0.0512105
9490000 0.0511979
9500000 0.0511831
9510000 0.0511727
9520000 0.0511732
9530000 0.0511576
9540000 0.0511493
9550000 0.0511407
9560000 0.0511387
9570000 0.0511268
9580000 0.0511137
9590000 0.0511032
9600000 0.051097
9610000 0.0510921
9620000 0.0510832
9630000 0.0510704
9640000 0.0510599
9650000 0.0510474
9660000 0.0510339
9670000 0.0510384
9680000 0.0510341
9690000 0.0510248
9700000 0.0510326
9710000 0.0510206
9720000 0.0510161
9730000 0.0510125
9740000 0.0510115
9750000 0.0510061
9760000 0.0509956
9770000 0.0509938
9780000 0.0509853
9790000 0.0509738
9800000 0.0509778
9810000 0.0510597
9820000 0.0510497
9830000 0.0510471
9840000 0.0510467
9850000 0.0510515
9860000 0.0510546
9870000 0.0510475
9880000 0.0510417
9890000 0.0510435
9900000 0.0510275
9910000 0.0510181
9920000 0.0510151
9930000 0.0510058
9940000 0.05101
9950000 0.0510067
9960000 0.0509988
9970000 0.0509957
9980000 0.0509983
9990000 0.0510016
10000000 0.0509934


==> Figures/2DResults/Interior/NeumannBackward.tex <==
10000 0.938872
20000 0.677092
30000 0.557056
40000 0.491679
50000 0.448096
60000 0.419332
70000 0.392622
80000 0.373315
90000 0.35741
100000 0.343107
110000 0.33153
120000 0.322939
130000 0.313959
140000 0.307064
150000 0.300279
160000 0.294422
170000 0.288001
180000 0.282867
190000 0.278838
200000 0.275976
210000 0.272771
220000 0.269256
230000 0.26584
240000 0.262333
250000 0.259461
260000 0.256595
270000 0.25399
280000 0.251302
290000 0.248962
300000 0.246581
310000 0.244492
320000 0.242988
330000 0.241463
340000 0.239479
350000 0.237511
360000 0.236087
370000 0.23485
380000 0.233707
390000 0.232428
400000 0.230697
410000 0.229687
420000 0.22885
430000 0.227937
440000 0.227402
450000 0.226665
460000 0.224894
470000 0.223762
480000 0.222879
490000 0.222222
500000 0.221539
510000 0.220935
520000 0.220046
530000 0.218952
540000 0.218198
550000 0.217558
560000 0.216829
570000 0.216049
580000 0.215523
590000 0.214679
600000 0.213914
610000 0.213271
620000 0.212818
630000 0.212325
640000 0.211912
650000 0.211512
660000 0.211143
670000 0.211016
680000 0.210591
690000 0.21043
700000 0.209693
710000 0.209432
720000 0.209158
730000 0.209241
740000 0.208797
750000 0.208577
760000 0.207747
770000 0.207443
780000 0.20703
790000 0.206873
800000 0.206363
810000 0.206224
820000 0.20593
830000 0.205627
840000 0.205219
850000 0.20529
860000 0.205075
870000 0.204744
880000 0.204459
890000 0.20417
900000 0.204064
910000 0.20394
920000 0.203716
930000 0.203517
940000 0.203212
950000 0.202993
960000 0.202684
970000 0.202812
980000 0.202664
990000 0.202239
1000000 0.201731
1010000 0.201539
1020000 0.201388
1030000 0.201343
1040000 0.201148
1050000 0.2009
1060000 0.200789
1070000 0.200501
1080000 0.200467
1090000 0.200679
1100000 0.20038
1110000 0.200215
1120000 0.200027
1130000 0.199863
1140000 0.199904
1150000 0.199719
1160000 0.199518
1170000 0.199445
1180000 0.199323
1190000 0.199005
1200000 0.198915
1210000 0.198868
1220000 0.198767
1230000 0.198545
1240000 0.198342
1250000 0.198286
1260000 0.198197
1270000 0.198053
1280000 0.197903
1290000 0.197698
1300000 0.197443
1310000 0.197308
1320000 0.197243
1330000 0.197125
1340000 0.197044
1350000 0.196932
1360000 0.196793
1370000 0.196759
1380000 0.196795
1390000 0.196696
1400000 0.196672
1410000 0.196527
1420000 0.196358
1430000 0.196242
1440000 0.196186
1450000 0.196163
1460000 0.196133
1470000 0.19583
1480000 0.195723
1490000 0.195478
1500000 0.19543
1510000 0.195356
1520000 0.195288
1530000 0.19511
1540000 0.194959
1550000 0.194721
1560000 0.19464
1570000 0.194525
1580000 0.194485
1590000 0.194337
1600000 0.194232
1610000 0.194101
1620000 0.19428
1630000 0.194271
1640000 0.194141
1650000 0.193978
1660000 0.193857
1670000 0.193821
1680000 0.19383
1690000 0.193753
1700000 0.193649
1710000 0.193514
1720000 0.193484
1730000 0.193396
1740000 0.193326
1750000 0.193266
1760000 0.193201
1770000 0.193094
1780000 0.193023
1790000 0.193019
1800000 0.192968
1810000 0.192892
1820000 0.192836
1830000 0.192699
1840000 0.192571
1850000 0.192478
1860000 0.192506
1870000 0.192486
1880000 0.192382
1890000 0.192283
1900000 0.192239
1910000 0.19221
1920000 0.192191
1930000 0.192214
1940000 0.192136
1950000 0.192073
1960000 0.191982
1970000 0.191973
1980000 0.191961
1990000 0.191885
2000000 0.191767
2010000 0.191578
2020000 0.191447
2030000 0.191568
2040000 0.191583
2050000 0.191517
2060000 0.191424
2070000 0.191326
2080000 0.191322
2090000 0.191408
2100000 0.191308
2110000 0.191237
2120000 0.191119
2130000 0.190968
2140000 0.19092
2150000 0.190922
2160000 0.190951
2170000 0.190959
2180000 0.190772
2190000 0.190731
2200000 0.190639
2210000 0.190605
2220000 0.19061
2230000 0.190531
2240000 0.190425
2250000 0.190344
2260000 0.190229
2270000 0.190181
2280000 0.190143
2290000 0.190141
2300000 0.190087
2310000 0.190017
2320000 0.189971
2330000 0.189966
2340000 0.189918
2350000 0.189876
2360000 0.189813
2370000 0.18973
2380000 0.18964
2390000 0.189661
2400000 0.189629
2410000 0.189603
2420000 0.189439
2430000 0.189362
2440000 0.189336
2450000 0.189322
2460000 0.189319
2470000 0.189274
2480000 0.18922
2490000 0.189225
2500000 0.189129
2510000 0.189167
2520000 0.189101
2530000 0.1891
2540000 0.188992
2550000 0.188866
2560000 0.188806
2570000 0.188883
2580000 0.188855
2590000 0.188783
2600000 0.18872
2610000 0.188715
2620000 0.188674
2630000 0.188689
2640000 0.18864
2650000 0.188609
2660000 0.188531
2670000 0.188505
2680000 0.188494
2690000 0.188501
2700000 0.188506
2710000 0.188397
2720000 0.188352
2730000 0.188304
2740000 0.188298
2750000 0.188304
2760000 0.188258
2770000 0.188137
2780000 0.188093
2790000 0.188107
2800000 0.188079
2810000 0.188099
2820000 0.18815
2830000 0.188086
2840000 0.188078
2850000 0.188033
2860000 0.188035
2870000 0.188028
2880000 0.188021
2890000 0.187935
2900000 0.187876
2910000 0.187883
2920000 0.187913
2930000 0.18794
2940000 0.187961
2950000 0.187856
2960000 0.187821
2970000 0.187828
2980000 0.187809
2990000 0.187834
3000000 0.187861
3010000 0.187785
3020000 0.187699
3030000 0.187649
3040000 0.187726
3050000 0.187739
3060000 0.187784
3070000 0.18771
3080000 0.187669
3090000 0.187641
3100000 0.187709
3110000 0.187677
3120000 0.18771
3130000 0.187618
3140000 0.187576
3150000 0.187572
3160000 0.187601
3170000 0.187571
3180000 0.187587
3190000 0.187462
3200000 0.187437
3210000 0.187397
3220000 0.187453
3230000 0.187501
3240000 0.187477
3250000 0.187475
3260000 0.187422
3270000 0.18739
3280000 0.187404
3290000 0.187375
3300000 0.187385
3310000 0.187289
3320000 0.187347
3330000 0.187319
3340000 0.187269
3350000 0.187228
3360000 0.187216
3370000 0.187124
3380000 0.187104
3390000 0.187125
3400000 0.187152
3410000 0.187159
3420000 0.187112
3430000 0.18702
3440000 0.186973
3450000 0.187004
3460000 0.186995
3470000 0.186994
3480000 0.186966
3490000 0.186889
3500000 0.186849
3510000 0.186842
3520000 0.186846
3530000 0.186812
3540000 0.186779
3550000 0.186741
3560000 0.186736
3570000 0.186723
3580000 0.186747
3590000 0.186757
3600000 0.186782
3610000 0.186727
3620000 0.186709
3630000 0.186701
3640000 0.186721
3650000 0.186661
3660000 0.186632
3670000 0.186581
3680000 0.186576
3690000 0.1866
3700000 0.186594
3710000 0.186621
3720000 0.186555
3730000 0.186504
3740000 0.186526
3750000 0.186518
3760000 0.186588
3770000 0.186585
3780000 0.186566
3790000 0.18652
3800000 0.186496
3810000 0.186464
3820000 0.186516
3830000 0.186562
3840000 0.186534
3850000 0.186476
3860000 0.186462
3870000 0.186467
3880000 0.186455
3890000 0.186458
3900000 0.186397
3910000 0.186374
3920000 0.186347
3930000 0.186387
3940000 0.186356
3950000 0.186377
3960000 0.186375
3970000 0.186353
3980000 0.186334
3990000 0.186375
4000000 0.186339
4010000 0.186299
4020000 0.186273
4030000 0.186247
4040000 0.186227
4050000 0.186271
4060000 0.186252
4070000 0.18626
4080000 0.186207
4090000 0.186163
4100000 0.18613
4110000 0.186162
4120000 0.186172
4130000 0.186134
4140000 0.186042
4150000 0.186019
4160000 0.18602
4170000 0.186071
4180000 0.186078
4190000 0.186059
4200000 0.186046
4210000 0.186021
4220000 0.186017
4230000 0.185998
4240000 0.18599
4250000 0.185964
4260000 0.185909
4270000 0.185932
4280000 0.185962
4290000 0.185968
4300000 0.185948
4310000 0.185969
4320000 0.185944
4330000 0.185932
4340000 0.185932
4350000 0.185924
4360000 0.185881
4370000 0.185844
4380000 0.185833
4390000 0.185837
4400000 0.185842
4410000 0.185848
4420000 0.185878
4430000 0.185878
4440000 0.185836
4450000 0.185799
4460000 0.185798
4470000 0.185813
4480000 0.185806
4490000 0.185781
4500000 0.185737
4510000 0.185741
4520000 0.185784
4530000 0.185796
4540000 0.185785
4550000 0.185765
4560000 0.18577
4570000 0.185734
4580000 0.185755
4590000 0.185738
4600000 0.185734
4610000 0.185714
4620000 0.185687
4630000 0.185693
4640000 0.185698
4650000 0.185711
4660000 0.185717
4670000 0.185721
4680000 0.1857
4690000 0.185647
4700000 0.185681
4710000 0.185648
4720000 0.185626
4730000 0.185587
4740000 0.185562
4750000 0.185507
4760000 0.185581
4770000 0.185598
4780000 0.185603
4790000 0.185588
4800000 0.185573
4810000 0.185584
4820000 0.185585
4830000 0.185553
4840000 0.185547
4850000 0.18553
4860000 0.185526
4870000 0.185487
4880000 0.185509
4890000 0.185485
4900000 0.185488
4910000 0.185467
4920000 0.185416
4930000 0.185424
4940000 0.185467
4950000 0.185446
4960000 0.185458
4970000 0.185375
4980000 0.185354
4990000 0.185331
5000000 0.18538
5010000 0.18539
5020000 0.185371
5030000 0.185367
5040000 0.185319
5050000 0.185303
5060000 0.185306
5070000 0.18532
5080000 0.185328
5090000 0.185303
5100000 0.185285
5110000 0.185273
5120000 0.18528
5130000 0.185269
5140000 0.185237
5150000 0.185219
5160000 0.185202
5170000 0.185194
5180000 0.185217
5190000 0.185212
5200000 0.185186
5210000 0.185166
5220000 0.185163
5230000 0.185188
5240000 0.185196
5250000 0.185204
5260000 0.185177
5270000 0.185117
5280000 0.185109
5290000 0.18513
5300000 0.185185
5310000 0.185193
5320000 0.185164
5330000 0.185161
5340000 0.185167
5350000 0.185186
5360000 0.185197
5370000 0.185194
5380000 0.185188
5390000 0.18519
5400000 0.185146
5410000 0.185152
5420000 0.185164
5430000 0.185179
5440000 0.185135
5450000 0.18512
5460000 0.185105
5470000 0.185118
5480000 0.18516
5490000 0.185159
5500000 0.185128
5510000 0.185106
5520000 0.185091
5530000 0.185092
5540000 0.18509
5550000 0.185084
5560000 0.185068
5570000 0.185041
5580000 0.185041
5590000 0.185077
5600000 0.185087
5610000 0.185081
5620000 0.18505
5630000 0.185062
5640000 0.185058
5650000 0.185068
5660000 0.185066
5670000 0.185046
5680000 0.184999
5690000 0.184989
5700000 0.184968
5710000 0.18499
5720000 0.184987
5730000 0.184961
5740000 0.184931
5750000 0.184931
5760000 0.184946
5770000 0.184978
5780000 0.184964
5790000 0.184995
5800000 0.184953
5810000 0.184917
5820000 0.184903
5830000 0.184929
5840000 0.184907
5850000 0.184903
5860000 0.184902
5870000 0.184903
5880000 0.184897
5890000 0.18491
5900000 0.184878
5910000 0.184871
5920000 0.184872
5930000 0.184892
5940000 0.184877
5950000 0.184854
5960000 0.184834
5970000 0.184827
5980000 0.184826
5990000 0.1848
6000000 0.184788
6010000 0.184781
6020000 0.184792
6030000 0.184788
6040000 0.184753
6050000 0.184776
6060000 0.184807
6070000 0.184826
6080000 0.18481
6090000 0.184786
6100000 0.184781
6110000 0.184798
6120000 0.184791
6130000 0.184785
6140000 0.184769
6150000 0.184752
6160000 0.184753
6170000 0.184708
6180000 0.184715
6190000 0.184736
6200000 0.184727
6210000 0.184699
6220000 0.184666
6230000 0.184633
6240000 0.184667
6250000 0.184655
6260000 0.184673
6270000 0.184664
6280000 0.184662
6290000 0.184661
6300000 0.184657
6310000 0.184653
6320000 0.184658
6330000 0.184634
6340000 0.184604
6350000 0.184603
6360000 0.184621
6370000 0.18464
6380000 0.184628
6390000 0.18462
6400000 0.184619
6410000 0.184593
6420000 0.184608
6430000 0.184612
6440000 0.18462
6450000 0.184616
6460000 0.184632
6470000 0.184614
6480000 0.184631
6490000 0.184633
6500000 0.184674
6510000 0.184676
6520000 0.184659
6530000 0.184644
6540000 0.18468
6550000 0.184716
6560000 0.184698
6570000 0.184683
6580000 0.184666
6590000 0.184686
6600000 0.184707
6610000 0.184731
6620000 0.184732
6630000 0.184698
6640000 0.18471
6650000 0.184699
6660000 0.184731
6670000 0.184737
6680000 0.18469
6690000 0.184652
6700000 0.184641
6710000 0.184622
6720000 0.184642
6730000 0.184633
6740000 0.1846
6750000 0.184555
6760000 0.184552
6770000 0.184582
6780000 0.184578
6790000 0.184602
6800000 0.184603
6810000 0.184584
6820000 0.184563
6830000 0.184539
6840000 0.184552
6850000 0.184548
6860000 0.184538
6870000 0.184539
6880000 0.184558
6890000 0.184587
6900000 0.184591
6910000 0.184591
6920000 0.184554
6930000 0.184534
6940000 0.184534
6950000 0.184546
6960000 0.184541
6970000 0.184567
6980000 0.184552
6990000 0.184537
7000000 0.18453
7010000 0.184555
7020000 0.184552
7030000 0.184534
7040000 0.18449
7050000 0.184504
7060000 0.184498
7070000 0.184497
7080000 0.184491
7090000 0.184484
7100000 0.184468
7110000 0.184436
7120000 0.184432
7130000 0.184443
7140000 0.18444
7150000 0.184445
7160000 0.184425
7170000 0.184432
7180000 0.184428
7190000 0.184412
7200000 0.184413
7210000 0.18438
7220000 0.18436
7230000 0.184338
7240000 0.184329
7250000 0.184339
7260000 0.184355
7270000 0.184371
7280000 0.184331
7290000 0.184292
7300000 0.184293
7310000 0.184293
7320000 0.184293
7330000 0.184279
7340000 0.184271
7350000 0.184234
7360000 0.184225
7370000 0.184241
7380000 0.18426
7390000 0.184238
7400000 0.184239
7410000 0.184224
7420000 0.184234
7430000 0.184239
7440000 0.184271
7450000 0.184268
7460000 0.184253
7470000 0.184271
7480000 0.184269
7490000 0.184284
7500000 0.184295
7510000 0.1843
7520000 0.184306
7530000 0.18431
7540000 0.184318
7550000 0.184326
7560000 0.184309
7570000 0.184282
7580000 0.184258
7590000 0.184254
7600000 0.184247
7610000 0.184241
7620000 0.184244
7630000 0.184232
7640000 0.184206
7650000 0.184188
7660000 0.18419
7670000 0.184188
7680000 0.184197
7690000 0.184176
7700000 0.184161
7710000 0.184158
7720000 0.184184
7730000 0.184184
7740000 0.184202
7750000 0.184189
7760000 0.184191
7770000 0.184151
7780000 0.184156
7790000 0.184168
7800000 0.184164
7810000 0.184144
7820000 0.184131
7830000 0.184117
7840000 0.184148
7850000 0.184155
7860000 0.184156
7870000 0.184149
7880000 0.18415
7890000 0.184148
7900000 0.184157
7910000 0.184172
7920000 0.184202
7930000 0.184171
7940000 0.184146
7950000 0.184147
7960000 0.184151
7970000 0.184137
7980000 0.184149
7990000 0.184124
8000000 0.184112
8010000 0.184111
8020000 0.184117
8030000 0.18412
8040000 0.184119
8050000 0.184073
8060000 0.184062
8070000 0.18404
8080000 0.184049
8090000 0.184055
8100000 0.184054
8110000 0.184043
8120000 0.184045
8130000 0.184067
8140000 0.184081
8150000 0.184096
8160000 0.184064
8170000 0.184044
8180000 0.184018
8190000 0.183999
8200000 0.184
8210000 0.184016
8220000 0.184024
8230000 0.183995
8240000 0.183985
8250000 0.183991
8260000 0.183998
8270000 0.183998
8280000 0.183986
8290000 0.183966
8300000 0.183948
8310000 0.183983
8320000 0.18401
8330000 0.18402
8340000 0.184021
8350000 0.184009
8360000 0.183982
8370000 0.183979
8380000 0.183998
8390000 0.184016
8400000 0.184013
8410000 0.183979
8420000 0.183984
8430000 0.184
8440000 0.184002
8450000 0.18401
8460000 0.184006
8470000 0.183988
8480000 0.18399
8490000 0.183995
8500000 0.183999
8510000 0.183965
8520000 0.183974
8530000 0.183951
8540000 0.183956
8550000 0.183979
8560000 0.183963
8570000 0.18397
8580000 0.18395
8590000 0.183935
8600000 0.183932
8610000 0.183932
8620000 0.183933
8630000 0.183941
8640000 0.183922
8650000 0.183908
8660000 0.183886
8670000 0.183891
8680000 0.183901
8690000 0.183908
8700000 0.183896
8710000 0.183883
8720000 0.183866
8730000 0.183872
8740000 0.183878
8750000 0.183884
8760000 0.183864
8770000 0.183857
8780000 0.183864
8790000 0.183869
8800000 0.183866
8810000 0.183873
8820000 0.183851
8830000 0.183848
8840000 0.183862
8850000 0.183873
8860000 0.183877
8870000 0.183876
8880000 0.183863
8890000 0.183856
8900000 0.183852
8910000 0.183874
8920000 0.183887
8930000 0.183886
8940000 0.183858
8950000 0.183841
8960000 0.18386
8970000 0.183845
8980000 0.183836
8990000 0.183828
9000000 0.183797
9010000 0.183784
9020000 0.183793
9030000 0.183801
9040000 0.183803
9050000 0.183785
9060000 0.183778
9070000 0.183763
9080000 0.183786
9090000 0.183804
9100000 0.183823
9110000 0.18381
9120000 0.183796
9130000 0.183782
9140000 0.183796
9150000 0.183813
9160000 0.183797
9170000 0.183782
9180000 0.18378
9190000 0.183786
9200000 0.183802
9210000 0.183818
9220000 0.183839
9230000 0.183835
9240000 0.183806
9250000 0.183792
9260000 0.183805
9270000 0.183829
9280000 0.183823
9290000 0.183823
9300000 0.183825
9310000 0.183812
9320000 0.18383
9330000 0.183828
9340000 0.183848
9350000 0.183843
9360000 0.183838
9370000 0.183829
9380000 0.18382
9390000 0.183813
9400000 0.183803
9410000 0.183786
9420000 0.183785
9430000 0.183774
9440000 0.183775
9450000 0.183782
9460000 0.183787
9470000 0.183768
9480000 0.183788
9490000 0.183773
9500000 0.183799
9510000 0.183818
9520000 0.183826
9530000 0.183822
9540000 0.18382
9550000 0.183822
9560000 0.183842
9570000 0.183862
9580000 0.183855
9590000 0.183814
9600000 0.18382
9610000 0.183802
9620000 0.183809
9630000 0.183824
9640000 0.183816
9650000 0.183789
9660000 0.183772
9670000 0.183773
9680000 0.18378
9690000 0.18379
9700000 0.18379
9710000 0.183781
9720000 0.18378
9730000 0.183776
9740000 0.183785
9750000 0.18379
9760000 0.183781
9770000 0.183768
9780000 0.183769
9790000 0.183777
9800000 0.183808
9810000 0.183817
9820000 0.183813
9830000 0.1838
9840000 0.183784
9850000 0.183797
9860000 0.18379
9870000 0.183799
9880000 0.183772
9890000 0.183764
9900000 0.183747
9910000 0.183763
9920000 0.18378
9930000 0.183784
9940000 0.183761
9950000 0.183746
9960000 0.183742
9970000 0.183734
9980000 0.183738
9990000 0.183743
10000000 0.183722


==> Figures/2DResults/Interior/NeumannForward.tex <==
10000 0.615625
20000 0.445476
30000 0.385294
40000 0.344087
50000 0.326825
60000 0.308665
70000 0.29458
80000 0.285428
90000 0.275499
100000 0.26785
110000 0.262258
120000 0.257164
130000 0.254196
140000 0.253317
150000 0.249505
160000 0.246855
170000 0.244685
180000 0.239515
190000 0.237009
200000 0.234463
210000 0.232135
220000 0.233218
230000 0.231964
240000 0.230724
250000 0.229766
260000 0.227284
270000 0.225973
280000 0.224793
290000 0.22346
300000 0.223377
310000 0.223697
320000 0.222964
330000 0.222282
340000 0.221555
350000 0.219429
360000 0.218915
370000 0.218101
380000 0.21741
390000 0.218535
400000 0.21824
410000 0.217446
420000 0.217204
430000 0.215576
440000 0.214939
450000 0.214086
460000 0.213612
470000 0.214292
480000 0.214643
490000 0.214126
500000 0.21388
510000 0.213607
520000 0.212507
530000 0.212243
540000 0.211669
550000 0.21128
560000 0.211987
570000 0.211503
580000 0.211061
590000 0.211216
600000 0.210097
610000 0.209813
620000 0.209306
630000 0.209151
640000 0.209487
650000 0.209694
660000 0.209552
670000 0.20935
680000 0.209144
690000 0.208292
700000 0.208108
710000 0.207782
720000 0.20757
730000 0.208315
740000 0.207895
750000 0.207736
760000 0.20778
770000 0.206958
780000 0.206808
790000 0.20656
800000 0.20647
810000 0.206853
820000 0.206898
830000 0.206708
840000 0.206666
850000 0.206348
860000 0.205769
870000 0.205648
880000 0.205521
890000 0.205434
900000 0.20587
910000 0.205509
920000 0.205423
930000 0.205317
940000 0.204561
950000 0.204387
960000 0.204144
970000 0.204081
980000 0.2046
990000 0.204614
1000000 0.204557
1010000 0.204492
1020000 0.204277
1030000 0.203876
1040000 0.203813
1050000 0.203878
1060000 0.203808
1070000 0.204303
1080000 0.204068
1090000 0.204087
1100000 0.20406
1110000 0.203429
1120000 0.203404
1130000 0.203309
1140000 0.203173
1150000 0.203637
1160000 0.203557
1170000 0.203431
1180000 0.203425
1190000 0.203126
1200000 0.202815
1210000 0.202648
1220000 0.202669
1230000 0.202654
1240000 0.203114
1250000 0.202917
1260000 0.20295
1270000 0.203054
1280000 0.202533
1290000 0.202454
1300000 0.202249
1310000 0.202162
1320000 0.202607
1330000 0.202622
1340000 0.202528
1350000 0.20258
1360000 0.202304
1370000 0.202168
1380000 0.202022
1390000 0.202068
1400000 0.202194
1410000 0.202441
1420000 0.202279
1430000 0.202302
1440000 0.202278
1450000 0.201833
1460000 0.201909
1470000 0.201817
1480000 0.201796
1490000 0.202092
1500000 0.202053
1510000 0.201979
1520000 0.202006
1530000 0.201741
1540000 0.20159
1550000 0.201409
1560000 0.201343
1570000 0.201511
1580000 0.201705
1590000 0.201579
1600000 0.201493
1610000 0.20141
1620000 0.201136
1630000 0.201139
1640000 0.201037
1650000 0.200929
1660000 0.201282
1670000 0.201274
1680000 0.201187
1690000 0.201295
1700000 0.201013
1710000 0.200915
1720000 0.200782
1730000 0.2007
1740000 0.200972
1750000 0.201074
1760000 0.201043
1770000 0.200967
1780000 0.200921
1790000 0.200654
1800000 0.200639
1810000 0.200537
1820000 0.200442
1830000 0.200771
1840000 0.200737
1850000 0.200705
1860000 0.200797
1870000 0.200492
1880000 0.200423
1890000 0.200318
1900000 0.200258
1910000 0.200433
1920000 0.200578
1930000 0.200501
1940000 0.200508
1950000 0.20041
1960000 0.200189
1970000 0.200196
1980000 0.200156
1990000 0.200082
2000000 0.200395
2010000 0.200292
2020000 0.200316
2030000 0.200316
2040000 0.199968
2050000 0.199955
2060000 0.199853
2070000 0.199863
2080000 0.200096
2090000 0.200132
2100000 0.200098
2110000 0.200167
2120000 0.200036
2130000 0.199802
2140000 0.199816
2150000 0.19976
2160000 0.199697
2170000 0.199962
2180000 0.199867
2190000 0.199898
2200000 0.199916
2210000 0.199622
2220000 0.199602
2230000 0.199486
2240000 0.1995
2250000 0.199744
2260000 0.199728
2270000 0.199649
2280000 0.199723
2290000 0.199569
2300000 0.199421
2310000 0.199391
2320000 0.199417
2330000 0.199434
2340000 0.199686
2350000 0.199581
2360000 0.199538
2370000 0.199531
2380000 0.199291
2390000 0.199286
2400000 0.199234
2410000 0.199194
2420000 0.199457
2430000 0.199488
2440000 0.199407
2450000 0.199413
2460000 0.199271
2470000 0.199147
2480000 0.199089
2490000 0.199106
2500000 0.199156
2510000 0.199344
2520000 0.199265
2530000 0.199318
2540000 0.199379
2550000 0.199125
2560000 0.199137
2570000 0.199044
2580000 0.19901
2590000 0.199221
2600000 0.199229
2610000 0.199195
2620000 0.199218
2630000 0.199092
2640000 0.198988
2650000 0.198938
2660000 0.198918
2670000 0.199064
2680000 0.199201
2690000 0.199124
2700000 0.199137
2710000 0.199177
2720000 0.198974
2730000 0.199032
2740000 0.19898
2750000 0.198935
2760000 0.19915
2770000 0.199136
2780000 0.199092
2790000 0.19914
2800000 0.198948
2810000 0.198888
2820000 0.198837
2830000 0.198822
2840000 0.198973
2850000 0.199072
2860000 0.199036
2870000 0.199049
2880000 0.199005
2890000 0.198854
2900000 0.198875
2910000 0.198829
2920000 0.198785
2930000 0.198997
2940000 0.198958
2950000 0.19893
2960000 0.199027
2970000 0.198815
2980000 0.198812
2990000 0.198765
3000000 0.198763
3010000 0.198947
3020000 0.199014
3030000 0.198964
3040000 0.198964
3050000 0.198955
3060000 0.198797
3070000 0.198792
3080000 0.198785
3090000 0.198777
3100000 0.198966
3110000 0.198896
3120000 0.198893
3130000 0.198949
3140000 0.19875
3150000 0.198696
3160000 0.198623
3170000 0.198595
3180000 0.198734
3190000 0.198804
3200000 0.198738
3210000 0.198751
3220000 0.198685
3230000 0.198566
3240000 0.198543
3250000 0.198539
3260000 0.198485
3270000 0.198675
3280000 0.198591
3290000 0.198584
3300000 0.198633
3310000 0.198446
3320000 0.198438
3330000 0.198367
3340000 0.198347
3350000 0.198514
3360000 0.198584
3370000 0.198536
3380000 0.198551
3390000 0.19849
3400000 0.198382
3410000 0.19836
3420000 0.198343
3430000 0.198319
3440000 0.198488
3450000 0.198463
3460000 0.198492
3470000 0.198523
3480000 0.198337
3490000 0.19836
3500000 0.198298
3510000 0.198262
3520000 0.198433
3530000 0.198456
3540000 0.198434
3550000 0.198486
3560000 0.198389
3570000 0.198303
3580000 0.198264
3590000 0.198268
3600000 0.198269
3610000 0.198411
3620000 0.198321
3630000 0.198368
3640000 0.198409
3650000 0.198237
3660000 0.198246
3670000 0.198185
3680000 0.198134
3690000 0.198284
3700000 0.198302
3710000 0.198256
3720000 0.198293
3730000 0.198181
3740000 0.198129
3750000 0.198052
3760000 0.198035
3770000 0.198104
3780000 0.198224
3790000 0.198176
3800000 0.198206
3810000 0.198222
3820000 0.198106
3830000 0.198151
3840000 0.19811
3850000 0.198103
3860000 0.19828
3870000 0.198268
3880000 0.198259
3890000 0.198317
3900000 0.198196
3910000 0.198184
3920000 0.198132
3930000 0.198102
3940000 0.19819
3950000 0.198271
3960000 0.198223
3970000 0.198233
3980000 0.198209
3990000 0.198075
4000000 0.198068
4010000 0.198039
4020000 0.19802
4030000 0.198169
4040000 0.198167
4050000 0.1981
4060000 0.198149
4070000 0.198018
4080000 0.197992
4090000 0.197937
4100000 0.197906
4110000 0.19802
4120000 0.198052
4130000 0.198061
4140000 0.19804
4150000 0.198024
4160000 0.197886
4170000 0.19788
4180000 0.197867
4190000 0.197869
4200000 0.198008
4210000 0.197988
4220000 0.197958
4230000 0.198007
4240000 0.197876
4250000 0.197858
4260000 0.197817
4270000 0.197803
4280000 0.197922
4290000 0.197951
4300000 0.197938
4310000 0.197923
4320000 0.197894
4330000 0.197811
4340000 0.197793
4350000 0.19779
4360000 0.197753
4370000 0.197919
4380000 0.197858
4390000 0.197831
4400000 0.197847
4410000 0.197716
4420000 0.197715
4430000 0.197694
4440000 0.197697
4450000 0.197805
4460000 0.19782
4470000 0.197791
4480000 0.197785
4490000 0.197707
4500000 0.19762
4510000 0.197634
4520000 0.19763
4530000 0.197613
4540000 0.197741
4550000 0.197684
4560000 0.197702
4570000 0.197735
4580000 0.197595
4590000 0.197585
4600000 0.197559
4610000 0.197539
4620000 0.19767
4630000 0.197668
4640000 0.19764
4650000 0.197643
4660000 0.197592
4670000 0.197527
4680000 0.197497
4690000 0.197513
4700000 0.197532
4710000 0.197634
4720000 0.197602
4730000 0.197602
4740000 0.197631
4750000 0.197517
4760000 0.1975
4770000 0.197463
4780000 0.197423
4790000 0.197543
4800000 0.197554
4810000 0.197541
4820000 0.197551
4830000 0.197469
4840000 0.19741
4850000 0.19738
4860000 0.197383
4870000 0.197411
4880000 0.197488
4890000 0.197445
4900000 0.197459
4910000 0.197481
4920000 0.197341
4930000 0.197349
4940000 0.197314
4950000 0.197299
4960000 0.197418
4970000 0.197421
4980000 0.197399
4990000 0.197423
5000000 0.197337
5010000 0.1973
5020000 0.197279
5030000 0.197269
5040000 0.197315
5050000 0.197376
5060000 0.197373
5070000 0.197345
5080000 0.197337
5090000 0.197236
5100000 0.197255
5110000 0.197214
5120000 0.197201
5130000 0.197333
5140000 0.197324
5150000 0.197302
5160000 0.19733
5170000 0.197218
5180000 0.197194
5190000 0.197175
5200000 0.197168
5210000 0.197237
5220000 0.197277
5230000 0.197279
5240000 0.197275
5250000 0.197268
5260000 0.197187
5270000 0.197208
5280000 0.197178
5290000 0.197153
5300000 0.197263
5310000 0.197261
5320000 0.197237
5330000 0.197283
5340000 0.197161
5350000 0.197153
5360000 0.19711
5370000 0.197096
5380000 0.197184
5390000 0.197217
5400000 0.197198
5410000 0.197209
5420000 0.197211
5430000 0.197154
5440000 0.197157
5450000 0.197153
5460000 0.197126
5470000 0.197233
5480000 0.197222
5490000 0.19722
5500000 0.197257
5510000 0.197136
5520000 0.197131
5530000 0.197122
5540000 0.19708
5550000 0.197179
5560000 0.197204
5570000 0.197199
5580000 0.197219
5590000 0.197179
5600000 0.197127
5610000 0.197128
5620000 0.197107
5630000 0.197093
5640000 0.197204
5650000 0.197195
5660000 0.197192
5670000 0.197191
5680000 0.197101
5690000 0.197108
5700000 0.197092
5710000 0.197069
5720000 0.197171
5730000 0.197188
5740000 0.197181
5750000 0.197185
5760000 0.197138
5770000 0.197068
5780000 0.197056
5790000 0.197048
5800000 0.197056
5810000 0.19716
5820000 0.197122
5830000 0.197134
5840000 0.197166
5850000 0.197056
5860000 0.197031
5870000 0.197023
5880000 0.197023
5890000 0.197127
5900000 0.197138
5910000 0.197136
5920000 0.19716
5930000 0.197124
5940000 0.197083
5950000 0.197057
5960000 0.197066
5970000 0.197093
5980000 0.197174
5990000 0.197136
6000000 0.197139
6010000 0.19714
6020000 0.197036
6030000 0.197016
6040000 0.196994
6050000 0.196955
6060000 0.197034
6070000 0.197034
6080000 0.197003
6090000 0.197004
6100000 0.196938
6110000 0.196902
6120000 0.196861
6130000 0.196874
6140000 0.196907
6150000 0.19696
6160000 0.196942
6170000 0.196964
6180000 0.196982
6190000 0.196916
6200000 0.196909
6210000 0.196887
6220000 0.196867
6230000 0.196973
6240000 0.196971
6250000 0.196959
6260000 0.196983
6270000 0.196931
6280000 0.196906
6290000 0.196889
6300000 0.19687
6310000 0.196927
6320000 0.196976
6330000 0.196946
6340000 0.196962
6350000 0.196948
6360000 0.19687
6370000 0.19687
6380000 0.196828
6390000 0.19681
6400000 0.196913
6410000 0.196922
6420000 0.196919
6430000 0.196959
6440000 0.196882
6450000 0.196858
6460000 0.196836
6470000 0.196818
6480000 0.19689
6490000 0.196918
6500000 0.196896
6510000 0.196906
6520000 0.196903
6530000 0.196824
6540000 0.196807
6550000 0.196797
6560000 0.196762
6570000 0.196858
6580000 0.196831
6590000 0.196808
6600000 0.196844
6610000 0.196751
6620000 0.196729
6630000 0.196718
6640000 0.196695
6650000 0.196748
6660000 0.196778
6670000 0.196777
6680000 0.196796
6690000 0.196776
6700000 0.196702
6710000 0.196707
6720000 0.196704
6730000 0.196705
6740000 0.196804
6750000 0.196775
6760000 0.196786
6770000 0.196801
6780000 0.196689
6790000 0.196672
6800000 0.196643
6810000 0.19664
6820000 0.196718
6830000 0.196738
6840000 0.196737
6850000 0.196754
6860000 0.196724
6870000 0.196674
6880000 0.196675
6890000 0.196684
6900000 0.196691
6910000 0.196783
6920000 0.196761
6930000 0.196757
6940000 0.196771
6950000 0.196665
6960000 0.196667
6970000 0.196653
6980000 0.196651
6990000 0.196717
7000000 0.196729
7010000 0.196723
7020000 0.196729
7030000 0.196663
7040000 0.196631
7050000 0.196623
7060000 0.196636
7070000 0.196648
7080000 0.196732
7090000 0.196713
7100000 0.196709
7110000 0.196724
7120000 0.196628
7130000 0.196615
7140000 0.196592
7150000 0.196579
7160000 0.196658
7170000 0.196661
7180000 0.196644
7190000 0.19667
7200000 0.196623
7210000 0.196584
7220000 0.196551
7230000 0.196556
7240000 0.196578
7250000 0.196635
7260000 0.196617
7270000 0.196634
7280000 0.196637
7290000 0.196559
7300000 0.19656
7310000 0.19655
7320000 0.196547
7330000 0.196628
7340000 0.196623
7350000 0.196615
7360000 0.19662
7370000 0.196567
7380000 0.196536
7390000 0.196522
7400000 0.196516
7410000 0.196556
7420000 0.196611
7430000 0.196587
7440000 0.196587
7450000 0.196584
7460000 0.196524
7470000 0.196527
7480000 0.196509
7490000 0.196499
7500000 0.196583
7510000 0.196594
7520000 0.196568
7530000 0.196579
7540000 0.196511
7550000 0.196484
7560000 0.196453
7570000 0.196444
7580000 0.196499
7590000 0.196515
7600000 0.196507
7610000 0.196513
7620000 0.196513
7630000 0.196456
7640000 0.196463
7650000 0.196435
7660000 0.196431
7670000 0.196522
7680000 0.196529
7690000 0.196525
7700000 0.196555
7710000 0.196468
7720000 0.196454
7730000 0.196428
7740000 0.196415
7750000 0.196489
7760000 0.196507
7770000 0.196487
7780000 0.196484
7790000 0.196478
7800000 0.196417
7810000 0.196409
7820000 0.19639
7830000 0.196385
7840000 0.196468
7850000 0.196452
7860000 0.196455
7870000 0.196478
7880000 0.196396
7890000 0.196395
7900000 0.196379
7910000 0.196376
7920000 0.196437
7930000 0.196459
7940000 0.196442
7950000 0.196455
7960000 0.196431
7970000 0.196373
7980000 0.196386
7990000 0.196385
8000000 0.196385
8010000 0.196462
8020000 0.196434
8030000 0.196443
8040000 0.196452
8050000 0.196364
8060000 0.196363
8070000 0.196343
8080000 0.19634
8090000 0.19641
8100000 0.196425
8110000 0.196414
8120000 0.19642
8130000 0.196403
8140000 0.196362
8150000 0.196348
8160000 0.196357
8170000 0.196353
8180000 0.196438
8190000 0.196412
8200000 0.196415
8210000 0.196431
8220000 0.196352
8230000 0.196359
8240000 0.196356
8250000 0.196355
8260000 0.196434
8270000 0.196448
8280000 0.196447
8290000 0.196443
8300000 0.196424
8310000 0.196393
8320000 0.196379
8330000 0.196385
8340000 0.196388
8350000 0.196444
8360000 0.196431
8370000 0.196437
8380000 0.196451
8390000 0.19637
8400000 0.196376
8410000 0.196357
8420000 0.19633
8430000 0.196408
8440000 0.196405
8450000 0.19641
8460000 0.196418
8470000 0.196394
8480000 0.196367
8490000 0.196353
8500000 0.19637
8510000 0.196403
8520000 0.196448
8530000 0.19644
8540000 0.196447
8550000 0.196446
8560000 0.196369
8570000 0.196374
8580000 0.196351
8590000 0.196352
8600000 0.196411
8610000 0.196407
8620000 0.1964
8630000 0.19641
8640000 0.196377
8650000 0.196357
8660000 0.196334
8670000 0.196337
8680000 0.196365
8690000 0.196387
8700000 0.196371
8710000 0.196386
8720000 0.196375
8730000 0.196317
8740000 0.196337
8750000 0.196318
8760000 0.196301
8770000 0.196367
8780000 0.19637
8790000 0.196348
8800000 0.196371
8810000 0.19631
8820000 0.196288
8830000 0.196266
8840000 0.196266
8850000 0.196321
8860000 0.196356
8870000 0.196345
8880000 0.196351
8890000 0.196336
8900000 0.196294
8910000 0.196296
8920000 0.196276
8930000 0.196266
8940000 0.196347
8950000 0.196351
8960000 0.19635
8970000 0.196382
8980000 0.196314
8990000 0.196306
9000000 0.196281
9010000 0.196276
9020000 0.196328
9030000 0.196367
9040000 0.196357
9050000 0.196363
9060000 0.196354
9070000 0.19629
9080000 0.196287
9090000 0.196284
9100000 0.196277
9110000 0.196363
9120000 0.196349
9130000 0.196338
9140000 0.196351
9150000 0.196276
9160000 0.196276
9170000 0.196261
9180000 0.196256
9190000 0.196302
9200000 0.19632
9210000 0.196313
9220000 0.196324
9230000 0.196289
9240000 0.196254
9250000 0.196251
9260000 0.196254
9270000 0.19625
9280000 0.196305
9290000 0.196296
9300000 0.196296
9310000 0.196308
9320000 0.196237
9330000 0.196231
9340000 0.196217
9350000 0.19621
9360000 0.196272
9370000 0.196294
9380000 0.196292
9390000 0.196297
9400000 0.196265
9410000 0.196216
9420000 0.196212
9430000 0.196218
9440000 0.196219
9450000 0.196273
9460000 0.196244
9470000 0.19625
9480000 0.196276
9490000 0.19621
9500000 0.196211
9510000 0.196206
9520000 0.1962
9530000 0.196268
9540000 0.196271
9550000 0.196258
9560000 0.196259
9570000 0.196228
9580000 0.196197
9590000 0.196177
9600000 0.196186
9610000 0.196196
9620000 0.196241
9630000 0.196224
9640000 0.19622
9650000 0.196243
9660000 0.196163
9670000 0.196158
9680000 0.196144
9690000 0.196129
9700000 0.196192
9710000 0.196187
9720000 0.196182
9730000 0.196189
9740000 0.196155
9750000 0.196139
9760000 0.196129
9770000 0.196129
9780000 0.196163
9790000 0.196205
9800000 0.196193
9810000 0.196204
9820000 0.196209
9830000 0.196151
9840000 0.196158
9850000 0.196148
9860000 0.196145
9870000 0.196199
9880000 0.196202
9890000 0.196196
9900000 0.196211
9910000 0.196166
9920000 0.196141
9930000 0.196132
9940000 0.196121
9950000 0.196159
9960000 0.196192
9970000 0.196178
9980000 0.196182
9990000 0.196178
10000000 0.196141


==> Figures/2DResults/Interior/Robin.tex <==
10000 0.515928
20000 0.385326
30000 0.302988
40000 0.262614
50000 0.235901
60000 0.215748
70000 0.199799
80000 0.186581
90000 0.175734
100000 0.167004
110000 0.160137
120000 0.155763
130000 0.148799
140000 0.142957
150000 0.138273
160000 0.134657
170000 0.133118
180000 0.129747
190000 0.129136
200000 0.12566
210000 0.123542
220000 0.120228
230000 0.117478
240000 0.116402
250000 0.113778
260000 0.111557
270000 0.110598
280000 0.11154
290000 0.109534
300000 0.107682
310000 0.106058
320000 0.106211
330000 0.104813
340000 0.103373
350000 0.101645
360000 0.100437
370000 0.0989675
380000 0.0974332
390000 0.0960266
400000 0.0946245
410000 0.0936558
420000 0.0924548
430000 0.0912282
440000 0.0900597
450000 0.0896348
460000 0.0888232
470000 0.0879299
480000 0.0896864
490000 0.0885844
500000 0.0878966
510000 0.0869398
520000 0.0860974
530000 0.0859623
540000 0.0852847
550000 0.0843355
560000 0.0835083
570000 0.0826954
580000 0.0819635
590000 0.0811261
600000 0.0803765
610000 0.0796676
620000 0.078928
630000 0.0781086
640000 0.077509
650000 0.0769296
660000 0.0764768
670000 0.0766156
680000 0.0760607
690000 0.0756643
700000 0.0752609
710000 0.074653
720000 0.0740789
730000 0.0735235
740000 0.0730091
750000 0.0726546
760000 0.0721957
770000 0.0716352
780000 0.0712005
790000 0.0709452
800000 0.0704862
810000 0.0701706
820000 0.069642
830000 0.0691274
840000 0.0687572
850000 0.0683172
860000 0.0681157
870000 0.0677799
880000 0.0673411
890000 0.0669272
900000 0.0666326
910000 0.0663363
920000 0.0659328
930000 0.0658267
940000 0.0663566
950000 0.0660036
960000 0.0656285
970000 0.0652555
980000 0.0649786
990000 0.0646321
1000000 0.0642437
1010000 0.0639992
1020000 0.0636123
1030000 0.0633549
1040000 0.0633003
1050000 0.0629788
1060000 0.0626283
1070000 0.0623145
1080000 0.0620272
1090000 0.061699
1100000 0.0614954
1110000 0.0612704
1120000 0.0610519
1130000 0.0610448
1140000 0.0608702
1150000 0.0606069
1160000 0.0603366
1170000 0.0601034
1180000 0.0597883
1190000 0.0594134
1200000 0.0591439
1210000 0.0590659
1220000 0.0588012
1230000 0.0588001
1240000 0.0586826
1250000 0.0585176
1260000 0.0582949
1270000 0.0582739
1280000 0.0580949
1290000 0.0578982
1300000 0.0578247
1310000 0.0576187
1320000 0.0573647
1330000 0.057147
1340000 0.0569632
1350000 0.0568544
1360000 0.0566439
1370000 0.0564046
1380000 0.0562052
1390000 0.0559851
1400000 0.0557222
1410000 0.0555571
1420000 0.0553811
1430000 0.0551853
1440000 0.0550111
1450000 0.0548563
1460000 0.0545973
1470000 0.0544667
1480000 0.0542603
1490000 0.0541319
1500000 0.0539481
1510000 0.0538137
1520000 0.05366
1530000 0.0536256
1540000 0.0535356
1550000 0.0533949
1560000 0.0533212
1570000 0.0532105
1580000 0.0531147
1590000 0.0530664
1600000 0.0529372
1610000 0.052845
1620000 0.0526477
1630000 0.0524674
1640000 0.052355
1650000 0.0522833
1660000 0.0521628
1670000 0.0528087
1680000 0.052691
1690000 0.0525773
1700000 0.0525426
1710000 0.0524067
1720000 0.052358
1730000 0.0522432
1740000 0.0521699
1750000 0.0520313
1760000 0.0519061
1770000 0.0518294
1780000 0.052027
1790000 0.0520135
1800000 0.051897
1810000 0.0517603
1820000 0.0516639
1830000 0.0515861
1840000 0.0514534
1850000 0.0513172
1860000 0.0511734
1870000 0.0510545
1880000 0.0510042
1890000 0.0509496
1900000 0.0508239
1910000 0.0507804
1920000 0.0507209
1930000 0.050601
1940000 0.0504847
1950000 0.0503591
1960000 0.050321
1970000 0.051365
1980000 0.051299
1990000 0.051116
2000000 0.0511143
2010000 0.0510181
2020000 0.0508637
2030000 0.0508619
2040000 0.0507996
2050000 0.050705
2060000 0.050548
2070000 0.0504675
2080000 0.0504207
2090000 0.050393
2100000 0.0504524
2110000 0.0504143
2120000 0.0503411
2130000 0.0502623
2140000 0.0501544
2150000 0.050079
2160000 0.0499657
2170000 0.0498683
2180000 0.0498028
2190000 0.0497305
2200000 0.0510939
2210000 0.0510169
2220000 0.0510258
2230000 0.0509067
2240000 0.0507824
2250000 0.0507349
2260000 0.0506378
2270000 0.0505818
2280000 0.0507362
2290000 0.050751
2300000 0.0514052
2310000 0.0512912
2320000 0.0517031
2330000 0.0516375
2340000 0.0515603
2350000 0.0514541
2360000 0.051315
2370000 0.0512022
2380000 0.051073
2390000 0.0512242
2400000 0.0511688
2410000 0.0510276
2420000 0.0509
2430000 0.0507521
2440000 0.0507086
2450000 0.0506607
2460000 0.0505463
2470000 0.0504837
2480000 0.0504215
2490000 0.0503566
2500000 0.0502826
2510000 0.05018
2520000 0.0500809
2530000 0.0500166
2540000 0.0499276
2550000 0.0498372
2560000 0.0497305
2570000 0.0496752
2580000 0.049601
2590000 0.0495301
2600000 0.0494344
2610000 0.0493305
2620000 0.0492389
2630000 0.0491451
2640000 0.0490411
2650000 0.0490397
2660000 0.048987
2670000 0.0489012
2680000 0.0488503
2690000 0.0487712
2700000 0.0486962
2710000 0.0486339
2720000 0.048553
2730000 0.0484443
2740000 0.0483083
2750000 0.0482468
2760000 0.04815
2770000 0.0480461
2780000 0.0479829
2790000 0.0479014
2800000 0.0478402
2810000 0.0477647
2820000 0.0476636
2830000 0.0475998
2840000 0.0475122
2850000 0.0474682
2860000 0.0475176
2870000 0.0474164
2880000 0.0473373
2890000 0.0472504
2900000 0.0476721
2910000 0.0475803
2920000 0.0474641
2930000 0.047369
2940000 0.0472889
2950000 0.0472399
2960000 0.0471919
2970000 0.0471087
2980000 0.047107
2990000 0.0470256
3000000 0.046947
3010000 0.0468744
3020000 0.0468305
3030000 0.0467911
3040000 0.0466952
3050000 0.0466404
3060000 0.0465787
3070000 0.0465264
3080000 0.0464649
3090000 0.0463768
3100000 0.0463401
3110000 0.0462936
3120000 0.0462525
3130000 0.0462022
3140000 0.046166
3150000 0.0460879
3160000 0.0460551
3170000 0.0459783
3180000 0.0459055
3190000 0.0458404
3200000 0.0457778
3210000 0.0457338
3220000 0.0456827
3230000 0.0456155
3240000 0.0455916
3250000 0.0455321
3260000 0.0454974
3270000 0.0454502
3280000 0.0454067
3290000 0.0453811
3300000 0.0452974
3310000 0.0452827
3320000 0.0452117
3330000 0.0451594
3340000 0.0450741
3350000 0.0450396
3360000 0.0449842
3370000 0.0449867
3380000 0.0449321
3390000 0.0449211
3400000 0.0448655
3410000 0.0447987
3420000 0.0447408
3430000 0.0446953
3440000 0.0446377
3450000 0.0446217
3460000 0.0445955
3470000 0.0445478
3480000 0.0444995
3490000 0.0444408
3500000 0.0444097
3510000 0.0443226
3520000 0.044246
3530000 0.044216
3540000 0.0441612
3550000 0.0441099
3560000 0.0440113
3570000 0.0439335
3580000 0.0439023
3590000 0.0438402
3600000 0.0438201
3610000 0.0437689
3620000 0.0436917
3630000 0.0437126
3640000 0.0436367
3650000 0.0435559
3660000 0.0435426
3670000 0.0434931
3680000 0.0434294
3690000 0.0433823
3700000 0.0433401
3710000 0.0432894
3720000 0.0432245
3730000 0.0431654
3740000 0.0431155
3750000 0.0430535
3760000 0.0430247
3770000 0.0429923
3780000 0.0429352
3790000 0.0429455
3800000 0.0429603
3810000 0.0428973
3820000 0.0428827
3830000 0.0428415
3840000 0.0428138
3850000 0.0427596
3860000 0.0427073
3870000 0.0426482
3880000 0.0425623
3890000 0.0425285
3900000 0.042453
3910000 0.0423982
3920000 0.0423232
3930000 0.0423053
3940000 0.042281
3950000 0.0422755
3960000 0.0422185
3970000 0.042203
3980000 0.0421637
3990000 0.0421248
4000000 0.0421244
4010000 0.0421772
4020000 0.0421473
4030000 0.0421266
4040000 0.0420805
4050000 0.0420739
4060000 0.0420453
4070000 0.041991
4080000 0.0419319
4090000 0.0419061
4100000 0.0419762
4110000 0.0419544
4120000 0.0419406
4130000 0.0419217
4140000 0.0418648
4150000 0.0418381
4160000 0.0418171
4170000 0.0417822
4180000 0.0417455
4190000 0.0417388
4200000 0.0417144
4210000 0.0417051
4220000 0.0416708
4230000 0.0416188
4240000 0.0415729
4250000 0.0415588
4260000 0.0415431
4270000 0.0430977
4280000 0.0430702
4290000 0.0430416
4300000 0.043004
4310000 0.0429665
4320000 0.0429193
4330000 0.0428779
4340000 0.0430367
4350000 0.0430289
4360000 0.04301
4370000 0.0429791
4380000 0.0429795
4390000 0.0429387
4400000 0.0429144
4410000 0.0428618
4420000 0.0428399
4430000 0.0428008
4440000 0.0427572
4450000 0.0427176
4460000 0.0427075
4470000 0.0427184
4480000 0.0426792
4490000 0.0426266
4500000 0.0425795
4510000 0.0425269
4520000 0.0424934
4530000 0.042449
4540000 0.0424197
4550000 0.0423958
4560000 0.0423663
4570000 0.0423307
4580000 0.0422959
4590000 0.0422581
4600000 0.0422789
4610000 0.0422876
4620000 0.0422665
4630000 0.0422197
4640000 0.0421864
4650000 0.0421881
4660000 0.0421693
4670000 0.0421464
4680000 0.0420941
4690000 0.0420443
4700000 0.0420419
4710000 0.0420205
4720000 0.0419641
4730000 0.041926
4740000 0.0419082
4750000 0.041878
4760000 0.041822
4770000 0.0417618
4780000 0.0417516
4790000 0.0417171
4800000 0.0416647
4810000 0.0416586
4820000 0.0416333
4830000 0.041589
4840000 0.0415682
4850000 0.041567
4860000 0.0415449
4870000 0.0416043
4880000 0.0415683
4890000 0.0415531
4900000 0.0414973
4910000 0.0414637
4920000 0.0414249
4930000 0.0413681
4940000 0.0413454
4950000 0.0413335
4960000 0.0412883
4970000 0.0412551
4980000 0.041218
4990000 0.0412343
5000000 0.0412152
5010000 0.0411785
5020000 0.0411449
5030000 0.0411047
5040000 0.0410843
5050000 0.041048
5060000 0.0409807
5070000 0.0409346
5080000 0.0409012
5090000 0.040888
5100000 0.0408607
5110000 0.040846
5120000 0.0408587
5130000 0.0408239
5140000 0.0407781
5150000 0.0407584
5160000 0.0407491
5170000 0.0407346
5180000 0.0407321
5190000 0.0407021
5200000 0.0407139
5210000 0.0406848
5220000 0.0406504
5230000 0.0406226
5240000 0.0406069
5250000 0.0405762
5260000 0.0405547
5270000 0.0405512
5280000 0.0405031
5290000 0.0404889
5300000 0.0404589
5310000 0.0404989
5320000 0.0404766
5330000 0.0404253
5340000 0.0403964
5350000 0.0403818
5360000 0.0403315
5370000 0.0403368
5380000 0.0403024
5390000 0.0402996
5400000 0.0402764
5410000 0.0402465
5420000 0.0402244
5430000 0.0401845
5440000 0.0401506
5450000 0.0401272
5460000 0.0401167
5470000 0.0400781
5480000 0.0400546
5490000 0.04004
5500000 0.0400119
5510000 0.039989
5520000 0.0399705
5530000 0.0399854
5540000 0.0399464
5550000 0.0399131
5560000 0.0399048
5570000 0.0398991
5580000 0.0398889
5590000 0.0398864
5600000 0.0398615
5610000 0.0398388
5620000 0.0398393
5630000 0.0398105
5640000 0.0397855
5650000 0.0397424
5660000 0.0397092
5670000 0.0396983
5680000 0.0397014
5690000 0.0396894
5700000 0.0396734
5710000 0.0396469
5720000 0.0396626
5730000 0.0396494
5740000 0.0395955
5750000 0.0396705
5760000 0.039634
5770000 0.0396245
5780000 0.0396158
5790000 0.0396005
5800000 0.0395878
5810000 0.0395687
5820000 0.0395207
5830000 0.039486
5840000 0.0394585
5850000 0.0394157
5860000 0.0393925
5870000 0.0393763
5880000 0.0393475
5890000 0.0394233
5900000 0.0393986
5910000 0.0393747
5920000 0.039337
5930000 0.0393253
5940000 0.0392952
5950000 0.039277
5960000 0.0392639
5970000 0.0392457
5980000 0.0392238
5990000 0.03919
6000000 0.0391522
6010000 0.0391519
6020000 0.0391333
6030000 0.0391156
6040000 0.0391003
6050000 0.039093
6060000 0.0390748
6070000 0.0390642
6080000 0.0390387
6090000 0.0390136
6100000 0.0389557
6110000 0.0389641
6120000 0.0389559
6130000 0.0389344
6140000 0.0389007
6150000 0.0388804
6160000 0.0389089
6170000 0.0388759
6180000 0.038859
6190000 0.0388419
6200000 0.0388328
6210000 0.0388174
6220000 0.0387925
6230000 0.0387829
6240000 0.0387629
6250000 0.0387507
6260000 0.0387208
6270000 0.0386884
6280000 0.0386557
6290000 0.0386279
6300000 0.0386
6310000 0.0385921
6320000 0.0385537
6330000 0.0386452
6340000 0.0386149
6350000 0.0386026
6360000 0.0385625
6370000 0.0385514
6380000 0.038539
6390000 0.0385158
6400000 0.0385057
6410000 0.0384917
6420000 0.0384696
6430000 0.0384376
6440000 0.0384008
6450000 0.0383897
6460000 0.0383645
6470000 0.0383295
6480000 0.0383048
6490000 0.0382755
6500000 0.0382503
6510000 0.0382423
6520000 0.0382489
6530000 0.0382393
6540000 0.0382163
6550000 0.0381941
6560000 0.0381744
6570000 0.0381579
6580000 0.0381323
6590000 0.0381083
6600000 0.0380991
6610000 0.03807
6620000 0.0380507
6630000 0.0380383
6640000 0.038031
6650000 0.0380149
6660000 0.0379906
6670000 0.0379815
6680000 0.0379778
6690000 0.0379719
6700000 0.0379568
6710000 0.0379546
6720000 0.0379256
6730000 0.0379144
6740000 0.0379116
6750000 0.0378975
6760000 0.0378901
6770000 0.0378776
6780000 0.0378727
6790000 0.037846
6800000 0.0378423
6810000 0.0378302
6820000 0.0378035
6830000 0.0377866
6840000 0.0377708
6850000 0.0377695
6860000 0.0377528
6870000 0.0377199
6880000 0.0376953
6890000 0.0376835
6900000 0.0376671
6910000 0.0376592
6920000 0.0376586
6930000 0.0376687
6940000 0.0376492
6950000 0.0376179
6960000 0.0376026
6970000 0.0376309
6980000 0.0376108
6990000 0.0375904
7000000 0.0375781
7010000 0.0375682
7020000 0.0375573
7030000 0.0375496
7040000 0.0375432
7050000 0.0375383
7060000 0.0375177
7070000 0.0375
7080000 0.0374728
7090000 0.0374473
7100000 0.0374186
7110000 0.0374064
7120000 0.0373725
7130000 0.0373819
7140000 0.0373736
7150000 0.0373387
7160000 0.0373268
7170000 0.0372891
7180000 0.0372537
7190000 0.0372451
7200000 0.0372431
7210000 0.0372151
7220000 0.0372228
7230000 0.037209
7240000 0.0371847
7250000 0.0371751
7260000 0.0371505
7270000 0.0371427
7280000 0.037122
7290000 0.0371183
7300000 0.0371229
7310000 0.0371366
7320000 0.0371039
7330000 0.0370849
7340000 0.0370771
7350000 0.037059
7360000 0.0370431
7370000 0.0370292
7380000 0.0370048
7390000 0.0369883
7400000 0.0369575
7410000 0.037324
7420000 0.037316
7430000 0.0373086
7440000 0.0373196
7450000 0.0373056
7460000 0.037284
7470000 0.0372751
7480000 0.0372544
7490000 0.037242
7500000 0.0372308
7510000 0.0372326
7520000 0.0372089
7530000 0.0372071
7540000 0.0371574
7550000 0.0371175
7560000 0.0371058
7570000 0.0370961
7580000 0.0370712
7590000 0.0370807
7600000 0.037075
7610000 0.0370596
7620000 0.0370543
7630000 0.0370387
7640000 0.0370111
7650000 0.0370078
7660000 0.0369972
7670000 0.0369861
7680000 0.0369779
7690000 0.0369663
7700000 0.0369448
7710000 0.0369346
7720000 0.0369019
7730000 0.0368887
7740000 0.0368795
7750000 0.0368707
7760000 0.0368788
7770000 0.0368461
7780000 0.0368683
7790000 0.0368555
7800000 0.0368574
7810000 0.0368419
7820000 0.0368303
7830000 0.0368165
7840000 0.036826
7850000 0.0368067
7860000 0.0368139
7870000 0.0368049
7880000 0.0367887
7890000 0.0367891
7900000 0.0368412
7910000 0.0368248
7920000 0.0368277
7930000 0.0368111
7940000 0.0368017
7950000 0.0367931
7960000 0.0367543
7970000 0.0367278
7980000 0.0366962
7990000 0.036679
8000000 0.0366831
8010000 0.0366714
8020000 0.0366395
8030000 0.0366231
8040000 0.0366163
8050000 0.0365992
8060000 0.0365869
8070000 0.0365654
8080000 0.0365502
8090000 0.0365363
8100000 0.0365096
8110000 0.0364925
8120000 0.0364769
8130000 0.0364613
8140000 0.0364545
8150000 0.0364569
8160000 0.0364342
8170000 0.0364159
8180000 0.0364026
8190000 0.036392
8200000 0.036388
8210000 0.036366
8220000 0.0363528
8230000 0.0363441
8240000 0.0363233
8250000 0.0363084
8260000 0.0362963
8270000 0.0362863
8280000 0.0362952
8290000 0.0362943
8300000 0.0362878
8310000 0.0362707
8320000 0.0362545
8330000 0.0362467
8340000 0.0362374
8350000 0.0362371
8360000 0.0362292
8370000 0.036196
8380000 0.0361894
8390000 0.036167
8400000 0.0361661
8410000 0.0361479
8420000 0.03614
8430000 0.03613
8440000 0.0361176
8450000 0.0361095
8460000 0.0361034
8470000 0.0361054
8480000 0.0360994
8490000 0.0360987
8500000 0.0360892
8510000 0.0360779
8520000 0.0360634
8530000 0.0360448
8540000 0.0360236
8550000 0.0360142
8560000 0.0360036
8570000 0.0359898
8580000 0.0359746
8590000 0.0360767
8600000 0.0360698
8610000 0.0360571
8620000 0.0360699
8630000 0.0360642
8640000 0.0360603
8650000 0.0360469
8660000 0.0360237
8670000 0.0360088
8680000 0.0359984
8690000 0.0359926
8700000 0.0359871
8710000 0.0359899
8720000 0.0359856
8730000 0.0359929
8740000 0.0359891
8750000 0.0359697
8760000 0.0359529
8770000 0.0359525
8780000 0.0359558
8790000 0.0359328
8800000 0.0359282
8810000 0.0359072
8820000 0.0358997
8830000 0.0358919
8840000 0.0358857
8850000 0.0358674
8860000 0.0358673
8870000 0.0358626
8880000 0.0358463
8890000 0.0358493
8900000 0.0358332
8910000 0.035833
8920000 0.0358249
8930000 0.0358084
8940000 0.0357999
8950000 0.0357884
8960000 0.0357716
8970000 0.0357701
8980000 0.0357635
8990000 0.035759
9000000 0.0357522
9010000 0.0357536
9020000 0.035732
9030000 0.0356897
9040000 0.0356809
9050000 0.03568
9060000 0.0356823
9070000 0.0356686
9080000 0.0356789
9090000 0.0356735
9100000 0.0356665
9110000 0.0356539
9120000 0.0356563
9130000 0.0356663
9140000 0.0356608
9150000 0.0356538
9160000 0.0356465
9170000 0.0356391
9180000 0.0356339
9190000 0.0356158
9200000 0.0355977
9210000 0.0355895
9220000 0.0355714
9230000 0.0355644
9240000 0.0355717
9250000 0.0355606
9260000 0.035556
9270000 0.0355335
9280000 0.0355204
9290000 0.0355128
9300000 0.0354955
9310000 0.0354855
9320000 0.0354773
9330000 0.0354656
9340000 0.0354609
9350000 0.0354502
9360000 0.0354488
9370000 0.0354338
9380000 0.0354301
9390000 0.0354239
9400000 0.0354142
9410000 0.0354013
9420000 0.0353924
9430000 0.035385
9440000 0.0353854
9450000 0.0353824
9460000 0.0353804
9470000 0.0353567
9480000 0.0353529
9490000 0.0353432
9500000 0.0353294
9510000 0.0353153
9520000 0.0352945
9530000 0.0352866
9540000 0.0352741
9550000 0.035255
9560000 0.0352419
9570000 0.0352236
9580000 0.0352176
9590000 0.0351975
9600000 0.0352052
9610000 0.0352011
9620000 0.0351752
9630000 0.0351685
9640000 0.0351743
9650000 0.0351743
9660000 0.0351788
9670000 0.0351577
9680000 0.0351378
9690000 0.0351286
9700000 0.0351137
9710000 0.0351016
9720000 0.0351322
9730000 0.0351261
9740000 0.0351105
9750000 0.0351107
9760000 0.0350935
9770000 0.0350857
9780000 0.0350591
9790000 0.0350621
9800000 0.0350577
9810000 0.0350421
9820000 0.0350356
9830000 0.0350295
9840000 0.0350076
9850000 0.0349984
9860000 0.0349896
9870000 0.0350006
9880000 0.0349854
9890000 0.0350236
9900000 0.0350176
9910000 0.0350016
9920000 0.0349905
9930000 0.0349756
9940000 0.0349535
9950000 0.0349573
9960000 0.0349549
9970000 0.0349422
9980000 0.0349379
9990000 0.0349246
10000000 0.034916

